When Can We Learn General-Sum Markov Games with a Large Number of Players Sample-Efficiently?

Multi-agent reinforcement learning has made substantial empirical progresses in solving games with a large number of players. However, theoretically, the best known sample complexity for finding a Nash equilibrium in general-sum games scales exponentially in the number of players due to the size of the joint action space, and there is a matching exponential lower bound. This paper investigates what learning goals admit better sample complexities in the setting of $m$-player general-sum Markov games with $H$ steps, $S$ states, and $A_i$ actions per player. First, we design algorithms for learning an $\epsilon$-Coarse Correlated Equilibrium (CCE) in $\widetilde{\mathcal{O}}(H^5S\max_{i\le m} A_i / \epsilon^2)$ episodes, and an $\epsilon$-Correlated Equilibrium (CE) in $\widetilde{\mathcal{O}}(H^6S\max_{i\le m} A_i^2 / \epsilon^2)$ episodes. This is the first line of results for learning CCE and CE with sample complexities polynomial in $\max_{i\le m} A_i$. Our algorithm for learning CE integrates an adversarial bandit subroutine which minimizes a weighted swap regret, along with several novel designs in the outer loop. Second, we consider the important special case of Markov Potential Games, and design an algorithm that learns an $\epsilon$-approximate Nash equilibrium within $\widetilde{\mathcal{O}}(S\sum_{i\le m} A_i / \epsilon^3)$ episodes (when only highlighting the dependence on $S$, $A_i$, and $\epsilon$), which only depends linearly in $\sum_{i\le m} A_i$ and significantly improves over existing efficient algorithm in the $\epsilon$ dependence. Overall, our results shed light on what equilibria or structural assumptions on the game may enable sample-efficient learning with many players.

==> Sections/Conclusion.tex <==
\section{Conclusion}
This paper investigates the question of when can we solve general-sum Markov games (MGs) sample-efficiently with a mild dependence on the number of players. Our results show that this is possible for learning approximate (Coarse) Correlated Equilibria in general-sum MGs, as well as learning approximate Nash equilibrium in Markov potential games. In both cases, our sample complexity bounds improve over existing results in many aspects. Our work opens up many interesting directions for future work, such as sharper algorithms for both problems, sample complexity lower bounds, or how to perform sample-efficient learning in general-sum MGs with function approximations. In addition to Markov potential games, it would also be interesting to explore alternative structural assumptions that permit sample-efficient learning.

\section*{Acknowledgement}
Ziang Song is partially supported by the elite undergraduate training program of School of
Mathematical Sciences in Peking University.


==> Sections/MPG.tex <==
\section{Learning Nash Equilibria in Markov Potential Games}
\label{sec:MPG}


%With the setting in [Li Na's <Gradient Play...>]. For softmax parameterization:
% \begin{align*}
%     \pi_{i,\theta_i}(a_i|s)=\frac{\exp \theta_{s,a_i}}{\sum_{a_j\in\mc{A}_i}\exp \theta_{s,a_j}}.
% \end{align*}
% Since this is a differentiable parameterization that explicitly constrains $\pi_\theta(\cdot|s)$ to be in the simplex, then we have
% \begin{align*}
%     \nabla_{\theta} \mathbb{E}_{s_{0} \sim \rho} V_{i}^{\theta}\left(s_{0}\right)=\frac{1}{1-\gamma} \mathbb{E}_{s \sim d_{\theta}} \mathbb{E}_{a \sim \pi_{\theta}(\cdot | s)}\left[\nabla_{\theta} \log \pi_{\theta}(a \mid s) A_{i}^{\theta}(s, a)\right], \quad i=1,2, \ldots, n.
% \end{align*}
% Moreover, we have
% \begin{align*}
%     \frac{\partial \log \pi_{\theta}\left(a^{\prime} | s^{\prime}\right)}{\partial \theta_{s, a_{i}}}=\frac{\partial \log \pi_{\theta_{i}}\left(a_{i}^{\prime} | s^{\prime}\right)}{\partial \theta_{s, a_{i}}} &=\textbf{1}\left\{ s^{\prime}=s\right\} \paren{\textbf{1}\{a'=a\}-\pi_{\theta_i}(a_i|s)}\\
% &=\textbf{1}\left\{a_{i}^{\prime}=a_{i}, s^{\prime}=s\right\} -\textbf{1}\{s'=s\}\pi_{\theta_i}(a_i|s).
% \end{align*}
% So we can prove that
% \begin{lemma}
% $$\frac{\partial J_i(\theta)}{\partial \theta_{s,a_i}} =\frac{1}{1-\gamma} d_\theta(s)\pi_{\theta_i}(a_i|s) \up{A_i^\theta}(s,a_i). $$
% Moreover, if this is a Markov Potential Game(MPG) with potential function $\Phi$, then
% $$
% \frac{\partial \Phi (\theta)}{\partial \theta_{s,a_i}}=\frac{\partial J_i(\theta)}{\partial \theta_{s,a_i}} =\frac{1}{1-\gamma} d_\theta(s)\pi_{\theta_i}(a_i|s) \up{A_i^\theta}(s,a_i). 
% $$
% \end{lemma}
% Another important lemma is the \textbf{Performance difference lemma}:
% \begin{align*}
%     J_{i}\left(\theta^{\prime}\right)-J_{i}(\theta)=\frac{1}{1-\gamma} \mathbb{E}_{s \sim d_{\theta^{\prime}}} \mathbb{E}_{a \sim \pi_{\theta^{\prime}}} A_{i}^{\theta}(s, a), \quad i=1,2, \ldots, n.
% \end{align*}

% The NPG algorithm defines a Fisher information matrix
% (induced by $\pi$), and performs gradient updates in the geometry induced by this matrix as follows:
% \begin{align*}
%     \begin{array}{l}
% F_{\rho}(\theta)=\mathbb{E}_{s \sim d_\theta(\cdot)} \mathbb{E}_{a \sim \pi_{\theta}(\cdot| s)}\left[\nabla_{\theta} \log \pi_{\theta}(a | s)\left(\nabla_{\theta} \log \pi_{\theta}(a | s)\right)^{\top}\right] \\
% \theta^{(t+1)}=\theta^{(t)}+\eta F_{\rho}\left(\theta^{(t)}\right)^{\dagger} \nabla_{\theta} \Phi(\theta^{(t)}).
% \end{array}
% \end{align*}

% In multi-player case, this update rule doesn't have a convenient form.(?)

% Alternatively, we can consider another update rule. In each step, we perform NPG update for each single player (fix other players' policy) simultaneously ,i.e.
% \begin{align*}
%     \pi_i^{(t+1)}(a_i | s)=\pi_i^{(t)}(a_i | s) \frac{\exp \left(\eta \up{A_i^{\theta^{(t)}}}(s, a_i) /(1-\gamma)\right)}{Z_{i,t}(s)}, \quad i=1,2, \ldots, n.
% \end{align*}
% By performance difference lemma, 
% $$
% J_{i}\left(\theta_{i}^{\prime}, \theta_{-i}\right)-J_{i}\left(\theta_{i}, \theta_{-i}\right)=\frac{1}{1-\gamma} \sum_{s, a_{i}} d_{\theta^{\prime}}(s) \pi_{\theta_{i}^{\prime}}\left(a_{i} \mid s\right) \overline{A_{i}^{\theta}}\left(s, a_{i}\right),
% $$
% it's not difficult to get
% $$
% J_i(\theta_i^{(t+1)},\theta_{-i}^{(t)})-
% J_i(\theta_i^{(t)},\theta_{-i}^{(t)})\ge
% \frac{1-\gamma}{\eta}\mathbb{E}_{s_0\sim\rho}\log Z_{i,t}(s_0)\ge 0.
% $$
% By the definition of MPG, this becomes
% $$
% \Phi(\theta_i^{(t+1)},\theta_{-i}^{(t)})-
% \Phi(\theta_i^{(t)},\theta_{-i}^{(t)})\ge
% \frac{1-\gamma}{\eta}\mathbb{E}_{s_0\sim\rho}\log Z_{i,t}(s_0)\ge 0
% $$

% If we update each player's policy sequentially, we can get a coordinate ascent algorithm for $\Phi$.
% By performance difference lemma, 
% \begin{align*}
%   J_{i}\left(\theta_{i}^*, \theta_{-i}\right)-J_{i}\left(\theta_{i}, \theta_{-i}\right)
%   &=\frac{1}{1-\gamma} \sum_{s, a_{i}} d_{\theta^*}(s) \pi_{\theta_{i}^*}\left(a_{i} \mid s\right) \overline{A_{i}^{\theta}}\left(s, a_{i}\right) 
% \end{align*}


In this section, we consider learning Nash equilibria in Markov Potential Games (MPGs), an important subclass of general-sum MGs. Despite the curse of number of players of learning Nash in general-sum MGs, recent work shows that learning Nash in MPGs does not require sample size exponential in $m$, by using stochastic policy gradient based algorithms~\citep{leonardos2021global, zhang2021gradient}. In this section, we provide an alternative algorithm \nashca~that also achieves a mild dependence on $m$ and an improved dependence on $\eps$ by a simple reduction to single-agent learning.

% In particular, they show that this problem can be solved by the policy gradient algorithm with sample complexity $\mc{O}(\sum_{i = 1}^m A_i / \eps^6)$\ziang{how to change this sample complexity?}. In this section, we provide a simple algorithm \nashca~that achieves a better sample complexity bound $\mc{O}(\sum_{i = 1}^m A_i / \eps^3)$. 

\subsection{Markov potential games}

We first present the definition of MPGs. Our definition is the finite-horizon variant\footnote{Our results can easily adapted to the discounted infinite time horizon setup.} of the definitions of \citet{macua2018learning,leonardos2021global,zhang2021gradient} and is slightly more general as we only require~\eqref{equation:VPhi_potential} on the total return. Throughout this section, $\pi$ denotes a Markov product policy.
\begin{definition}(Markov potential games)
A general-sum Markov game is a Markov potential game if there exists a potential function $\Phi$ mapping any product policy to a real number in $[0, \Phimax]$,
%$\Phi:(\Delta_{\mc{A}_1})^H\times\cdots\times (\Delta_{\mc{A}_m})^H \to[0, \Phimax]$
such that for any $i \in [m]$, any two policies $\pi_i, \pi_i'$ of the \ith player, and any policy $\pi_{-i}$ of other players, the difference of the value functions of the \ith player with policies $(\pi_i, \pi_{-i})$ and $(\pi_i', \pi_{-i})$ is equals the difference of the potential function on the same policies, i.e., 
\begin{equation}
\label{equation:VPhi_potential}
   V_{1,i}^{\pi_i,\pi_{-i}}(s_1)-V_{1,i}^{\pi'_i,\pi_{-i}}(s_1)=\Phi(\pi_i,\pi_{-i})-\Phi(\pi_i',\pi_{-i}). 
\end{equation}
\end{definition}

%Comparing to the definition in \cite{macua2018learning}, we only assume a potential function $\Phi$ indexed by the policy of all players. Our definition is also more general than \cite{leonardos2021global} where the definition needs $s$ potential function for every initial state. \sm{These two sentences need to be modified. } %In Markov potential games, if one player change its policy, the change in its value function equals the change in the  potential function. Then we point a special class of Markov potential games.

% \paragraph{Markov cooperative games}
%\ziang{cooperative or cooperative?} \sm{Cooperative} 

%  (by shifting by a constant if necessary).

Note that the range of the potential function $\Phimax$ admits a trivial upper bound $\Phimax \le mH$ (this can be seen by varying $\pi_i$ for one $i$ at a time). An important example of MPGs is Markov Cooperative Games (MCGs) where all players share the same reward $r_i\equiv r$. 
%~\citep{claus1998dynamics}
% dding a constant on $\Phi$ doesn't affect the value of $\Phi(\pi_i,\pi_{-i})-\Phi(\pi_i',\pi_{-i})$. So with out loss of generality, we assume $\min_\pi\Phi(\pi)=0$. 



% More specifically, a MCG is a general-sum MG in which all players receive the same reward in each time step, i.e. $r_{h,i}=r_h$ for any $i \in [m]$ and $h \in [H]$. We can thus define the potential function of the MCG as the value function of any player $\Phi(\pi)=V_{1,i}^\pi(s_1)$, so that a MCG is a MPG. It is interesting to note that one can view a MCG as a MDP with action space $\otimes_{i \in [m]} \mc{A}_i$, and the optimal policy of the MDP is a Nash equilibrium of the MCG. Consequently, any reinforcement learning algorithm learning the $\eps$-optimal policy of the MDP returns an $\eps$-approximate Nash equilibrium of the MCG. However, any such algorithm will require $\Omega(\prod_{i\in [m]} A_i / \eps^2)$ samples, which is not efficient when the number of players $m$ is large. 

%Multi-agent reinforcement learning can be formulated as Markov cooperative games. However, because potential games are general than cooperative games, Markov cooperative games is a proper subset of MPGs. 


% \paragraph{State-based potential games v.s. MPGs}Potential games have been studied extensively, the MPG can be seen as a generalization of potential games ($H=1,S=1$). If for a Markov games, in each state $s$ and step  $h$, the reward $r_h(s,\bm{a})$ admits a potential function, i.e. $r_h(s,a_i,\bm{a}_{-i})-r_h(s,a_i',\bm{a}_{-i})=\phi(a_i,\bm{a}_{-i})-\phi(a_i',\bm{a}_{-i})$, we call this game a state-based potential game. In \cite{leonardos2021global}, Example 1 and Example 2 illustrate that a state-based potential game doesn't have to be a MPG and Example 3 illustrates that a MPG doesn't have to be a state-based potential game. Moreover, Proposition 3.2 in \cite{leonardos2021global} gives the sufficient condition for a state-based potential game to be a MPG. The difference between state-based potential games and MPGs is the consequence of transitions which add a lot complexity.~\yub{remove discussion about state-based since this is a patheological definition as we already see in Leonardos, and irrelevant to our result.}


%Pure-strategy Nash equilibrium is attractive because each player can take action deterministically. Note that the left side of (\ref{equation:VPhi_potential}) can be seen as the difference of two value function. Therefore, when $\pi_{-i}$ and $\pi_i'$ are fixed, allowing $\pi_i$ to change. The left side can be maximized by a pure-strategy policy $\pi_i^\star$. So there exists a global maximizer $\pi^\star$ of $\Phi$ such that $\pi$ is a pure-strategy policy. By (\ref{equation:VPhi_potential}), we have for any $i$
% $$
% V_{1,i}^{\pi_i,\pi_{-i}}(s_1)-V_{1,i}^{\pi'_i,\pi_{-i}}(s_1)=\Phi(\pi_i,\pi_{-i})-\Phi(\pi_i',\pi_{-i})\ge0.
% $$
% So $\pi^\star$ is a Nash equilibrium. This gives a important feature of MPGs:

%A particular property of MPGs is that, there always exists a pure-strategy Nash equilibrium (see Appendix \ref{sec:MPG_pure_strategy_proof} for a proof). Such a property does not hold for every general-sum MG. Pure-strategy Nash equilibria are preferred in many scenarios \sm{example? citation?} since each player can take deterministic actions. In this section, we will focus on learning a pure-strategy Nash equilibrium of MPGs. 

% Pure-strategy Nash equilibrium is attractive because each player can take deterministic actions. Note that the left side of (\ref{equation:VPhi_potential}) can be seen as the difference of two value function. Therefore, when $\pi_{-i}$ and $\pi_i'$ are fixed, allowing $\pi_i$ to change. The left side can be maximized by a pure-strategy policy $\pi_i^\star$. So there exists a global maximizer $\pi^\star$ of $\Phi$ such that $\pi$ is a pure-strategy policy. By (\ref{equation:VPhi_potential}), we have for any $i$
% $$
% V_{1,i}^{\pi_i,\pi_{-i}}(s_1)-V_{1,i}^{\pi'_i,\pi_{-i}}(s_1)=\Phi(\pi_i,\pi_{-i})-\Phi(\pi_i',\pi_{-i})\ge0.
% $$
% So $\pi^\star$ is a Nash equilibrium. This gives a important feature of MPGs:

%\ziang{approximate Nash}
%Pure-strategy Nash equilibrium is attractive because each player can take action deterministically. In fact, any coordinate-wisely local maximizer of $\Phi$ gives a Nash equilibrium for the MPG. We can take advantage of this structure to learn a Nash equilibrium. 

%In the following, we present an algorithm to efficiently learn an $\epsilon$-approximate pure-strategy Nash equilibrium.  

%\yub{directly used Equation (1) to define, then say previous literature assumes slightly stronger potential game structure, such as decomposable potential function, or equation (1) for every state, not just initial state.}\ziang{$\surd$}


%\subsection{Algorithm with iteration complexity $\frac{Cn(\Phi_{\text{max}}-\Phi_{\text{min}})}{(1-\gamma)^2\epsilon^2}$}


%\paragraph{Analysis:}
%For Algorithm \ref{NPG_general}, each time we update the policy, we have
%$$
%\Phi(\hat\pi_i,\pi_{-i})-\Phi(\pi) = J_i(\hat\pi_i,\pi_{-i})-J_i(\pi)\ge \epsilon/2 .
%$$
%So there are at most $2(\Phi_{\text{max}}-\Phi_{\text{min}})/\epsilon$ times update. On the other hand, if $\Delta\le\epsilon/2$, we have for all $i\in[n]$,
%\begin{align*}
%    J_i(\pi_i^*,\pi_{-i})-J_i(\pi)&=J_i(\pi_i^*,\pi_{-i})-J_i(\hat\pi_i,\pi_{-i})+J_i(\hat\pi_i,\pi_{-i})-J_i(\pi)\\
%    &\le \epsilon/2+\epsilon/2 .
%\end{align*}
%The inequality follows from the convergence rate of NPG and $\Delta\le\epsilon/2$.

%Overall, we need $\frac{2n(\Phi_{\text{max}}-\Phi_{\text{min}})}{\epsilon}$ times NPG, each NPG iterate $T=\frac{4}{(1-\gamma)^2\epsilon}$ times.

%\paragraph{Sample complexity:} While NPG update in subroutine gives a low iteration complexity, we can replace NPG with any other algorithm.

\subsection{Algorithm and theoretical guarantee}

% \paragraph{Algorithm description}
We present a simple algorithm \nashca~(Nash Coordinate Ascent) for learning an $\eps$-Nash in MPGs. 
As its name suggests, the algorithm operates by solving single-agent Markov Decision Processes (MDPs) one player at a time, and intrinsically performing coordinate ascent on the potential function of the Markov game. Due to the potential structure of MPGs and the boundedness of the potential function, the local improvements of players across the steps can have an accumulative effect on the potential function, and the algorithm is guaranteed to stop after a bounded number of steps. We give the full description of the \nashca~in Algorithm \ref{algorithm:BR_general}. We remark that \nashca~is additionally guaranteed to output a \emph{pure-strategy} Nash equilibrium (cf. Appendix~\ref{section:proof in MPG} for definition). 

% \paragraph{Algorithm description}
% In each step of the while loop of Algorithm \ref{algorithm:BR_general}, we first search for an $\eps/8$-optimal policy for each player while fixing the policies of all other players. Note that by fixing all other players' policies, such a Markov game becomes an MDP, so we can use any standard RL algorithm (e.g. \ucbviuplow) to search for the approximate optimal policy (best response) of each player. Next, in each step of the while loop, we only modify the policy of the player with the largest estimated increment on the potential function. Due to the ``potential'' structure of the Markov potential game and the boundedness of the potential function, the local improvements of players across the steps can have an accumulative effect on the potential function, and the while loop is guaranteed to stop after a bounded number of steps. When the loop stops, it is guaranteed that no player can improve their policy by $\eps$, so that the policy at the stopping time is an $\eps$-approximate Nash equilibrium. 


%Our algorithm consists of Algorithm \ref{algorithm:BR_general} and Algorithm \ref{algorithm:NEgap}. During execution, we try to maximize $\Phi$. For the \ith player, when we fix other player's policy, we can find a near best response policy for the \ith player $\hat\pi_i$. 

%To find the best response of the \ith player, the policy of the others' policies are incorporated with the environment. In view of the \ith player, find a best response is equivalent with finding an optimal policy in an MDP with stochastic reward.





%On one hand, by the definition, $\pi$ is $\epsilon$-approximate Nash equilibrium if the most significant improvement is no bigger than $\epsilon$. On the other hand, the improvement on $V_{1,i}$ is also improvement on $\Phi$ by (\ref{equation:VPhi_potential}). Because of the boundness of the   potential function, in Algorithm \ref{algorithm:BR_general}, the loop would stop in finite time. 

%Finally, Algorithm \ref{algorithm:BR_general} together with Algorithm \ref{algorithm:NEgap} would learn a $\epsilon$-approximate pure-strategy Nash equilibrium.







% \subsection{Sample complexity}
%\yub{In this algorithm, use UCBVI-UPLOW to output a pure strategy. But mention that any efficient RL algorithm also works in principle, we only use this because it gives a pure strategy with high probability.}

% We give the sample complexity bound of the Nash-CA algorithm in the following theorem. 

\begin{algorithm}[t]
% \setstretch{1.2}
   \caption{\nashca~for Markov potential games}
   \label{algorithm:BR_general}
   \begin{algorithmic}[1]
   \REQUIRE Error tolerance $\epsilon$
   \STATE {\bfseries Initialize:} $\pi=\set{\pi_{i}}_{i\in [m]}$, where $\pi_i = \set{\pi_{h,i}}_{(h,i)\in[H]\times[m]}$ for some deterministic policy $\pi_{h, i}$. %and $\pi_{h,i}(a_i|s)=\indic{a_i=a_{i,s,h}^0}$ for $a_{i,s,h}^0 \in \mc{A}_i$.
      \WHILE{true}
      \STATE Execute policy $\pi$ for $N = \Theta(\frac{H^2\iota}{\eps^2})$ episodes and obtain $\hat V_{1,i}(\pi)$ which is the empirical average of the total return under policy $\pi$.
      \FOR{player $i=1,\dots,m$}
      \STATE Fix $\pi_{-i}$, and let the \ith player run \ucbviuplow~(Algorithm~\ref{algorithm:ucbviuplow}) for $ K_i = \Theta(\frac{H^3SA_i\iota}{\epsilon^2}+\frac{H^3S^2A_i\iota^2}{\eps})$  episodes and get a new deterministic policy $\hat\pi_i$.%~\yub{use Azar et al.}
      \STATE Execute policy $(\hat{\pi}_i,\pi_{-i})$ for $N= \Theta(\frac{H^2\iota}{\eps^2})$ episodes and obtain $\hat V_{1,i}(\hat\pi_i,\pi_{-i})$ which is the empirical average of the total return under policy $(\hat\pi_i,\pi_{-i})$. 
      \STATE Set $\Delta_i \setto \hat V_{1,i}(\hat\pi_i,\pi_{-i})-\hat V_{1,i}(\pi)$.
      \ENDFOR
      \IF{$\max_{i\in[m]} {\Delta_i} > \epsilon/2$}
      \STATE Update $\pi_j \setto \hat \pi_j$ where $j = \arg\max_{i\in[m]} {\Delta_i}$.
      \ELSE 
      \RETURN $\pi$
      \ENDIF
      \ENDWHILE
   \end{algorithmic}
\end{algorithm}

\begin{theorem}[Sample complexity for \nashca]
\label{theorem:sample_complexity_general-sum}
For Markov potential games, with probability at least $1-p$, Algorithm \ref{algorithm:BR_general} terminates within $4\Phi_\text{max}/\eps$ steps of the while loop, and outputs an $\epsilon$-approximate (pure-strategy) Nash equilibrium. The total episodes of play is at most
\begin{align*}
    K = \cO \left(\frac{\Phimax H^3S\sum_{i=1}^m A_i \iota}{\epsilon^3}+\frac{\Phimax H^3S^2\sum_{i=1}^m A_i\iota^2}{\epsilon^2}\right),
\end{align*}
where $\iota = \log(\frac{mHSK\max_{1\le i\le m} A_i }{\epsilon p})$ is a log factor.
\end{theorem}
% \ziang{as long as,..., $K\ge$ $\to$ with...,$K=$? }

\paragraph{Discussions}
For small enough $\eps$, the sample complexity for the \nashca~algorithm in the above theorem is $\tO(\Phimax H^3S\sum_{i\le m}A_i / \eps^3)$. As $\Phi_{\max}\le m H$, this at most scales with the number of players as $m\sum_{i\le m}A_i$, which is much better than the exponential in $m$ sample complexity for general-sum MGs without additional structures. Compared with recent results on learning Nash via policy gradients~\citep{leonardos2021global,zhang2021gradient}, the \nashca~algorithm also achieves ${\rm poly}(m, \max_{i\le m}A_i)$ dependence, and significantly improves on the $\epsilon$ dependence from their $\epsilon^{-6}$ to $\epsilon^{-3}$. In addition, our algorithm does not require assumptions on bounded distribution mismatch coefficient as they do, due to the exploration nature of our single-agent MDP subroutine.

Also, compared with the sample complexity bound $\widetilde{\mc{O}}(H^4S^2\prod_{i=1}^mA_i/\epsilon^2)$ of the Nash-VI algorithm~\citep{liu2021sharp} for general-sum MGs (not restricted to MPGs), our \nashca~algorithm doesn't suffer from the exponential dependence on $m$ thanks to the MPG structure. We do achieve a looser in the dependence on $\eps$, yet overall our sample complexity is still better unless $\epsilon < ( \sum_{i=1}^m A_i)/( \prod_{i=1}^m A_i)$ is exponentially small. The proof of Theorem~\ref{theorem:sample_complexity_general-sum} can be found in Appendix~\ref{section:proof in MPG}.

% Moreover, the Nash-CA algorithm doesn't have to suffer from the distribution mismatch coefficient in the sample complexity bound of policy gradient algorithms, which could be quite large in some cases.

%As another minor difference, the Nash-CA algorithm always outputs a pure-strategy policy, where Nash-VI algorithm does not. 
%\yub{Compare with Nash-VI. Say in passing that, their algorithm works for any general-sum MG, but cannot give pure strategy Nash when restricted to MPG.}\ziang{$\surd$}

%It' worth noticing that under some special cases, our algorithm has more optimal sample complexity. For example, if each player's reward only depend on it's own action and the state, Algorithm \ref{algorithm:BR_general} would stop before $m+1$ loops. The overall sample complexity is $\widetilde{O} (H^3Sm\sum_{i=1}^mA_i/\epsilon^2)$. \yub{Can we formalize a general good case and write a Corollary?}

\paragraph{A lower bound} To accompany Theorem~\ref{theorem:sample_complexity_general-sum}, we establish a sample complexity lower bound of $\Omega(H^2\sum_{i = 1}^m A_i / \eps^2)$ for learning pure-strategy Nash in MCGs and hence MPGs (Theorem~\ref{theorem:MDP_lowerbound} in Appendix~\ref{app:MPG-lower-bound}). This lower bound improves in the $A_i$ dependence over the naive reduction to single-player MDPs~\citep{domingues2021episodic}, which gives $\Omega(H^3S\max_{i\in[m]} A_i/\eps^2)$, though is loose on the $S, H$ dependence. The improved $A_i$ dependence is achieved by constructing a novel class of hard instances of on one-step games (Lemma~\ref{lemma:matrix_game_lowerbound2}), which may be of further technical interest. However, there is still a large gap between these lower bounds and the best current upper bound of either our $\tO(\sum_{i = 1}^m A_i / \eps^3)$ or the $\tO(\prod_{i = 1}^m A_i / \eps^2)$ of~\citet{liu2021sharp}, which we leave as future work.

% Given the state-of-art the sample complexity upper bound 

%\sm{If we move the lower bound to the appendix, we can comment the lower bound in one paragraph here. }

==> Sections/abstract.tex <==
\begin{abstract}
Multi-agent reinforcement learning has made substantial empirical progresses in solving games with a large number of players. However, theoretically, the best known sample complexity for finding a Nash equilibrium in general-sum games scales exponentially in the number of players due to the size of the joint action space, and there is a matching exponential lower bound.
This paper investigates what learning goals admit better sample complexities in the setting of $m$-player general-sum Markov games with $H$ steps, $S$ states, and $A_i$ actions per player. First, we design algorithms for learning an $\epsilon$-Coarse Correlated Equilibrium (CCE) in $\widetilde{\mathcal{O}}(H^5S\max_{i\le m} A_i / \epsilon^2)$ episodes, and an $\epsilon$-Correlated Equilibrium (CE) in $\widetilde{\mathcal{O}}(H^6S\max_{i\le m} A_i^2 / \epsilon^2)$ episodes. This is the first line of results for learning CCE and CE with sample complexities polynomial in $\max_{i\le m} A_i$. Our algorithm for learning CE integrates an adversarial bandit subroutine which minimizes a weighted swap regret, along with several novel designs in the outer loop. Second, we consider the important special case of Markov Potential Games, and design an algorithm that learns an $\epsilon$-approximate Nash equilibrium within $\widetilde{\mathcal{O}}(S\sum_{i\le m} A_i / \epsilon^3)$ episodes (when only highlighting the dependence on $S$, $A_i$, and $\epsilon$), which only depends linearly in $\sum_{i\le m} A_i$ and significantly improves over existing efficient algorithms in the $\epsilon$ dependence. Overall, our results shed light on what equilibria or structural assumptions on the game may enable sample-efficient learning with many players.
% ~\yub{shorten if needed}
\end{abstract}

% Such exponential dependence is also unavoidable in the worst case due to recently established sample complexity lower bounds.


% We complement this result with a new sample complexity lower bound for this problem that slightly improves in the $A_i$ dependency over naive reduction techniques. 


% Below is ICLR abstract ddl version
% Multi-agent reinforcement learning has made substantial empirical progresses in solving games with a large number of players. However, theoretically, the best known sample complexity for finding the Nash equilibrium in general-sum games scales exponentially in the number of players due to the size of the joint action space. Such exponential dependence is also unavoidable in the worst case due to recently established sample complexity lower bounds.

% This paper investigates when such exponential sample complexity can be improved in $m$-player general-sum Markov games with $H$ steps, $S$ states, and $A_i$ actions per player. First, we design an algorithm that finds the $\epsilon$-Coarse Correlated Equilibrium (CCE) in $\wt{O}({\rm poly}(H)S\max_{i\le m} A_i / \eps^2)$ episodes, which has a much milder dependence on $m$. Second, we consider the important special case of Markov Potential Games, and design an algorithm that learns a pure-strategy $\eps$-approximate Nash equilibrium within $\wt{O}(S\sum_{i=1}^m A_i / \eps^3)$ episodes (when only highlighting the dependence on $S$, $A_i$, and $\epsilon$), which only depends polynomially in $m$ and significantly improves over the best known algorithm in the $\eps$ dependence. We complement this result with a new sample complexity lower bound for this problem that slightly improves in the $A_i$ dependency over naive reduction techniques. 

% We tackle this problem by studying alternative solution concepts or additional structure assumptions on the game.

% 

% of $\Omega(\sum_{i=1}^m A_i / \eps^2)$

% for learning a pure-strategy $\eps$-approximate Nash equilibrium in Markov Potential Games. 

% Towards improving over such exponential dependence, 

% presents two new sample-efficient learning results for general-sum Markov Games. 


==> Sections/algorithm.tex <==
\section{Simplified version Algorithm 1 with theoretical guarantee}

If we consider a simplified version of algorithm \ref{algorithm:nash_v_adv}, i.e. the update rule is \begin{align*}
    \text{If } n\in\mathcal{L}, \text{ then } 
    \up{V}_h(s_h) \setto \frac{\check{v}}{\check{n}}+\bar{b},
\end{align*}
we can prove that this algorithm achieve regret bound $\mathcal{O}(H^5S(A+B)K)$.

\yub{switch to using V-OL algorithm of Tiancheng et al.?}


\begin{lemma} For each update time, the following inequality holds with high probability, where $\check{k}_i$ represent the index of the ith visit at s at the h-th step in this stage
\begin{align*}
    \max_\mu \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu\times\nu_h^{\check{k}_i}}\left(r_h + \mathbb{P}_h\up{V}_{h+1}^{\check{k}_i}\right)(s)&-
    \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \left[r_h\left(s,a_h^{\check{k}_i},b_h^{\check{k}_i}\right) + \up{V}_{h+1}^{\check{k}_i}\left(s_{h+1}^{\check{k}_i}\right)\right]\\
    &\le c\sqrt{\frac{2H^2 A\iota}{\check{n}}}.
\end{align*} 
\end{lemma}
\begin{proof-of-lemma}[1]
First, by Azuma-Hoeffding, 
\begin{align*}
    \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu_h^{\check{k}_i}\times\nu_h^{\check{k}_i}}\left(r_h + \mathbb{P}_h\up{V}_{h+1}^{\check{k}_i}\right)(s)&-
    \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \left[r_h\left(s,a_h^{\check{k}_i},b_h^{\check{k}_i}\right) + \up{V}_{h+1}^{\check{k}_i}\left(s_{h+1}^{\check{k}_i}\right)\right]\\
    &\le 2\sqrt{\frac{2H^2 \iota}{\check{n}}}.
\end{align*}
To bound $$R_{\check{n}}=\max_\mu \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu\times\nu_h^{\check{k}_i}}\left(r_h + \mathbb{P}_h\up{V}_{h+1}^{\check{k}_i}\right)(s)-\sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu_h^{\check{k}_i}\times\nu_h^{\check{k}_i}}\left(r_h + \mathbb{P}_h\up{V}_{h+1}^{\check{k}_i}\right)(s)
,$$ we use the bandit lemma in [\cite{}], then we have
\begin{align*}
    R_{\check{n}}/H&\le 2\frac{1}{\check{n}}\sqrt{A\check{n}\iota}+\frac{3\sqrt{A\iota}}{2}\sum_{i=1}^{\check{n}} \frac{1}{\check{n}\sqrt{i}}+\frac{1}{2}\frac{1}{\check{n}}\iota+\sqrt{2\iota\sum_{i=1}^{\check{n}} \frac{1}{\check{n}^2}}\\
    &=\mathcal{O}(\sqrt{\frac{A\iota}{\check{n}}}).
\end{align*}
Combining these two result together, we can get the desired result. Note that we can get a similar result for the min player.
\end{proof-of-lemma}
\begin{remark}
Every $\up{V}_h$ and $\underline{V}_h$ in this lemma should be considered as capped value (restricted in $[0,H-h+1]$).  
\end{remark}

\begin{lemma}
With high probability, the following two conclusions holds,
\begin{align*}
    \up{V}_h^k(s)\ge V_h^\star(s)\ge \underline{V}_h^k (s) \text{ for all } (s,h,k)\in\mathcal{S}\times[K]\times[H].
\end{align*}
\begin{align*}
    (1/K)\sum_{k=1}^K( \up{V}_h^k-\underline{V}_h^k )(s_1)\le \mathcal{O}(\sqrt{H^5S(A+B)\iota/K}).
\end{align*}
\end{lemma}
\begin{proof-of-lemma}[2]
The first claim can be proved by backward induction. First of all, we should always keep in mind that at each stage, $\up{V}_h^k(s), \underline{V}_h^k(s)$ is fixed. We only update them when a stage is over.  So at each stage, the value of  $\up{V}_h^k(s), \underline{V}_h^k(s)$ only depends on the last stage before this stage. The claim is true for $h=H+1$. Assume for any s, $\up{V}_{h+1}^k(s)\ge V_{h+1}^\star(s)\ge \underline{V}_{h+1}^k (s)$. For fixed $s$ and $k$, let $\check{n}$ be the number of s was visited at h-th step in last stage and the index of such time is $\check{k}_1,\dots,\check{k}_{\check{n}}$, By Bellman equation,
\begin{align*}
    V_h^\star(s)&=\max_\mu \min_\nu \mathbb{D}_{\mu\times\nu}\left(r_h + \mathbb{P}_h V_{h+1}^\star\right)(s)\\
    &=\max_\mu \sum_{i=1}^{\check{n}}\frac{1}{\check{n}}\min_\nu \mathbb{D}_{\mu\times\nu}\left(r_h + \mathbb{P}_h V_{h+1}^\star\right)(s)\\
    &\le \max_\mu \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu\times\nu_h^{\check{k}_i}}\left(r_h + \mathbb{P}_h V_{h+1}^\star\right)(s)\\
    &\le \max_\mu \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu\times\nu_h^{\check{k}_i}}\left(r_h + \mathbb{P}_h\up{V}_{h+1}^{\check{k}_i}\right)(s).
\end{align*}
Comparing with the last lemma, if we choose bonus $\up{\beta} = c\sqrt{H^2A\iota/\check{n}}$. We would have $\up{V}_h^k(s)\ge V_h^\star(s)$. Similarly, $\underline{\beta} = c\sqrt{H^2B\iota/\check{n}}$ gives $V_h^\star(s)\ge \underline{V}_h^k (s)$.

Finally, we are ready to prove the regret bound. Letting $\delta_h^k := \up{V}_h^k(s_h^k)-\underline{V}_h^k (s_h^k)$, $\check{n}_h^k$ be the number of $s_h^k$ was visited at h-th step in last stage and the index of such time is $\check{l}_h^1,\dots,\check{l}_h^{\check{n}_h^k}$ . $\check{n}_h^k=0$ if this is the first stage. By this algorithm, 
\begin{align*}
    \delta_h^k &= \up{V}_h^k(s_h^k)-\underline{V}_h^k (s_h^k)\\
    &= H\mathbf{1}_{\{\check{n}_h^k=0\}}+
    \sum_{i=1}^{\check{n}_h^k}\frac{1}{\check{n}_h^k}\paren{\up{V}_{h+1}^{\check{l}_h^i}(s_{h+1}^{\check{l}_h^i})-\underline{V}_{h+1}^{\check{l}_h^i}(s_{h+1}^{\check{l}_h^i})}+\up{\beta}_k-\underline{\beta}_k\\
    &\le H\mathbf{1}_{\{\check{n}_h^k=0\}}+
    \sum_{i=1}^{\check{n}_h^k}\frac{1}{\check{n}_h^k}\paren{\up{V}_{h+1}^{\check{l}_h^i}(s_{h+1}^{\check{l}_h^i})-\underline{V}_{h+1}^{\check{l}_h^i}(s_{h+1}^{\check{l}_h^i})}+ c\sqrt{\frac{H^2 (A+B)\iota }{\check{n}_h^k}}\mathbf{1}_{\{\check{n}_h^k>0\}}\\
    &=H\mathbf{1}_{\{\check{n}_h^k=0\}}+
    \sum_{i=1}^{\check{n}_h^k}\frac{1}{\check{n}_h^k}\delta_{h+1}^{\check{l}_h^i}+ c\sqrt{\frac{H^2 (A+B)\iota }{\check{n}_h^k}}\mathbf{1}_{\{\check{n}_h^k>0\}}.
\end{align*}

Taking the summation w.r.t. k, the first term is 
\begin{align*}
    \sum_{k=1}^K H\mathbf{1}_{\{\check{n}_h^k=0\}}\le HSe_1.
\end{align*}

The second term is 
\begin{align*}
    \sum_{k=1}^K \sum_{i=1}^{\check{n}_h^k}\frac{1}{\check{n}_h^k}\delta_{h+1}^{\check{l}_h^i}\le 
    \sum_{k=1}^K \delta_{h+1}^k(1+\frac{1}{H}).
\end{align*}
To get this inequality, we first exchange the order of summation, then we find that the coefficient of $\delta_{h+1}^k$ is contributed by the next stage's k. Because $e_{i+1}=\floor{(1+1/H)e_i}$, the coefficients are bounded by $1+\frac{1}{H}.$

The last term is 
\begin{align*}
    \sum_{k=1}^K c\sqrt{\frac{H^2 (A+B)\iota }{\check{n}_h^k}}\mathbf{1}_{\{\check{n}_h^k>0\}}
    &=c \sum_s\sum_{k:s_h^k = s}\sqrt{\frac{H^2 (A+B)\iota }{\check{n}_h^k}}\mathbf{1}_{\{\check{n}_h^k>0\}}\\
    &\le c(1+\frac{1}{H}) \sum_s \sum_{0<i<N_s^K}\sqrt{H^2(A+B)\iota e_i},
\end{align*}
where $N_s^K$ means till K, s is in its $N_s^K$-th stage at step h. When $N_s^K$ equal for all $s$, we attain maximum. So we can further derive
\begin{align*}
    \sum_{k=1}^K c\sqrt{\frac{H^2 (A+B)\iota }{\check{n}_h^k}}\mathbf{1}_{\{\check{n}_h^k>0\}}&\le
    \mathcal{O}(1)S\sum_{i=1}^{N}\sqrt{H^2(A+B)\iota e_i}\\&=\mathcal{O}(1)S\sqrt{H^2(A+B)\iota e_1}\frac{\sqrt{1+1/H}^N-1}{\sqrt{1+1/H}-1},
\end{align*}
where $$N \approx \frac{\log \paren{1+\frac{K}{SHe_1}}}{\log\paren{1+\frac{1}{H}}}.$$
After some calculation, we get
\begin{align*}
    \sum_{k=1}^K c\sqrt{\frac{H^2 (A+B)\iota }{\check{n}_h^k}}\mathbf{1}_{\{\check{n}_h^k>0\}}&\le \mathcal{O}(1)S\sqrt{H^2(A+B)\iota e_1}\mathcal{O}(H\sqrt{\frac{K}{SHe_1}})\\
    &=C\sqrt{H^3S(A+B)\iota K}
\end{align*}

So
\begin{align*}
    \sum_{k=1}^K \delta_h^k&\le HSe_1+(1+\frac{1}{H})\sum_{k=1}^K \delta_{h+1}^k+C\sqrt{H^3S(A+B)\iota K})\\
    &=SH^2+(1+\frac{1}{H})\sum_{k=1}^K \delta_{h+1}^k+C\sqrt{H^3S(A+B)\iota K}).
\end{align*}
If $K\to \infty$, this gives
$$
(1/K)\sum_{k=1}^K( \up{V}_h^k-\underline{V}_h^k )(s_1)\le \mathcal{O}(\sqrt{H^5S(A+B)\iota/K}).
$$
\end{proof-of-lemma}

We can define certified policies (Algorithm \ref{algorithm:certified policy})to extract a policy after playing. This policy can achieve sample complexity $\mathcal{O}(H^5S(A+B)/\epsilon^2)$ and the algorithm is model-free.

\begin{algorithm}[t]
% \setstretch{1.2}
   \caption{Certified policy}
   \label{algorithm:certified policy}
   \begin{algorithmic}[1]
      \STATE sample k $\setto$ Uniform([K]).
      \FOR{step $h=1,\dots,H$}
      \STATE observe $s_h$, and set $t\setto \check{n}_h^k(s_h)$.
      \STATE sample $m\in[t]$ with $\P(m=i) = 1/t$.
      \STATE $k\setto \check{l}_t^i(s_h)$.
      \STATE take action $a_h\sim \mu_h^k(\cdot|s_h)$.
      \ENDFOR
   \end{algorithmic}
\end{algorithm}

\section{Discussion on Sample Complexity Lower Bound of Finding Approximate Nash Equilibrium in General-Sum Markov Games}
In this section, we investigate the query complexity for computing Nash or approximate Nash in bimatrix games. 

\subsection{Sample complexity upper bound}

\subsection{Lower bound of query complexity in general-sum games}
\begin{theorem}
There exists a general sum Markov games M=\text{MG}$(H,\mc{S},\{\mc{A}_i\}_{i=1}^m,\mathbb{P},\{r_i\}_{i=1}^m)$ and two positive number $epsilon$ and c such that: for any algorithm, after $2^{\Omega(m/\log m)}$ episodes, with probability at least $p=1-2^{-cm/\log m}$, the algorithm failed to output a $\epsilon$-Nash equilibrium.
\end{theorem}
\yub{Cite Rubinstein 16 and Cheng Yu et al. 15}.

\begin{lemma}
There exists two constant $\epsilon>0$ and $c>0$ such that:

$$
\text{QC}_p(\text{ANE}(m,\epsilon))=2^{\Omega(m/\log m)}, \text{ where } p=2^{-cm/\log m}.
$$
\end{lemma}
Even in this case, with $m$ players, and $A_i=2$, with noiseless payoff query, there is still $2^{\Omega(m)}$ query complexity lower bound for finding $\epsilon$-Nash with $\epsilon$ being some small constant. 

\section{Approximate CCE for General Sum Markov Games}
In this section, we present an algorithm which can find CCE for general sum Markov games in $\tilde O(H^5 S \sum_{i=1}^m A_i /\epsilon^2)$ episodes.
\begin{algorithm}[t]
% \setstretch{1.2}
   \caption{Nash-V-Learning for the i-th player}
   \label{algorithm:nash_v_general}
   \begin{algorithmic}[1]
      \STATE {\bfseries Initialize:} For any $(s, a, h)$, set $\up{V}_{h,i}(s)\setto H$, $\underline{V}_{h,i}(s)\setto 0$, $\up{L}_{h,i}\setto 0$, $\mu_h(a|s) \setto 1/A_i$, $N_h(s)\setto 0$.
      \FOR{episode $k=1,\dots,K$}
      \STATE Receive $s_1$.
      \FOR{step $h=1,\dots, H$}
      \STATE Take action $a_h \sim \mu_h(\cdot |s_h)$, observe the action $a'_h$ from the other players.
      \STATE Observe reward $r_h=r_h(s_h, a_h, a'_h)$ and next state $s_{h+1}$ from the environment.
      \STATE Update accumulators: $t\defeq N_{h}(s_h)\setto N_{h}(s_h) + 1$.
      \STATE $\up{V}_{h,i}\left(s_{h}\right) \setto  \left(1-\alpha_{t}\right) \bar{V}_{h,i}\left(s_{h}\right)+\alpha_{t}\left(r_{h,i}\left(s_{h}, a_{h}, a'_{h}\right)+\bar{V}_{h+1,i}\left(s_{h+1}\right)+\bar{\beta}_{t}\right)$
      \STATE $\underline{V}_{h,i}\left(s_{h}\right) \setto  \left(1-\alpha_{t}\right) \underline{V}_{h,i}\left(s_{h}\right)+\alpha_{t}\left(r_{h,i}\left(s_{h}, a_{h}, a'_{h}\right)+\underline{V}_{h+1,i}\left(s_{h+1}\right)-\bar{\beta}_{t}\right)$
      \FOR{all $a \in \mc{A}_i$}
      \STATE $\up{\ell}_{h,i}(s_h, a) \setto [H - r_{h,i}-\min\{\up{V}_{h+1,i}(s_{h+1}),H-h\}] \mathbb{I}\{a_h=a\}/[\mu_h(a_h|s_{h}) +\up{\eta}_{t}]$.
      \STATE $\up{L}_{h,i}(s_h,a)\setto (1-\alpha_t)\up{L_{h,i}}(s_h,a)+\alpha_t\up{L}_{h,i}(s_h,a)$
      % \STATE $\up{L}_h( s_h, a)  \setto ( 1-\alpha _t )\up{L}_h( s_h,a ) +\alpha_t \up{\ell}_h(s_h, a)$.
      \ENDFOR
      \STATE Set $\mu_h(\cdot |s_h) \propto \exp[-(\up{\eta}_t/\alpha_t) \up{L}_{h,i}( s_h, \cdot)]$.
      \ENDFOR
      \ENDFOR
   \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
% \setstretch{1.2}
   \caption{Certified policy $\hat\pi$ for general-sum Markov games}
   \label{certified_policy_general}
   \begin{algorithmic}[1]
      \STATE sample $k$ $\setto$ Uniform([K]).
      \FOR{step $h=1,\dots,H$}
      \STATE observe $s_h$, and set $t\setto N_h^k(s_h)$.
      \STATE sample $l\in[t]$ with $\P(l=j) = \alpha_t^j$.
      \STATE $k\setto k_t^l(s_h)$.
      \STATE jointly take action $(a_{h,1}, a_{h,2},\dots,a_{h,m})\sim \prod_{i=1}^m\mu_{h,i}^k(\cdot|s_h)$.
      \ENDFOR
   \end{algorithmic}
\end{algorithm}

We choose all hyperparameters as follows, for some large constant $c$, and log factors $\iota$.
\begin{align*}
    \alpha_{t}=\frac{H+1}{H+t}, \quad \eta_{t}=\sqrt{\frac{H\log A_i}{A_i t}}, \quad \bar{\beta}_{t}=c \sqrt{\frac{H^{3} A_i \iota}{t}}.
\end{align*}
Value function of certified policy can be decomposed as 
$$
V^{\hat\pi}_{1,i}(s) = \frac{1}{K}\sum_{k=1}^K V^{\hat\pi^k}_{1,i}(s),
$$
where the decomposition is due to the first line in the algorithm: sample $k\setto $Uniform([K]).

After running  Algorithm \ref{algorithm:nash_v_general} for all $m$ players and Algorithm \ref{certified_policy_general}, we can learn a certified policy $\hat\pi$. Then,
\begin{theorem}\label{proof_general_cce}
With probability at least $1-p$, if we run Algorithm \ref{algorithm:nash_v_general} for all $m$ players and Algorithm \ref{certified_policy_general} for $K$ episodes with 
$$
K\ge \Omega(H^5 S \max_{i\in[m]}A_i \iota /\epsilon^2),
$$
then the certified policy $\hat\pi$ will be $\epsilon$-approximate CCE, i.e. $V_{1,i}^{\dagger,\hat\pi_{-i}}(s)- V_{1,i}^{\hat\pi} (s)\le \epsilon$ for all $i=1,2,\dots,m$ and $s\in \mc{S}$.
\end{theorem}

Before proving Theorem \ref{proof_general_cce}, there's a simple consequence of the update rule in Algorithm \ref{algorithm:nash_v_general}, which will be used several times later. To simplify the notation, we omit index $i$ which represent the i-th player.
\begin{lemma}
Let $t=N_h^k(s)$ and suppose s was previously visited at episodes $k^1,\dots,k^t<k$ at the h-th step. The update rule in Algorithm \ref{algorithm:nash_v_general} is equivalent to the following equations.
\begin{align}
    \up{V}_{h}^{k}(s)&=\alpha_{t}^{0} H+\sum_{j=1}^{t} \alpha_{t}^{j}\left[r_{h}\left(s, a_{h}^{k^{j}}, {a'}_{h}^{k^{j}}\right)+\up{V}_{h+1}^{k^{j}}\left(s_{h+1}^{k^{j}}\right)+\bar{\beta}_{j}\right]\\
    \underline{V}_{h}^{k}(s)&=\sum_{j=1}^{t} \alpha_{t}^{j}\left[r_{h}\left(s, a_{h}^{k_{h}^{j}}, {a'}_{h}^{k_{h}^{j}}\right)+\underline{V}_{h+1}^{k_{h}^{j}}\left(s_{h+1}^{k_{h}^{j}}\right)-\up{\beta}_{j}\right]
\end{align}
\end{lemma}

\begin{lemma}
\label{bandit_lemma_general}
Let $t=N_h^k(s)$ and suppose s was previously visited at episodes $k^1,\dots,k^t<k$ at the h-th step. With probability $1-\frac{p}{2m}$, for any $(s,h,t)\in\mc{S}\times[H]\times[K]$, there exist a constant c s.t.

\begin{gather*}
    \max _{\mu} \sum_{j=1}^{t} \alpha_{t}^{j} \mathbb{D}_{\mu \times \mu_{h,-i}^{k^{j}}}\left(r_{h}+\mathbb{P}_{h} \min\{\up{V}_{h+1,i}(s_{h+1}),H-h\}\right)(s)\\-\sum_{j=1}^{t} \alpha_{t}^{j}\left[r_{h}\left(s, a_{h}^{k^{j}}, b_{h}^{k^{j}}\right)+\min\{\up{V}_{h+1,i}(s_{h+1}),H-h\}\left(s_{h+1}^{k^{i}}\right)\right] \leq c \sqrt{2 H^{3} A \iota / t}
\end{gather*}

\end{lemma}
\begin{proof-of-lemma}[\ref{bandit_lemma_general}]
The proof consists of two parts, the first one is applying Azuma-Hoeffding inequality and another is (\red{slight stronger}) adversarial bandit lemma.
\end{proof-of-lemma}
\begin{remark}
The inequality in Lemma \ref{bandit_lemma_general} holds with probability $1-p/2m$. Take a union bound, we can conclude that the inequality holds for all the player with probability $1-p/2$.
\end{remark}

\begin{lemma}
\label{key-lemma-general}
If the inequality in Lemma \ref{bandit_lemma_general} holds for all m players, then we have
\begin{align*}
    \up{V}_{h,i}^k(s)\ge V_{h,i}^{\dagger,\hat\pi_{-i}^k}(s),\quad
    \underline{V}_{h,i}^k(s)\le V_{h,i}^{\hat\pi^k}(s)
\end{align*}
for all $[k,h,s]\in [K]\times[H]\times\mc{S}$ with probability at least $1-p/2$.
\end{lemma}
\begin{proof-of-lemma}[\ref{key-lemma-general}]
We proof the first claim by backward induction. The claim is true for $h = H + 1$. Suppose the claim is true for $h+1$.
We begin with $V_{h,i}^{\dagger,\hat\pi_{-i}^k}(s)$, by the definition of certified policy, letting $t = N_h^k(s)$, we have
\begin{align*}
    V_{h,i}^{\dagger,\hat\pi_{-i}^k}(s) &= \sup_{\mu_i}\mathbb{D}_{\mu_i\times\hat\pi_{-i}^k} [r_{h,i}+\mathbb{P}_h V_{h+1,i}^{\dagger,\hat\pi_{-i}^k}](s)\\
    &=\sup_{\mu_i}\sum_{j=1}^t \alpha_t^j \mathbb{D}_{\mu_i\times\mu_{h,-i}^{k^j}}[r_{h,i}+\mathbb{P}_h V_{h+1,i}^{\dagger,\hat\pi_{-i}^k}](s)\\
    &\le \sup_{\mu_i}\sum_{j=1}^t \alpha_t^j \mathbb{D}_{\mu_i\times\mu_{h,-i}^{k^j}}[r_{h,i}+\mathbb{P}_h \min\{\up{V}_{h+1,i}(s_{h+1}),H-h\}](s)\\
    &\le\sum_{j=1}^{t} \alpha_{t}^{j}\left[r_{h}\left(s, a_{h}^{k^{j}}, b_{h}^{k^{j}}\right)+\min\{\up{V}_{h+1,i}(s_{h+1}),H-h\}\left(s_{h+1}^{k^{i}}\right)\right] + c \sqrt{2 H^{3} A \iota / t}\\
    &\le \sum_{j=1}^{t} \alpha_{t}^{j}\left[r_{h}\left(s, a_{h}^{k^{j}}, b_{h}^{k^{j}}\right)+\min\{\up{V}_{h+1,i}(s_{h+1}),H-h\}\left(s_{h+1}^{k^{i}}\right)+\up{\beta}_j\right]\\
    &= \up{V}_{h,i}^k(s).
\end{align*}
Here, the first inequality is due to induction hypothesis and bounded value function. For the last inequality, we use $\frac{1}{\sqrt{t}} \leq \sum_{i=1}^{t} \frac{\alpha_{t}^{i}}{\sqrt{i}} \leq \frac{2}{\sqrt{t}}$. So if we choose $\up{\beta}_t = c\sqrt{\frac{H^3 A_i \iota}{t}}$ for large $c$, the inequality holds. 
Meanwhile, by the definition of certified policy, 
\begin{align*}
    V_{h,i}^{\hat\pi^k}(s) &= \sum_{j=1}^t \alpha_t^j \mathbb{D}_{\pi^{k^j}}[r_h+\mathbb{P}_h V_{h+1,i}^{\hat\pi^{k^j}}](s)\\
    &\ge \sum_{j=1}^t \alpha_t^j \mathbb{D}_{\pi^{k^j}}[r_h+\mathbb{P}_h \underline{V}^{k^j}_{h+1,i}](s).
\end{align*}
So by Azuma-Hoeffding inequality, with probability at least $1-\frac{p}{2SKH}$
\begin{align*}
    \sum_{j=1}^t \alpha_t^j \mathbb{D}_{\pi^{k^j}}[r_h+\mathbb{P}_h \underline{V}^{k^j}_{h+1,i}](s)&\ge \sum_{j=1}^{t} \alpha_{t}^{j}\left[r_{h}\left(s, a_{h}^{k_{h}^{j}}, {a'}_{h}^{k_{h}^{j}}\right)+\underline{V}_{h+1}^{k_{h}^{j}}\left(s_{h+1}^{k_{h}^{j}}\right)\right] -\sqrt{\frac{H^3 A_i\iota}{t}}\\
    &\ge\sum_{j=1}^{t} \alpha_{t}^{j}\left[r_{h}\left(s, a_{h}^{k_{h}^{j}}, {a'}_{h}^{k_{h}^{j}}\right)+\underline{V}_{h+1}^{k_{h}^{j}}\left(s_{h+1}^{k_{h}^{j}}\right)-\up{\beta}_{j}\right]\\
    & = \underline{V}^{k^j}_{h,i}(s).
\end{align*}
Taking a union bound, then Lemma \ref{key-lemma-general} is proved by induction.
\end{proof-of-lemma}

Equipped with these lemmas, we are ready to prove Theorem \ref{proof_general_cce}. 

\begin{proof-of-theorem}[\ref{proof_general_cce}]
Suppose Lemma \ref{bandit_lemma_general} and Lemma \ref{key-lemma-general} all hold (this happens with probability at least $1-p$), then 
\begin{align*}
    V_{1,i}^{\dagger,\hat\pi^k_{-i}}(s_1)- V_{1,i}^{\hat\pi^k} (s_1)\le \up{V}_{1,i}^k(s_1)-\underline{V}_{1,i}^k(s_1).
\end{align*}
So we have
\begin{align*}
     V_{1,i}^{\dagger,\hat\pi_{-i}}(s_1)- V_{1,i}^{\hat\pi} (s_1)
     \le&\frac{1}{K} \sum_{k=1}^K\left( V_{1,i}^{\dagger,\hat\pi^k_{-i}}(s_1)- V_{1,i}^{\hat\pi^k} (s_1)\right)\\
     \le& \frac{1}{K} \sum_{k=1}^K\left(\up{V}_{1,i}^k(s_1)-\underline{V}_{1,i}^k(s_1)\right) .
\end{align*}

Letting $\delta_{h,i}^k := \up{V}_{h,i}^k(s_h^k)-\underline{V}_{h,i}^k (s_h^k)$ and $t=N_h^k(s)$. By the update rule, 
\begin{align*}
    \delta_{h,i}^k &= \up{V}_{h,i}^k(s_h^k)-\underline{V}_{h,i}^k (s_h^k)\\
    &= \alpha^0_t H + \sum_{j=1}^t \alpha_t^j [\up{V}_{h+1,i}^k(s_{h+1}^{k^j})-\underline{V}_{h+1,i}^k(s_{h+1}^{k^j})+2\up{\beta_j}]\\
    &= \alpha_t^0H +\sum_{j=1}^t\alpha_t^j \delta_{h+1,i}^{k^j}+\sum_{j=1}^t 2\alpha_t^j\up{\beta}_j\\
    &\le \alpha_t^0H +\sum_{j=1}^t\alpha_t^j \delta_{h+1,i}^{k^j}+ 2c\sqrt{\frac{A_iH^3\iota}{t}}
\end{align*}

Taking the summation w.r.t. k, by the same argument in Nash V learning, we can get 
\begin{align*}
    &\frac{1}{K} \sum_{k=1}^K\left(\up{V}_{1,i}^k(s_1)-\underline{V}_{1,i}^k(s_1)\right) =\frac{1}{K} \sum_{k=1}^K \delta_{h,i}^k\\
    \le& eSH^2/K+ \mathcal{O}\left(\sqrt{H^{5} S\max_{i\in[m]} A_i \iota/K}\right).
\end{align*}
This complete the proof of Theorem \ref{proof_general_cce} because when $K\to\infty$, $\sqrt{H^{5} S\max_{i\in[m]} A_i \iota/K}$ is the dominant term.
\end{proof-of-theorem}


% \section{Difficulties in Finding Approximate Nash Equilibrium in General-Sum Markov Games}
% \subsection{Query complexity with noiseless payoff query}



% \subsection{Computation complexity}
% \subsection{No-regret learning}
% \subsection{Sub-linear regret and last iteration convergence}

\section{Efficient Algorithm to Compute pure $\epsilon$ Nash in Markov Potential Games}
%With the setting in [Li Na's <Gradient Play...>]. For softmax parameterization:
% \begin{align*}
%     \pi_{i,\theta_i}(a_i|s)=\frac{\exp \theta_{s,a_i}}{\sum_{a_j\in\mc{A}_i}\exp \theta_{s,a_j}}.
% \end{align*}
% Since this is a differentiable parameterization that explicitly constrains $\pi_\theta(\cdot|s)$ to be in the simplex, then we have
% \begin{align*}
%     \nabla_{\theta} \mathbb{E}_{s_{0} \sim \rho} V_{i}^{\theta}\left(s_{0}\right)=\frac{1}{1-\gamma} \mathbb{E}_{s \sim d_{\theta}} \mathbb{E}_{a \sim \pi_{\theta}(\cdot | s)}\left[\nabla_{\theta} \log \pi_{\theta}(a \mid s) A_{i}^{\theta}(s, a)\right], \quad i=1,2, \ldots, n.
% \end{align*}
% Moreover, we have
% \begin{align*}
%     \frac{\partial \log \pi_{\theta}\left(a^{\prime} | s^{\prime}\right)}{\partial \theta_{s, a_{i}}}=\frac{\partial \log \pi_{\theta_{i}}\left(a_{i}^{\prime} | s^{\prime}\right)}{\partial \theta_{s, a_{i}}} &=\textbf{1}\left\{ s^{\prime}=s\right\} \paren{\textbf{1}\{a'=a\}-\pi_{\theta_i}(a_i|s)}\\
% &=\textbf{1}\left\{a_{i}^{\prime}=a_{i}, s^{\prime}=s\right\} -\textbf{1}\{s'=s\}\pi_{\theta_i}(a_i|s).
% \end{align*}
% So we can prove that
% \begin{lemma}
% $$\frac{\partial J_i(\theta)}{\partial \theta_{s,a_i}} =\frac{1}{1-\gamma} d_\theta(s)\pi_{\theta_i}(a_i|s) \up{A_i^\theta}(s,a_i). $$
% Moreover, if this is a Markov Potential Game(MPG) with potential function $\Phi$, then
% $$
% \frac{\partial \Phi (\theta)}{\partial \theta_{s,a_i}}=\frac{\partial J_i(\theta)}{\partial \theta_{s,a_i}} =\frac{1}{1-\gamma} d_\theta(s)\pi_{\theta_i}(a_i|s) \up{A_i^\theta}(s,a_i). 
% $$
% \end{lemma}
% Another important lemma is the \textbf{Performance difference lemma}:
% \begin{align*}
%     J_{i}\left(\theta^{\prime}\right)-J_{i}(\theta)=\frac{1}{1-\gamma} \mathbb{E}_{s \sim d_{\theta^{\prime}}} \mathbb{E}_{a \sim \pi_{\theta^{\prime}}} A_{i}^{\theta}(s, a), \quad i=1,2, \ldots, n.
% \end{align*}

% The NPG algorithm defines a Fisher information matrix
% (induced by $\pi$), and performs gradient updates in the geometry induced by this matrix as follows:
% \begin{align*}
%     \begin{array}{l}
% F_{\rho}(\theta)=\mathbb{E}_{s \sim d_\theta(\cdot)} \mathbb{E}_{a \sim \pi_{\theta}(\cdot| s)}\left[\nabla_{\theta} \log \pi_{\theta}(a | s)\left(\nabla_{\theta} \log \pi_{\theta}(a | s)\right)^{\top}\right] \\
% \theta^{(t+1)}=\theta^{(t)}+\eta F_{\rho}\left(\theta^{(t)}\right)^{\dagger} \nabla_{\theta} \Phi(\theta^{(t)}).
% \end{array}
% \end{align*}

% In multi-player case, this update rule doesn't have a convenient form.(?)

% Alternatively, we can consider another update rule. In each step, we perform NPG update for each single player (fix other players' policy) simultaneously ,i.e.
% \begin{align*}
%     \pi_i^{(t+1)}(a_i | s)=\pi_i^{(t)}(a_i | s) \frac{\exp \left(\eta \up{A_i^{\theta^{(t)}}}(s, a_i) /(1-\gamma)\right)}{Z_{i,t}(s)}, \quad i=1,2, \ldots, n.
% \end{align*}
% By performance difference lemma, 
% $$
% J_{i}\left(\theta_{i}^{\prime}, \theta_{-i}\right)-J_{i}\left(\theta_{i}, \theta_{-i}\right)=\frac{1}{1-\gamma} \sum_{s, a_{i}} d_{\theta^{\prime}}(s) \pi_{\theta_{i}^{\prime}}\left(a_{i} \mid s\right) \overline{A_{i}^{\theta}}\left(s, a_{i}\right),
% $$
% it's not difficult to get
% $$
% J_i(\theta_i^{(t+1)},\theta_{-i}^{(t)})-
% J_i(\theta_i^{(t)},\theta_{-i}^{(t)})\ge
% \frac{1-\gamma}{\eta}\mathbb{E}_{s_0\sim\rho}\log Z_{i,t}(s_0)\ge 0.
% $$
% By the definition of MPG, this becomes
% $$
% \Phi(\theta_i^{(t+1)},\theta_{-i}^{(t)})-
% \Phi(\theta_i^{(t)},\theta_{-i}^{(t)})\ge
% \frac{1-\gamma}{\eta}\mathbb{E}_{s_0\sim\rho}\log Z_{i,t}(s_0)\ge 0
% $$

% If we update each player's policy sequentially, we can get a coordinate ascent algorithm for $\Phi$.
% By performance difference lemma, 
% \begin{align*}
%   J_{i}\left(\theta_{i}^*, \theta_{-i}\right)-J_{i}\left(\theta_{i}, \theta_{-i}\right)
%   &=\frac{1}{1-\gamma} \sum_{s, a_{i}} d_{\theta^*}(s) \pi_{\theta_{i}^*}\left(a_{i} \mid s\right) \overline{A_{i}^{\theta}}\left(s, a_{i}\right) 
% \end{align*}

\yub{For the definition, we only need $V_1$. By the example we have seen (cite), this is much weaker than per-step, per-state potential game assumption.}


%\subsection{Algorithm with iteration complexity $\frac{Cn(\Phi_{\text{max}}-\Phi_{\text{min}})}{(1-\gamma)^2\epsilon^2}$}

\begin{algorithm}[t]
% \setstretch{1.2}
   \caption{Best response for general-sum Markov potential games}
   \label{algorithm:BR_general}
   \begin{algorithmic}[1]
   \REQUIRE Error tolerance $\epsilon$
      \WHILE{true}
      \STATE $\Delta,j,\{\hat\pi_j(\cdot|s)\}_{s\in\mc{S}}=$ \textbf{Estimate\_NE-Gap($\pi,\epsilon/8 $)}
      \IF{$\Delta>\epsilon/2$}
      \STATE update $\pi_j(\cdot|s)\setto \hat\pi_j(\cdot|s)$ for all $s\in\mc{S}$
      \ELSE 
      \STATE output $\pi$
      \STATE break
      \ENDIF
      \ENDWHILE
   \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
% \setstretch{1.2}
   \caption{Estimate\_NE-Gap($\pi,\delta$)}
   \label{algorithm:NEgap}
   \begin{algorithmic}[1]
      \FOR{player $i=1,\dots,n$}
      \STATE fix $\pi_{-i}$, run UCBVI-UPLOW   for i-th player with $K=\mc{O}(\frac{H^3SA_i\iota}{\delta^2})$ times and get a new policy $\hat\pi_i$
      \STATE Simulate the MDP with policy $\hat{\pi}_i,\pi_{-i}$ for $N=\frac{CH^2\iota}{\delta^2}$ times and get $\hat V_{1,i}(\hat\pi_i,\pi_{-i})$, which is an unbiased estimator of $V_{1,i}((\hat\pi_i,\pi_{-i}))$
      \STATE then we get $\Delta_i=\hat V_{1,i}(\hat\pi_i,\pi_{-i})-\hat V_{1,i}(\pi)$
      \ENDFOR
      \STATE $j\setto \arg\max_{i\in[n]} {\Delta_i}$
      \RETURN $\Delta_j,j,\hat\pi_j$
   \end{algorithmic}
\end{algorithm}
%\paragraph{Analysis:}
%For Algorithm \ref{NPG_general}, each time we update the policy, we have
%$$
%\Phi(\hat\pi_i,\pi_{-i})-\Phi(\pi) = J_i(\hat\pi_i,\pi_{-i})-J_i(\pi)\ge \epsilon/2 .
%$$
%So there are at most $2(\Phi_{\text{max}}-\Phi_{\text{min}})/\epsilon$ times update. On the other hand, if $\Delta\le\epsilon/2$, we have for all $i\in[n]$,
%\begin{align*}
%    J_i(\pi_i^*,\pi_{-i})-J_i(\pi)&=J_i(\pi_i^*,\pi_{-i})-J_i(\hat\pi_i,\pi_{-i})+J_i(\hat\pi_i,\pi_{-i})-J_i(\pi)\\
%    &\le \epsilon/2+\epsilon/2 .
%\end{align*}
%The inequality follows from the convergence rate of NPG and $\Delta\le\epsilon/2$.

%Overall, we need $\frac{2n(\Phi_{\text{max}}-\Phi_{\text{min}})}{\epsilon}$ times NPG, each NPG iterate $T=\frac{4}{(1-\gamma)^2\epsilon}$ times.

%\paragraph{Sample complexity:} While NPG update in subroutine gives a low iteration complexity, we can replace NPG with any other algorithm.

\subsection{Sample Complexity}
The overall sample complexity would be
$$
\mc{O}\paren{\frac{(\Phi_\text{max}-\Phi_\text{min})H^3S\sum_{i=1}^m A_i}{\epsilon^3}}. 
$$
Moreover, this algorithm is computation efficient. 

\yub{In this algorithm, use UCBVI-UPLOW to output a pure strategy. But mention that any efficient RL algorithm also works in principle, we only use this because it gives a pure strategy with high probability.}

\begin{theorem}\label{theorem:sample_complexity_general-sum}
For any $p\in(0,1]$, letting $\iota = \log(\frac{S\max_{1\le i\le m} A_i m}{\epsilon p})$, then with probability at least $1-p$, after at most 
$$
\mc{O}(\frac{(\Phi_\text{max}-\Phi_\text{min})H^3S\sum_{i=1}^m A_i \iota}{\epsilon^3})
$$
episodes, Algorithm \ref{BR_general} outputs a $\epsilon$-Nash pure policy $\hat\pi$.
\end{theorem}

\begin{lemma}
\label{lemma:NEgap}
For Algorithm \ref{NEgap}, with $\iota=\log(\frac{S\max_{1\le i\le m} A_i m}{\epsilon p})$, the output $\Delta_j,j,\hat\pi_j$ satisfied
$$
|V_{1,j}(\hat\pi_j,\pi_{-j})-V_{1,j}(\pi)- \Delta_j|\le2\delta, \quad
\max_{\pi_j}V_{1,j}(\pi_j,\pi_{-j})-V_{1,j}(\hat\pi_j,\pi_{-j})\le \delta
$$
with probability at least $1-\frac{p\epsilon}{4m}$.
\end{lemma}
\begin{proof-of-lemma}[\ref{lemma_NEgap}]
For the execution of UCBVI-UPLOW, it return a $\delta$-optimal pure policy with probability at least $1-\frac{p\epsilon}{8m^2}$. For the unbiased estimator $\hat V_{1,j}$, it's bounded by $H$. Thus by Hoeffding inequality,
$$
\mathbb{P}(|\hat V_{1,j}-V_{1,j}|\ge \delta)\le2\exp(-\frac{c\delta^2}{H^2 N}) 
$$
for some absolute constant $c$. For $N=CH^2/\delta^2\iota$ for some large constant $C$, we have
$$
|\hat V_{1,j}-V_{1,j}|\le \delta \quad \text{with probability at least }\quad 1-\frac{p\epsilon}{16m^2}.
$$
As a result, with probability at least $1-\frac{p\epsilon}{4m}$, for any $i\in[m]$,
\begin{equation}\label{equation:NE-gap_acuracy}
 \begin{gathered}
\max_{\pi_j}V_{1,j}(\pi_j,\pi_{-j})-V_{1,j}(\hat\pi_j,\pi_{-j})\le \delta\\
|\hat V_{1,j}(\hat\pi_j,\pi_{-j})-V_{1,j}(\hat\pi_j,\pi_{-j})|\le \delta\\
|\hat V_{1,j}(\pi)-V_{1,j}(\pi_j)|\le \delta.
\end{gathered}   
\end{equation}

By definition, $\Delta_j=\hat V_{1,j}(\hat\pi_j,\pi_{-j})-\hat V_{1,j}(\pi)$, so we must have
$$
|V_{1,j}(\hat\pi_j,\pi_{-j})-V_{1,j}(\pi)- \Delta_j|\le2\delta, \quad
\max_{\pi_j}V_{1,j}(\pi_j,\pi_{-j})-V_{1,j}(\hat\pi_j,\pi_{-j})\le \delta.
$$
This finishes the proof of this lemma.
\end{proof-of-lemma}
\begin{proof-of-theorem}[\ref{sample_complexity_general-sum}] 
First, we would prove that Estimate\_NE-Gap would be called for at most $\frac{4(\Phi_\text{max}-\Phi_\text{min})}{\epsilon}$ times. Suppose Lemma \ref{lemma_NEgap} holds for the first $4m/\epsilon$ calls. By Lemma \ref{lemma_NEgap}, this is true with probability at least $1-p$. When $\Delta_j>\epsilon/2$, by the definition of MPG
\begin{align*}
    \Phi(\hat\pi_j,\pi_{-j})-\Phi(\pi) &= V_{1,j}(\hat\pi_j,\pi_{-j})-V_{1,j}(\pi)\\
    &\ge \Delta_j-2\epsilon/8\\
    &\ge \epsilon/4.
\end{align*}
Note that $\frac{4(\Phi_\text{max}-\Phi_\text{min})}{\epsilon}\le \frac{4m}{\epsilon}$. This means there are at most $\frac{4(\Phi_\text{max}-\Phi_\text{min})}{\epsilon}$ calls for  Estimate\_NE-Gap with probability $1-p$. After that, algorithm would stop. When the algorithm stops, by \ref{equation:NE-gap_acuracy}, for any $i\in[m]$
\begin{align*}
\max_{\pi_i}V_{1,i}(\pi_i,\pi_{-i})-V_{1,i}(\pi)&=\max_{\pi_j}V_{1,i}(\pi_i,\pi_{-i})-V_{1,i}(\hat\pi_i,\pi_{-i})+V_{1,i}(\hat\pi_i,\pi_{-i})-V_{1,i}(\pi)\\
&\le \delta + V_{1,i}(\hat\pi_i,\pi_{-i})-V_{1,i}(\pi)\\
&\le \delta +2\delta+\Delta_j\\
&\le \epsilon.
\end{align*}
So Algorithm \ref{BR_general} outputs an $\epsilon$-Nash. Moreover, because UCBVI-UPLOW outputs a pure policy, the output of Algorithm \ref{BR_general} would also be a pure policy.

The sample complexity of Algorithm \ref{NEgap} is $\mc{O}(H^3S\sum A_i\iota/\epsilon^2+H^2m\iota/\epsilon^2)=\mc{O}(H^3S\sum A_i\iota/\epsilon^2)$. So the overall sample complexity is at most $\mc{O}(\frac{(\Phi_\text{max}-\Phi_\text{min})H^3S\sum_{i=1}^m A_i \iota}{\epsilon^3}).$ 



\end{proof-of-theorem}


\section{Lower bound of sample complexity for finding \red{pure} $\epsilon$-Nash Equilibrium}
$\mc{O}\paren{\frac{\sum_{i=1}^m A_i}{\epsilon^2}}$ for matrix games

$\mc{O}\paren{\frac{H^3 S \sum_{i=1}^m A_i}{\epsilon^2}}$ for MDP?
\subsection{General-sum stochastic matrix games}

\begin{theorem}\label{theorem:matrix_game_lowerbound}
Suppose $A_i\ge 2$, $i=1,\dots,m$ . Then, there exists an absolute constant $c_0$ such that for any $\epsilon\le\frac{1}{2m}$ and any online finetuning algorithm that outputs a \textbf{pure} strategy $\hat\pi=(\hat\pi_1,\dots,\hat\pi_m)$, if the number of samples 
$$n\le c_0 \frac{\sum_{i=1}^m A_i}{\epsilon^2},$$
then there exists a problem instance $M$ with stochastic payoff on which the algorithm suffers from $\epsilon/5$-suboptimality
$$
\mathbb{E}_M \text{NE-Gap}(\hat\pi)=\mathbb{E}_M\max_i\left[\max_{\pi_i}u_i^{(\pi_i,\hat\pi_{-i})}-u_i^{\hat\pi}\right]\ge\epsilon/5,
$$
where the expectation $\mathbb{E}_M$ is w.r.t. the randomness during the algorithm execution within game M.
\end{theorem}

We consider the following family of Bernoulli matrix games: : Let $\bm{a}=(a_1,a_2,\dots,a_m)$.
\begin{gather*}
  \mathfrak{M}(\epsilon)=\{\mc{M}^{\bm{a}^\star}\in\mathbb{R}^{A_1\times A_2\times\cdots\times A_m} \text{ with }\\ \mc{M}^{\bm{a}^\star}_{\bm{a}}=\frac{1}{2}+(\bm{1}\set{a_1^\star=a_1}+\cdot\bm{1}\set{a_1^\star=a_1\&a_2^\star=a_2}+\cdots+
  \bm{1}\set{a_1^\star=a_1\&a_2^\star=a_2\&\cdots\&a_m^\star=a_m})\epsilon:\\
  \bm{a}^\star\in [A_1]\times\cdots\times[A_m]
  \},  
\end{gather*}
where in matrix game $\mc{M}^{\bm{a}^\star}$, the reward is sampled from $\text{Bernoulli}(\mc{M}^{\bm{a}^\star}_{\bm{a}})$ if the i-th player picks $a_i$ where $\bm{a}=(a_1,a_2,\dots,a_m).$ Moreover, we define $\mc{M}^0$ as a game in  $\mathfrak{M}(0)$. Here, we assume the action space of the i-th player is $[A_i]=\{1,2,\cdots,A_i\}.$

We further let $\nu$ denote the uniform distribution on $[A_1]\times\cdots\times[A_m]$. 

\begin{proof-of-theorem}[\ref{theorem:matrix_game_lowerbound}]
Fix a matrix game $\mc{M}^{\bm{a}^\star}\in \mathfrak{M}(\epsilon)$, it's clear that the only Nash (pure) strategy is $\bm{a}^\star=(a_1^\star,a_2^\star,\cdots,a_m^\star)$. In other words, the i-th player's action should be $a_i^\star$. For any online finetuning algorithm $\mc{A}$ that outputs a pure strategy $\hat\pi$, suppose $\hat\pi$ means the i-th player's action is $\hat a_i$ and let $\bm{\hat a}=(\hat a_1,\hat a_2,\cdots,\hat a_m)$. From the structure of the $\mathfrak{M}(\epsilon)$, we know
\begin{align*}
    \text{NE-Gap}(\hat\pi)\ge \epsilon\P_{\bm{a}^\star}(\bm{\hat a} \not= \bm{a}^\star).
\end{align*}
So we only need to use $n$, the number of samples to give a lower bound of $\P_{\bm{a}^\star}(\bm{\hat a} \not= \bm{a}^\star)$ or $\P_{\bm{a}^\star}(\hat a_i \not= a_i^\star)$ 

Let $N(\bm{a})$ be the number of 1s when action $\bm{a}$ is taken. In fact, $\{N(\bm{a}):\bm{a}\in[A_1]\times\cdots\times[A_m]\}$ is a sufficient statistics for the posterior distribution $\bm{a}^\star$, so we have
\begin{align*}
    \E_{\bm{a}^\star\sim \nu}\P_{\bm{a}^\star}(\hat a_1\not= a^\star_1)&\ge\inf_g \E_{\bm{a}^\star\sim \nu}\P_{\bm{a}^\star}(\hat a_1\not= g_1\{N(\bm{a})\})\\
    &\overset{(i)}{\ge}
    \inf_g \E_{\bm{a}^\star\sim \nu}\P_0(\hat a_1\not= g_1\{N(\bm{a})\})
    -\E_{\bm{a}^\star\sim \nu}\text{TV}(\{N(\bm{a})\}|_{\P_0,\mc{A}},\{N(\bm{a})\}|_{\P_{\bm{a}^\star},\mc{A}})\\
    &\overset{(ii)}{\ge}
    \frac{1}{2}
    -\E_{\bm{a}^\star\sim \nu}\text{TV}(\{N(\bm{a})\}|_{\P_0,\mc{A}},\{N(\bm{a})\}|_{\P_{\bm{a}^\star},\mc{A}})\\
    &\overset{(iii)}{\ge}
    \frac{1}{2}
    -\E_{\bm{a}^\star\sim \nu}\sqrt{\frac{1}{2}\text{KL}(\{N(\bm{a})\}|_{\P_0,\mc{A}}\|\{N(\bm{a})\}|_{\P_{\bm{a}^\star},\mc{A}})}\\
    &\overset{(iv)}{=}\frac{1}{2}-\E_{\bm{a}^\star\sim \nu}\sqrt{\frac{1}{2}\sum_{\bm{a}} 
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    \text{KL}(\P_0(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}.
\end{align*}
Above, (i) follows from the definition of total variation distance; (ii) uses the fact that under $\mathbb{P}_0$, we can't get any information about $\bm{a}^\star$, so $\E_{\bm{a}^\star\sim \nu}\P_{\bm{a}^\star}(\bm{\hat a} \not= g\{N(\bm{a})\})=1-\frac{1}{A_1\cdots A_m}$; (iii) uses Pinsker’s inequality; (iv) uses KL divergence decomposition.
Define 
$$
d(\bm{a},\bm{a}^\star)=
\max\{i\in\mathbb{N},i\le m:\bm{a}_j=\bm{a}_j^\star \text{ for all } 1\le j\le i\},$$ where $\max \emptyset =0$. Apparently, $0\le d(\bm{a},\bm{a}^\star)\le m$. After introducing $d(\bm{a},\bm{a}^\star)$, the expected reward $\mc{M}^{\bm{a}^\star}_{\bm{a}}$ is equal to $\frac{1}{2}+d(\bm{a},\bm{a}^\star)\epsilon.$ For the KL divergence, we have
\begin{align*}
    \text{KL}(\P_0(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))
    =&\text{KL}\paren{\paren{\frac{1}{2},\frac{1}{2}}\|\paren{\frac{1}{2}-d(\bm{a},\bm{a}^\star)\epsilon,\frac{1}{2}+d(\bm{a},\bm{a}^\star)\epsilon}}\\
    =&\frac{1}{2}\log \frac{1}{1-4d^2(\bm{a},\bm{a}^\star)\epsilon^2}\\
    \le&4d^2(\bm{a},\bm{a}^\star)\epsilon^2
\end{align*}
for $\epsilon\le\frac{1}{2m}.$ Therefore,
\begin{align*}
    &\frac{1}{2}-\E_{\bm{a}^\star\sim \nu}\sqrt{\frac{1}{2}\sum_{\bm{a}} 
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    \text{KL}(\P_0(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}\\
    \overset{(i)}{\ge}&\frac{1}{2}-\sqrt{\frac{1}{2}\E_{\bm{a}^\star\sim \nu}\sum_{\bm{a}} 
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    \text{KL}(\P_0(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}\\
    = & \frac{1}{2}-\sqrt{\frac{1}{2}\E_{\bm{a}^\star\sim \nu}
    \sum_{k=0}^m\sum_{\bm{a}:d(\bm{a},\bm{a}^\star)=k} 
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    \text{KL}(\P_0(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}\\
    = & \frac{1}{2}-\sqrt{\frac{1}{2}
    \sum_{k=1}^m\E_{\bm{a}^\star\sim \nu}\sum_{\bm{a}:d(\bm{a},\bm{a}^\star)=k}
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    \text{KL}(\P_0(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}\\
    \overset{(ii)}{\ge} & \frac{1}{2}-\sqrt{2
    \sum_{k=1}^m\E_{\bm{a}^\star\sim \nu}\sum_{\bm{a}:d(\bm{a},\bm{a}^\star)=k}
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    k^2\epsilon^2}\\
    = & \frac{1}{2}-\sqrt{\frac{2}{A_1\cdots A_m}
    \sum_{\bm{a},\bm{a}^{\star}:d(\bm{a},\bm{a}^\star)>0}
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    d(\bm{a},\bm{a}^\star)^2\epsilon^2}\\
    = & \frac{1}{2}-\sqrt{\frac{2}{A_1\cdots A_m}
    \sum_{\bm{a}}
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    \sum_{\bm{a}^\star} d^2(\bm{a},\bm{a}^\star)\epsilon^2}\\
    \overset{(iii)}{\ge} & \frac{1}{2}-\sqrt{\frac{20}{A_1}
    \sum_{\bm{a}}
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    \epsilon^2}\\
    =&\frac{1}{2}-\sqrt{\frac{20}{A_1}
    n
    \epsilon^2}
    % \overset{(iv)}{\ge}& \frac{1}{2}-\sqrt{\frac{40}{A_1}
    % \E_{\bm{a}^\star\sim \nu} \sum_{\bm{a}:a_1\not=a_1^\star}
    % \E_{\P_0,\mc{A}}[N(\bm{a})]
    % \epsilon^2}. 
\end{align*}
Above, (i) uses Jensen inequality; (ii) uses the KL divergence's upper bound that we derived. (iii) uses $\#\{\bm{a}^\star:d(\bm{a},\bm{a}^\star)=k\}=(A_{k+1}-1)\prod_{i=k+2}^{m}A_i$, so 
$$
\sum_{\bm{a}^\star}\frac{d^2(\bm{a},\bm{a}^\star)}{A_1\cdots A_m}\le
\sum_{k=1}^\infty \frac{k^2}{2^{k}}<10.
$$
%(iv) uses the fact that $\E_{\P_0,\mc{A}}[N(\bm{a})]$ is independent of $\bm{a}^\star$, so 
% $$
% \sum_{\bm{a}}\E_{\P_0,\mc{A}}[N(\bm{a})]=\frac{A_1}{A_1-1}\E_{\bm{a}^\star\sim \nu} \sum_{\bm{a}:a_1\not=a_1^\star}\E_{\P_0,\mc{A}}[N(\bm{a})].
% $$.
To summarize the argument, we proved that
\begin{align}
\label{equation:proof_lower_bound}
\E_{\bm{a}^\star\sim \nu}\P_{\bm{a}^\star}(\hat a_1 \not= a^\star_1)
\ge
\frac{1}{2}-\sqrt{\frac{20}{A_1}
    n
    \epsilon^2}.    
\end{align}
(\ref{proof_lower_bound}) tells us that if $n<\frac{A_1}{160\epsilon^2}$, we have
$$
\E_{\bm{a}^\star\sim \nu}\P_{\bm{a}^\star}(\hat a_1\not= a^\star_1)
\ge\frac{1}{4}.
$$
As a result, 
\begin{align*}
    \E_{\bm{a}^\star\sim \nu} \sum_{\bm{a}:\hat a_1\not= a^\star_1}
    \E_{\P_{\bm{a}^\star,\mc{A}}}N(a) &= \E_{\bm{a}^\star\sim \nu} \sum_{t=1}^n\P_{\bm{a}^\star}(\hat a_1\not= a^\star_1)\\
    &\ge \frac{n}{4}.
\end{align*}
To avoid $\epsilon/4$-sub-optimality, we must have $n\ge \frac{A_1}{160\epsilon^2}$, we still have
\begin{align}
\label{inequality:lowerbound1}
    \E_{\bm{a}^\star\sim \nu} \sum_{\bm{a}:\hat a_1\not= a^\star_1}
    \E_{\P_{\bm{a}^\star,\mc{A}}}N(a)
    \ge \frac{n}{4}\ge\frac{A_1}{640\epsilon^2}.
\end{align}
 
If we choose $\P_{\bm{a}^\star,k}$ as a base game, such that $\P_{\bm{a}^\star,k}$ and $\P_{\bm{a}^\star}$ only differ at $\bm{a}:d(\bm{a},\bm{a}^\star)> k$ where the reward of $\P_{\bm{a}^\star,k}$ is sampled from Bernoulli($\frac{1}{2}+k\epsilon$). Let $\bm{a}_{-k}$ denotes $(a_{k+1},\dots,a_m)$ and $\nu_{-k}$ denotes the uniform distribution on $[A_{k+1}],\dots,[A_m]$. Then fix $a^\star_1,\dots,a^\star_k$, by a similar argument, we can proved that to avoid $\epsilon/4$-sub-optimality for all game instance, we must have
\begin{align}
\label{inequality:lowerbound2}
    \E_{\bm{a}^\star_{-k}\sim \nu_{-k}} \sum_{\bm{a}:a_1=a^\star_1,\dots,a_k=a^\star_k,\hat a_{k+1}\not= a^\star_{k+1}}
    \E_{\P_{\bm{a}^\star,\mc{A}}}N(a)
    \ge\frac{A_{k+1}}{640\epsilon^2}.
\end{align}
Putting (\ref{inequality:lowerbound1}) and (\ref{inequality:lowerbound2}) together, to avoid $\epsilon/4$-sub-optimality, we must have 
\begin{align*}
    n&= \sum_{k=0}^{m-1}\E_{\bm{a}^\star\sim \nu}\sum_{\bm{a}:a_1=a^\star_1,\dots,a_k=a^\star_k,\hat a_{k+1}\not= a^\star_{k+1}}
    \E_{\P_{\bm{a}^\star,\mc{A}}}N(a)\\
    &\ge \frac{\sum_{i=1}^m A_i}{640\epsilon^2}.
\end{align*}
So we can choose $c_0$ as $\frac{1}{640}.$
\begin{align*}
    \E_{\bm{a}^\star_{-k}\sim \nu_{-k}}\P_{\bm{a}^\star}(\hat a_{k+1} \not= a_{k+1}^\star)&\ge\inf_g \E_{\bm{a}^\star_{-k}\sim \nu_{-k}}\P_{\bm{a}^\star}(\hat a_{k+1} \not= g_{k+1}\{N(\bm{a})\})\\
    &\ge\frac{1}{2}-\E_{\bm{a}^\star_{-k}\sim \nu_{-k}}\sqrt{\frac{1}{2}\sum_{\bm{a}} 
    \E_{\P_{\bm{a}^\star,k},\mc{A}}[N(\bm{a})]
    \text{KL}(\P_{\bm{a}^\star,k}(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}\\
    &\ge\frac{1}{2}-\sqrt{\frac{1}{2}\E_{\bm{a}^\star_{-k}\sim \nu_{-k}}\sum_{\bm{a}} 
    \E_{\P_{\bm{a}^\star,k},\mc{A}}[N(\bm{a})]
    \text{KL}(\P_{\bm{a}^\star,k}(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}\\
    &=  \frac{1}{2}-\sqrt{\frac{1}{2}\E_{\bm{a}^\star_{-k}\sim \nu_{-k}}
    \sum_{j=k+1}^m\sum_{\bm{a}:d(\bm{a},\bm{a}^\star)=j} 
    \E_{\P_{\bm{a}^\star,k},\mc{A}}[N(\bm{a})]
    \text{KL}(\P_{\bm{a}^\star,k}(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}\\
    &=  \frac{1}{2}-\sqrt{\frac{1}{2}
    \sum_{j=k+1}^m\E_{\bm{a}^\star_{-k}\sim \nu_{-k}}\sum_{\bm{a}:d(\bm{a},\bm{a}^\star)=j}
    \E_{\P_{\bm{a}^\star,k},\mc{A}}[N(\bm{a})]
    \text{KL}(\P_{\bm{a}^\star,k}(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}\\
    &\ge\frac{1}{2}-\sqrt{2
    \sum_{j=k+1}^m\E_{\bm{a}^\star_{-k}\sim \nu_{-k}}\sum_{\bm{a}:d(\bm{a},\bm{a}^\star)=j}
    \E_{\P_{\bm{a}^\star,k},\mc{A}}[N(\bm{a})]
    (j-k)^2\epsilon^2}\\
     &= \frac{1}{2}-\sqrt{\frac{2}{A_{k+1}\cdots A_m}
    \sum_{\bm{a},\bm{a}^{\star}:d(\bm{a},\bm{a}^\star)>k}
    \E_{\P_{\bm{a}^\star,k},\mc{A}}[N(\bm{a})]
    (d(\bm{a},\bm{a}^\star)-k)^2\epsilon^2}\\
    &\ge \frac{1}{2}-\sqrt{\frac{20}{A_{k+1}}
    \sum_{\bm{a}:a_1=a_1^\star,\dots,a_k=a_k^\star}
    \E_{\P_{\bm{a}^\star,k},\mc{A}}[N(\bm{a})]
    \epsilon^2}. 
\end{align*}
 
\end{proof-of-theorem}


==> Sections/cce.tex <==
\section{Efficient Learning of Coarse Correlated Equilibria (CCE)}
\label{section:cce}

Given the difficulty of learning Nash when the number of players $m$ is large , we consider learning other relaxed notions of equilibria for general-sum MGs. Two standard notions of equilibria for games are the Correlated Equilibrium (CE) and Coarse Correlated Equilibrium (CCE), and they satisfy $\set{{\rm Nash}} \subset \set{{\rm CE}}\subset \set{{\rm CCE}}$ for general-sum MGs~\citep{nisan2007algorithmic}.


% \yub{move to prelim?}
%\ yub{remove $\mc{B}$, and move to preliminaries}

We begin by considering learning CCE (most relaxed notion above) for Markov games.
\begin{definition}[$\epsilon$-approximate CCE for general-sum MGs]
  We say a (general) correlated policy $\pi$ is an \emph{$\epsilon$-approximate Coarse Correlated Equilibrium ($\epsilon$-CCE)} if
$$
\max_{i\in[m]} \paren{V_{1,i}^{\dagger,\pi_{-i}}(s_1)- V_{1,i}^{\pi} (s_1)} \le \epsilon.
$$
We say $\pi$ is an (exact) CCE if the above is satisfied with $\eps=0$.
\end{definition}


% ~\yub{Assume deterministic $s_1$.}~\ziang{$\surd$}

% To put it another way, CCE plays an role of a contract, if every player abide by this contract, then no player have motivation to change its policy. CCE always exists because Nash equilibrium is also a CCE. 

The following result shows that there exists an algorithm that can learn an $\epsilon$-approximate CCE in general-sum Markov games within $\widetilde{\mc{O}}(H^5 S \max_{i\in[m]} A_i /\epsilon^2)$ episodes of play. 
\begin{theorem}[Learning $\eps$-approximate CCE for general-sum MGs]
  \label{theorem:proof_general_cce}
  Suppose we run the \multiv~algorithm (Algorithm~\ref{algorithm:nash_v_general}) for all $m$ players and
  %There exists an algorithm \multiv~(Algorithm~\ref{algorithm:nash_v_general}) for $m$-player general-sum MGs, such that running it for 
  \begin{align*}
    K\ge \cO \paren{\frac{H^5S\max_{i\in[m]}A_i\iota}{\epsilon^2}+\frac{H^4S\iota^3}{\epsilon}}
  \end{align*}
  episodes ($\iota=\log (m\max_{i\in[m]} A_i HSK/ (p\epsilon))$ is a log factor). Then  with probability at least $1-p$, the certified policy $\hat\pi$ defined in Algorithm \ref{algorithm:certified_policy_general} is an $\epsilon$-CCE, i.e. $\max_{i\in[m]} ( V_{1,i}^{\dagger,\hat\pi_{-i}}(s_1)- V_{1,i}^{\hat\pi} (s_1) )\le \epsilon$.
\end{theorem}

\paragraph{Mild dependence on action space}
For small enough $\eps$, the sample complexity featured in Theorem~\ref{theorem:proof_general_cce} scales as $\tO (H^5S\max_{i\in[m]}A_i /\eps^2)$. Most notably, this is the first algorithm that scales with $\max_{i\in[m]} A_i$, and exhibits a sharp difference in learning Nash and learning CCE in view of the $\exp({\Omega(m)})$ lower bound for learning Nash in Proposition~\ref{theorem:rubinstein-formal}. Indeed, existing algorithms such as Multi-Nash-VI Algorithm with CCE subroutine~\citep{liu2021sharp} does require $\tO(H^4S^2\prod_{i=1}^mA_i/\epsilon^2)$ episodes of play, which scales with $\prod_{i\in[m]}A_i$ due to its model-based nature. We achieve significantly better dependence on $A_i$ and also $S$, though slightly worse $H$ dependence.

\paragraph{Overview of algorithm and techniques}
Our \multiv~algorithm (deferred to Appendix~\ref{appendix:cce-algorithm} due to space limit) is a multi-player adaptation of the Nash V-Learning algorithm of~\citet{bai2020near,tian2021online} for learning Nash equilibria in two-player zero-sum MGs. Similar as~\citet{bai2020near}, we show that this algorithm enjoys a ``no-regret'' like guarantee for each player at each $(h,s)$ (Lemma~\ref{lemma:cce-bonus}). We also adopted the choice of hyperparameters in \cite{tian2021online} so that the sample complexity has a slightly better dependence in $H$. When combined with the ``certified correlated policy'' procedure (Algorithm~\ref{algorithm:certified_policy_general}), our algorithm outputs a policy that is $\eps$-CCE. 
Our certified policy procedure is adapted from the certified policy of \cite{bai2020near}, and differs in that ours output a \emph{correlated} policy for all the players whereas \cite{bai2020near} outputs a product policy.
The key feature enabling this $\max_{i\in[m]}A_i$ dependence is that this algorithm uses decentralized learning for each player to learn the value function ($V$), instead of learning the $Q$ function (as in \citet{liu2021sharp}) that requires sample size scales as $\prod_{i \in [m]} A_i$.
The proof of Theorem~\ref{theorem:proof_general_cce} is in Appendix~\ref{section:proof in CCE}.
% The key feature enabling this $\max_{i\in[m]}A_i$ dependence is that this algorithm uses~\emph{uncoupled learning} for each player, as opposed to the centralized model-based algorithm of~\citet{liu2021sharp}. 
% \sm{}

% This can be seen in Algorithm~\ref{algorithm:certified_policy_general} as a common, randomly sampled $k$ and $l$ in Line \ref{sample_k} and Line \ref{sample_l}, are used by all the players.
% \yub{fix the quote sign}\ziang{fixed}

% For multi-player general-sum MGs, it not likely to learn Nash in general-sum Markov games (similar as independent no-regret dynamics for bimatrix games~\citep{hart2003uncoupled}). 

%  and is an uncoupled (independent) learning algorithm in which each player uses incremental value updates and the Follow-The-Regularized-Leader (FTRL) to compute her own policy. 
% We extend this algorithm naturally to the multi-player general-sum setting. 

% ~\yub{shall we say averaging leads to CCE is known in matrix games}


% This sample complexity upper bound $\widetilde O(H^5S\max_{i\in[m]}A_i/\epsilon^2)$ significantly improves the best existing sample complexity upper bound for approximate CCE, in \cite{liu2021sharp}. And from Theorem \ref{theorem:proof_general_cce}, we know that there's no exponential barrier w.r.t. $m$ in computing the approximate CCE in general-sum Markov games.

% \yub{algorithm}


%~\yub{proof is deferred to appendix xx}

% We can learn the approximate CCE from general-sum Markov games efficiently.


% \subsection{Algorithm Description}
% \yub{Change alg name to $V$-Learning.}
% The algorithm is adapted from Nash V-learning~\citep{bai2020near,tian2021online}. 

% There, Nash V-learning is proved to be a near optimal algorithm in learning $\epsilon$-approximate Nash equilibrium in zero-sum games with sample complexity $\widetilde O (H^6S\max\{A,B\})/\epsilon^2)$ , where $A,B$ is the number of actions of max-player and min-player. The output of Nash V-learning is a nested mixture of Markov policies. Here, we apply Nash V-learning in general-sum Markov games to learn $\epsilon$-approximate CCE. 






% \yub{algorithm box into 3 sub-boxes}

% \yub{definition}

% \yub{discussion of algorithm}

% \yub{theorem statement}

% \yub{discussion of techniques, comparison with prior works}



    %   \FOR{all $a,a' \in \mc{A}_i$}
    %   \STATE $\up{\ell}_{h,i}(s_h, a) \setto [H -h+1- r_{h,i}-\min\{\up{V}_{h+1,i}(s_{h+1}),H-h\}] \mathbb{I}\{a_h=a\}/[\mu_h(a_h|s_{h}) +\gamma_t]$.
    %   \STATE $\up{\ell}_{h,i}(s_h, \bm{p}) \defeq \sum_{a\in A_i}\up{\ell}_{h,i}(s_h, a) p(a) $
    %   \STATE $\up{L}^{a\to  a'}_{h,i}(s_h)\setto (1-\alpha_t)\up{L}^{a\to a'}_{h,i}(s_h,a,a')+\alpha_t\up{\ell}_{h,i}(s_h,\bm{p}_t^{a\to a'})$
    %   % \STATE $\up{L}_h( s_h, a)  \setto ( 1-\alpha _t )\up{L}_h( s_h,a ) +\alpha_t \up{\ell}_h(s_h, a)$.
      
    %   \STATE Set $u^{a\to a'}(\cdot |s_h) \propto \exp[-(\up{\eta}_t/\alpha_t) \up{L}^{a\to a'}_{h,i}( s_h)]$.
    %   \STATE Solve $\sum_{a\not=a'}u^{a\to a'} \Tilde{\bm{p}}^{a\to a'}=\Tilde{\bm{p}}$
    %   \STATE Set $\mu_{h,i}(s_h) = \Tilde{\bm{p}}_t$%=(1-\gamma_t)\Tilde{\bm{p}}+\frac{\gamma_t}{A_i}\textbf{1}.
    %   \ENDFOR
    % \STATE $\up{\ell}_{h,i}(s_h, a) \setto [H -h+1- r_{h,i}-\min\{\up{V}_{h+1,i}(s_{h+1}),H-h\}] \mathbb{I}\{a_h=a\}/[\mu_h(a_h|s_{h}) +\gamma_t]$
    % \STATE Call algorithm \ref{algorithm:external_to_swap} with input BLABLA....

==> Sections/ce.tex <==
\section{Efficient Learning of Correlated Equilibria (CE)}
\label{section:ce}

In this section, we move on to considering the harder problem of learning Correlated Equilibria (CE). We first present the definition of CE in Markov games.


% \ziang{define dagger for policy modification in this section}

\begin{definition}[Strategy modification for \ith player]
A strategy modification $\phi\defeq\set{\phi_{h,s}}_{(h,s)\in[H]\times\mc{S}}$ for player $i$ is a set of $H \times S$ functions $\phi_{h,s}:(\mc{S}\times \mc{A})^{h-1}\times\mc{A}_i\to\mc{A}_i$. A strategy modification $\phi$ can be composed with any policy $\pi$ to give a modified policy $\phi\circ\pi$ defined as follows: At any step $h$ and state $s$ with the history information $\tau_{h-1} = (s_1, \bm{a}_{1}, \cdots, s_{h-1}, \bm{a}_{ h-1})$, if $\pi$ chooses to play $\bm{a}=(a_1,\dots,a_m)$, the modified policy $\phi\circ\pi$ will play $(a_1,\dots,a_{i-1},\phi_{h,s}(\tau_{h-1},a_i),a_{i+1},\dots,a_m)$. We use $\Phi_i$ denote the set of all possible strategy modifications for player $i$.

% Here there's no restriction on policy $\pi$. 
% (we don't need to distinguish between Markov and non-Markov policy)
\end{definition}

\begin{definition}[$\eps$-approximate CE for general-sum MGs]
We say a (general) correlated policy $\pi$ is an $\eps$-approximate CE ($\epsilon$-CE) if 
\begin{align*}
    \max_{i\in[m]}\sup_{\phi\in\Phi_i} \paren{V_{1,i}^{\phi\circ\pi}(s_1) - V_{1,i}^{\pi}(s_1)} \le \epsilon.
\end{align*}
We say $\pi$ is an (exact) CE if the above is satisfied with $\eps=0$.
\end{definition}

% \begin{align*}
%     V_{h,i}^{\dagger,\hat\pi_{-i}}(s) \defeq
%     \sup_{\phi}V_{h,i}^{\phi_i\circ\pi}(s).
% \end{align*}

Our definition of CE follows~\citep{liu2021sharp} and is a natural generalization of the CE for the well-studied special case of one-step (i.e. normal form) games~\citep{nisan2007algorithmic}. 


\subsection{Algorithm description}

 Our algorithm \cev~(Algorithm~\ref{algorithm:ce_v_general}) builds further on top of \multiv~and Nash V-Learning, and makes several novel modifications in order to learn the CE. The key feature of \cev~is that it uses a weighted swap regret algorithm (mixed-expert FTRL) for every $(s,h,i)$. At a high-level, \cev~consists of the following steps:
\begin{itemize}[leftmargin=20pt, topsep=0pt]
    \item Line~\ref{line:cev-ftrl-1}-\ref{line:cev-ftrl-2} (Sample action using mixed-expert FTRL): For each $(h, s)$ we maintain $A_i$ ``sub-experts'' indexed by $b'\in[A_i]$ (Each sub-expert represents an independent ``expert'' that runs her own FTRL algorithm). Sub-expert $b'$ first computes an action distribution $q^{b'}(\cdot)\in\Delta_{\mc{A}_i}$ via Follow-the-Regularized-Leader (FTRL; Line~\ref{line:cev-ftrl-update}). Then we employ a two-step sampling procedure to obtain the action: First sample a sub-expert $b$ from a suitable distribution $\mu$ computed from $\{q^{b'}\}_{b'\in[A_i]}$, then sample the actual action $a_{h,i}$ from $q^b$. 
    \item Line~\ref{line:cev-observe-1}-\ref{line:cev-observe-2} (Take action and record observations): Player $i$ takes action $a_{h,i}$ and observes other player's actions, the reward, and the next state. Sub-expert $b$ then computes a loss estimator and weight according to the observations, which will be used in future FTRL updates.
    \item Line~\ref{line:cev-value} (Optimistic value update): Updates the optimistic estimate of the value $\up{V}_{h,i}$ using step-size $\alpha_t$ and bonus $\up{\beta}_t$.
\end{itemize}
Finally, after executing Algorithm~\ref{algorithm:ce_v_general} for $K$ episodes, we use the certified correlated policy procedure (Algorithm~\ref{algorithm:certified_policy_general}) to obtain our final output policy $\what{\pi}$. This procedure is a direct modification of the certified policy procedure of~\citep{bai2020near} and outputs a correlated policy (because the randomly sampled $k$ and $l$ in line \ref{sample_k} and line \ref{sample_l} of Algorithm \ref{algorithm:certified_policy_general} are used by all the players) instead of product policy. The same procedure is also used for learning CCEs earlier in Section~\ref{section:cce}. 

Here we specify the hyperparameters used in Algorithm~\ref{algorithm:ce_v_general}:
\begin{align}
\label{equation:alpha_t}
    \alpha_{t} = (H+1)/(H+t), \quad \eta_{t}=\sqrt{\iota/(A_i t)}, \quad \up{\beta}_{t}=cH^2 A_i \sqrt{\iota/t} + 2cH^2\iota/t.
\end{align}
The constants $\alpha_t^j$ used in Algorithm~\ref{algorithm:certified_policy_general} is defined as
\begin{align}
\label{equation:def_alpha_t^j}
    \textstyle
    \alpha_{t}^{0}:=\prod_{k=1}^{t}\left(1-\alpha_{k}\right),~~~ \alpha_{t}^{j}:=\alpha_{j} \prod_{k=j+1}^{t}\left(1-\alpha_{k}\right).
\end{align}
% Their properties are listed in the Lemma \ref{lemma:alpha_t^j}. 
Note that for any $t\ge 1$, $\{\alpha_t^j\}_{1\le j\le t}$ sums to one and defines a distribution over $[t]$.

% \ziang{$2c$ in bonus is because $\sum_{j=1}^t\alpha_t^j/j\le 1/(2t)$ instead of $1/t$, so taking $\beta$ from outside to inside need to pay 2, here $c$ is the constant in Lemma \ref{lemma:ce-bonus}}


% \paragraph{Certified policy} This part is the same... 


% \yub{Make a good name for algorithm. For example, CE-V?}


\begin{algorithm}[t]
   \caption{\cev~for general-sum MGs ($i$-th player's version)}
   \label{algorithm:ce_v_general}
   \begin{algorithmic}[1]
    \REQUIRE Hyperparameters: $\{ \alpha_t^j \}_{1 \le j \le t \le K}$, $\{ \alpha_t \}_{1 \le t \le K}$, $\{ \eta_t \}_{1 \le t \le K}$, $\{ \bar \beta_t \}_{1 \le t \le K}$. 
      \STATE {\bfseries Initialize:} For any $(s, a, h)$, set $\up{V}_{h,i}(s)\setto H$, $N_h(s)\setto 0$. Set $\mu_h(a|s)\setto 1/A_i$, $q^{b'}_h(a|s)\setto 1/A_i$, $\ell^{b'}_{h, t}(a|s)\setto 0$, $N_h^{b'}(s)\setto 0$ for all $(b', a, h, s, t)\in [A_i]\times [A_i]\times [H]\times \mc{S}\times [K]$.
      \FOR{episode $k=1,\dots,K$}
      \STATE Receive $s_1$.
      \FOR{step $h=1,\dots, H$}
      \STATE {\color{blue} // Compute \emph{proposal} action distributions by FTRL}
      \STATE Update accumulator $t\defeq N_{h}(s_h)\setto N_{h}(s_h) + 1$. Set $u_t \setto \alpha_t^t / \alpha_t^1$. \label{line:cev-ftrl-1}
      \STATE Let $t_{b'}\setto N_h^{b'}(s_h)$ for all $b'\in[A_i]$ for shorthand.
      \STATE \label{line:cev-ftrl-update} Compute the action distribution for all sub-experts $b'\in[A_i]$: 
      \begin{align*}
        \textstyle
        q_h^{b'}(a | s_h) \propto_a \exp\big( -(\eta_{t_{b'}} / u_t) \sum_{\tau=1}^{t_{b'}} w_{h, \tau}(b'|s_h) \ell^{b'}_{h, \tau}(a | s_h) \big).
      \end{align*}      
      % w_{h,t_b}(b|s_h)
      \vspace{-1em}
      \STATE {\color{blue} // Sample sub-expert $b$ and action from $q^b(\cdot)$}
      \STATE Compute $\mu_h(\cdot|s_h)\in\Delta_{[A_i]}$ by solving $\mu_h(\cdot | s_h) =\sum_{b'=1}^{A_i} \mu_h(b'|s_h) q_h^{b'}(\cdot | s_h)$. \label{line:cev-linear-system}
      \STATE Sample sub-expert $b\sim \mu_h(\cdot|s_h)$, and then action $a_{h,i}\sim q_h^b(\cdot |s_h)$. \label{line:cev-ftrl-2}
      \STATE {\color{blue} // Take action and feed the observations to sub-expert $b$}
      \STATE Take action $a_{h,i}$, observe the actions $\bm{a}_{h, -i}$ from all other players. \label{line:cev-observe-1}
      \STATE Observe reward $r_{h,i}=r_{h,i}(s_h, a_{h, i}, \bm{a}_{h, -i})$ and the next state $s_{h+1}$ from the environment.
      \STATE Update accumulator for the sampled sub-expert: $t_b\defeq N_h^b(s_h)\setto N_h^b(s_h)+1$.
      \STATE Compute and update loss estimator 
      \begin{align*}
          \ell^b_{h, t_b}(a| s_h) \setto \frac{\brac{H-h+1 - (r_{h,i} + \min\{\up{V}_{h+1,i}(s_{h+1}),H-h\})}/H    \cdot \indic{a_{h,i}=a} }{ q^b_h(a|s_h) + \eta_{t_b}}.
      \end{align*}
      \STATE Set $w_{h,t_b}(b|s_h) \setto u_t$. \label{line:cev-observe-2}
      % previous w_t are still correct b/c ratio is invariant to the subscript t.

      \STATE {\color{blue} // Optimistic value update}
      \STATE $\up{V}_{h,i}\left(s_{h}\right) \setto  \left(1-\alpha_{t}\right) \up{V}_{h,i}\left(s_{h}\right)+\alpha_{t}\left(r_{h,i}\left(s_{h}, a_{h,i}, \bm{a}_{h, -i}\right)+\up{V}_{h+1,i}\left(s_{h+1}\right)+\up{\beta}_{t}\right)$. \label{line:cev-value}
      \ENDFOR
      \ENDFOR
   \end{algorithmic}
\end{algorithm}

\subsection{Overview of techniques}
\label{section:ce-techniques}

Here we briefly overview the techniques used in Algorithm~\ref{algorithm:ce_v_general}.

{\bf Minimizing swap regret via mixed-expert FTRL } The key technical advance in our Algorithm~\ref{algorithm:ce_v_general} over \ccev~and Nash V-Learning is the use of mixed-expert FTRL (Line~\ref{line:cev-ftrl-1}-\ref{line:cev-ftrl-2}). The purpose of this is to allow the algorithm to achieve low \emph{swap regret} at each $(h,s)$ in a suitable sense---For one-step (normal form) games, it is known that combining low-swap-regret learning for each player leads to an approximate CE~\citep{stoltz2005incomplete,cesa2006prediction}. To integrate this into Markov games, we utilize a celebrated reduction from low-swap-regret learning to usual low-regret learning~\citep{blum2007external}, which for any bandit problem with $A_i$ actions maintains $A_i$ \emph{sub-experts} each running its own FTRL algorithm. Our particular application builds upon the \emph{two-step randomization} scheme of~\citet{ito2020tight} which first samples a sub-expert $b$ and the action from this sub-expert. The distribution $\mu(\cdot)$ for sampling the sub-expert is carefully chosen by solving a linear system (Line~\ref{line:cev-linear-system}) so that $\mu$ also coincides with the (marginal) distribution of the sampled action, from which the reduction follows. 

% \yub{1. It is known that low swap regret leads to CE, thus we use the mixed sub-experts technique of Blum and Mansour 2007, Ito 2020. 2. Fictitious distribution for all sub-experts, but only one of them actually plays, and the one that plays follows the correct weighted FTRL update. 3. Weighted swap regret requires each bandit admits random weights; we develop techniques for this.}

{\bf FTRL with predictable weights } Applied naively, the above reduction does not directly work for our purpose, as our analysis requires minimizing the \emph{weighted} swap regret with weights $\alpha_t^i$, whereas the reduction of~\cite{ito2020tight} relies crucially on the vanilla (average) regret. We address this challenge by using a slightly modified FTRL algorithm for each sub-expert that takes in random but \emph{predictable} weights (i.e. depending fully on prior information and ``external'' randomness). We present the analysis for such FTRL algorithm in Appendix~\ref{appendix:predictable-regret}, and the consequent analysis for the weighted swap regret in Appendix~\ref{appendix:swap-regret}-\ref{appendix:proof-swap}, both of which may be of independent interest.

{\bf Proposal distributions } Finally, a nuanced but important new design in \cev~is that all sub-experts compute a \emph{proposal} action distribution to sample the sub-expert and the associated action. Then, only the sampled sub-expert takes this action, and all other proposal distributions are discarded. This is different from the original algorithms of~\citep{blum2007external,ito2020tight} in which the FTRL update come \emph{after} the sub-expert sampling and only happens for the sampled sub-expert. Our design is required here as otherwise the sub-experts are required to predict the next time when it is sampled in order to compute the weighted FTRL update, which is impossible.


% Definition for V_lower (only for analysis): 
% $\underline{V}_{h,i}(s)\setto 0$
%   \STATE $\underline{V}_{h,i}\left(s_{h}\right) \setto  \left(1-\alpha_{t}\right) \underline{V}_{h,i}\left(s_{h}\right)+\alpha_{t}\left(r_{h,i}\left(s_{h}, a_{h}, a'_{h}\right)+\underline{V}_{h+1,i}\left(s_{h+1}\right)-\up{\beta}_{t}\right)$.


%   q_{\hat{a}}^{n_{\hat{a}}}\propto \exp{\set{-\eta_{n_{\hat{a}}}/w_{n_{\hat{a}}}(\hat{a})\sum_{k=1}^{n_{\hat{a}}-1}w_{k}(\hat{a})\hat{\ell}_{t_{\hat{a}}^k}}}
% where $w_{k}(\hat{a})=\alpha_{t_{\hat{a}}^k}^{t_{\hat{a}}^k}/\alpha_{t_{\hat{a}}^k}^1$, $t_{\hat{a}}^k$ is the index $t$ when $\hat{a}$ is chosen the $k$-th time.

% \yub{The following is copied from CCE part. I will move them.}
% ~\yub{in the sample complexity}.



% \paragraph{Certified policy} 
% The certified policy is constructed on the history of Algorithm \ref{algorithm:nash_v_general}, i.e. $\{\mu_{h,i}^k\}$ and $\{s_h^k\}$ for $h,i,k\in[H]\times[m]\times[K]$. $N_h^k(s_h)$ refers to the times that $s_h$ is observed at step $h$ in the first $k$ episodes. $k_t^l(s_h)$ refers to the episodes index when $s_h$ is observed for the l-th time. $\alpha_t^j$ is defined as 

% Note that we need all players use the same $k$ in certified policy, so $\hat\pi$ would be a correlated policy. This in different from Nash V-learning.


% Nash V-learning use independent certified for max-player and min-player. In fact, V-learning enables players to perform no-regret learning. In zero-sum games, no-regret learning against another player's empirical policy is equivalent to no-regret learning against another player's certified policy. Thus Nash equilibrium can be learned. However, in general-sum games, though each player still learns policy in a no-regret learning manner, other player's empirical policy is related to certified correlated policy. We can't decouple the correlation of empirical policy. Thus in general-sum games, independent certified policy does not work. So here, the learning objective becomes CCE.~\yub{Note to self: polish this discussion}

% Because each player independently follows no-regret learning, the sample complexity is only related to $A_i$, so the overall sample complexity only requires $\max_{i\in[m]}A_i$, getting rid of the (exponential) dependence of $m$.

% After running  Algorithm \ref{algorithm:nash_v_general} for all $m$ players, we use joint certified policy (Algorithm \ref{algorithm:certified_policy_general}) to get a general (non-Markov) correlated policy which is an $\epsilon$-approximate CCE.~\yub{Say in essence what is learned by V learning, and why that gives CCE.}~\yub{Later, comment on why this only requires $\max A_i$ samples. this is because of independent learning.}\ziang{$\surd$}

% After running  Algorithm \ref{algorithm:nash_v_general} for all $m$ players and Algorithm \ref{algorithm:certified_policy_general}, we can learn a certified policy $\hat\pi$. Then,

\begin{algorithm}[t]
  % \setstretch{1.2}
  \caption{Certified correlated policy $\hat\pi$ for general-sum MGs}
  \label{algorithm:certified_policy_general}
  \begin{algorithmic}[1]
    \STATE\label{sample_k} Sample $k$ $\setto$ $\text{Uniform}([K])$.
    \FOR{step $h=1,\dots,H$}
    \STATE Observe $s_h$, and set $t\setto N_h^k(s_h)$ (the value of $N_h(s_h)$ at the beginning of the $k$'th episode).
    \STATE\label{sample_l} Sample $l\in[t]$ with $\P(l=j) = \alpha_t^j$ (c.f. Eq. (\ref{equation:def_alpha_t^j})).
    \STATE Update $k\setto k_h^l(s_h)$ (the episode at the end of which the state $s_h$ is observed exactly $l$ times).
    \STATE Jointly take action $(a_{h,1}, a_{h,2},\dots,a_{h,m})\sim \prod_{i=1}^m\mu_{h,i}^k(\cdot|s_h)$, where $\mu_{h, i}^k(\cdot \vert s_h)$ is the policy $\mu_{h,i}(\cdot|s_h)$ at the beginning of the $k$'th episode. %\sm{begin or end?}
    % \sm{change $p$ to $\mu$}.
    % ~\yub{all players use the same $k$, therefore is correlated policy}
    \ENDFOR
  \end{algorithmic}
\end{algorithm}


\subsection{Theoretical guarantee}

We are now ready to present the theoretical guarantee for our \cev~algorithm.

\begin{theorem}[Learning $\eps$-approximate CE for general-sum MGs]
\label{theorem:proof_general_ce}
Suppose we run the \cev~algorithm (Algorithm~\ref{algorithm:ce_v_general}) for all $m$ players for 
$$
K\ge \mc{O}\paren{\frac{H^6S\max_{i\in[m]}A_i^2\iota}{\epsilon^2}+\frac{H^4S\max_{i\in[m]}A_i\iota^3}{\epsilon}}
$$
episodes ($\iota=\log (m\max_{i\in[m]} A_i HSK/ (p\epsilon))$ is a log factor). Then with probability at least $1-p$,  the certified correlated policy $\what{\pi}$ defined in Algorithm \ref{algorithm:certified_policy_general} is an $\eps$-CE, i.e. $\max_{i\in[m]} \sup_{\phi\in \Phi_i}(V_{1,i}^{\phi\circ\hat\pi}(s_1)- V_{1,i}^{\hat\pi} (s_1))\le \epsilon$.
\end{theorem}

\paragraph{Discussions}
To the best of our knowledge, Theorem~\ref{theorem:proof_general_ce} presents the first result for learning CE that scales polynomially with $\max_{i\in[m]} A_i$, which is significantly better than the best known existing algorithm of Multi-Nash-VI with CE subroutine~\citep{liu2021sharp} whose sample complexity scales with $\prod_{i\in[m]} A_i$. Similar as in Theorem~\ref{theorem:proof_general_cce}, this follows as our \cev~uses decentralized learning for each player to learn the value function ($V$) .
We also observe that our sample complexity for learning CE is higher than for learning CCE by a factor of $\tO(H\max_{i\in[m]} A_i)$; the additional $\max_{i\in[m]} A_i$ factor is expected as CE is a strictly harder notion of equilibrium. The proof of Theorem~\ref{theorem:proof_general_ce} can be found in Appendix~\ref{appendix:proof-ce}.

% and required a more sophisticated mixed-expert FTRL technique in the inner loop of the algorithm. \sm{We also observe that our sample complexity for learning CE is higher than for learning CCE by a factor of $\max_{i\in[m]} A_i$, which is expected as CE is a strictly harder notion of equilibrium. }

%Finally, combining Theorem~\ref{theorem:proof_general_cce} \&~\ref{theorem:proof_general_ce} with the exponential lower bound for learning Nash (Section~\ref{section:exp_nash}), we obtain a full characterization of which equilibria can be learned with ${\rm poly}(m)$ sample complexity in general-sum Markov games: This is possible for CCE and CE, but not Nash. 

% ~\yub{consider remove}


% There exists an algorithm \multiv~(Algorithm~\ref{algorithm:nash_v_general}) for $m$-player general-sum MGs, such that running it for $K$ episodes and using Algorithm \ref{algorithm:certified_policy_general} to obtain the certified policy $\what{\pi}$, we have with probability at least $1-p$ that $\hat\pi$ will be $\epsilon$-approximate CCE, i.e. $\max_{i\in[m]} V_{1,i}^{\dagger,\hat\pi_{-i}}(s_1)- V_{1,i}^{\hat\pi} (s_1)\le \epsilon$, as long as the number of episodes
%   \begin{align*}
%   K\ge \cO \paren{\frac{H^5S\max_{i\in[m]}A_i\iota}{\epsilon^2}+\frac{SH^2+H^3\iota^3}{\epsilon}},
%   \end{align*}

  
% \yub{discussions, again compare with liu et al. To the best of our knowledge this is first... Also compare with our own CCE results. say that we now have a complete picture over nash, CE, CCE.}

% \yub{technical-wise, we showed BLAH, which may be of independent interest.}

==> Sections/exponential_lower_bound.tex <==
\subsection{Exponential lower bound for learning approximate Nash equilibrium}
\label{section:exp_nash}

The focus of this paper is the setting where the number of players $m$ is large. Intuitively, as the joint action space has size $|\mc{A}|=\prod_{i=1}^m A_i$ which scales exponentially in $m$ (if each $A_i\ge 2$), naive algorithms for learning Nash equilibrium may learn all $r_i(\bm{a})$ by enumeratively querying all $\bm{a}\in\mc{A}$, and this costs exponential in $m$ samples. Unfortunately, recent work shows that such exponential in $m$ dependence is unavoidable in the worst-case for any algorithm---there is an $\exp(\Omega(m))$ sample complexity lower bound for learning approximate Nash, even in \emph{one-step} general-sum games~\citep{chen2015well,rubinstein2016settling} (see Proposition \ref{theorem:rubinstein-formal} for formal statement). 


% This is indeed the case for existing algorithms such as Multi-Nash-VI~\citep{liu2021sharp} which achieves sample complexity $\wt{\mc{O}}(H^4S^2\prod_{i=1}^m A_i/\epsilon^2)$ for learning the $\epsilon$-approximate Nash equilibrium in general-sum MGs.



% \begin{proposition}[Lower bound for learning approximate Nash ~\citep{rubinstein2016settling}; {\color{red} Formal version deferred to Proposition}~\ref{theorem:rubinstein-formal}]
%   \label{proposition:rubinstein-informal}
%   There exists some absolute constant $\epsilon_0>0$ and a family of $m$-player general-sum Markov games for any $m$ with $H=1$, $S=1$, $A_i=2$, and \emph{deterministic} rewards, such that any algorithm that is able to find an $\epsilon_0$-approximate Nash equilibrium with high probability must at least play $2^{\Omega(m)}$ samples (episodes). % % ~\yub{shorten}
%   %\sm{degrade it to a proposition or a lemma?}
% \end{proposition}

This suggests that the Nash equilibrium as a solution concept may be too hard to learn efficiently for MGs with a large number of players, and calls for alternative solution concepts or additional structural assumptions on the game in order to achieve an improved $m$ dependence.


% Proposition~\ref{proposition:rubinstein-informal} shows that learning $\epsilon_0$-approximate Nash already requires $2^{\Omega(m)}$ samples for some $\epsilon_0=\Theta(1)$. 

% \yub{Intuitively, joint action space has size $\exp(m)$, and therefore naive learning algorithms such as enumerating all joint actions has to pay exp in m samples. It turns out that such exp in m dependence is actually unavoidable, as is shown in the following seminal result of rubinstein...}


% Even in this case, with $m$ players, and $A_i=2$, with noiseless payoff query, there is still $2^{\Omega(m)}$ query complexity lower bound for finding $\epsilon$-Nash with $\epsilon$ being some small constant. It follows directly the sample complexity for computing $\epsilon$-approximate Nash equilibrium is exponential with respect to $m$ in general-sum Markov games. This matches the known lower bound $\widetilde O(H^4S^2  \prod_{i=1}^m A_i)$ in \cite{liu2021sharp}.

% In fact, this exponential dependence is almost inevitable if we want to learn a general-sum Markov games. In order to get rid of the exponential dependence, we need to consider other notions of solution or consider general-sum Markov games with some structures. In other words, Nash equilibrium in general-sum Markov games is too general to learn efficiently.



==> Sections/intro.tex <==
\section{Introduction}

Multi-agent reinforcement learning (RL) has achieved substantial recent successes in solving artificial intelligence challenges such as GO~\citep{silver2016mastering,silver2018general}, multi-player games with team play such as Starcraft~\citep{vinyals2019grandmaster} and Dota2~\citep{berner2019dota}, behavior learning in social interactions~\citep{baker2019emergent}, and economic simulation~\citep{zheng2020ai,trott2021building}. In many applications, multi-agent RL is able to yield high quality policies for multi-player games with a large number of players~\citep{wang2016display, yang2018mean}. 


% \yub{Empirical success of multi-agent RL... alphago... starcraft... emergent tool use... deepmind or openai newest paper...} 

Despite these empirical progresses, theoretical understanding of when we can sample-efficiently solve multi-player games with a large number of players remains elusive, especially in the setting of multi-player Markov games. A main bottleneck here is the \emph{exponential blow-up} of the \emph{joint action space}---The total number of joint actions in a generic game with simultaneous plays is equal to the product of the number of actions for each player, which scales exponentially in the number of players. Such an exponential dependence is indeed known to be unavoidable in the worst-case for certain standard problems. For example, for learning an approximate Nash equilibrium from payoff queries in an one-step multi-player general-sum game, the query complexity lower bound of~\citet{chen2015well} and \citet{rubinstein2016settling} shows that at least exponentially many queries (samples) is required, even when each player only has two possible actions and the query is noiseless. Moreover, for learning Nash equilibrium in Markov games, the best existing sample complexity upper bound also scales with the size of the joint action space~\citep{liu2021sharp}.


Nevertheless, these exponential lower bounds do not completely rule out interesting theoretical inquiries---there may well be other notions of equilibria or additional structures within the game that allow us to learn with a better sample complexity. This motivates us to ask the following
\begin{quote}
    {\bf Question}: When can we solve general-sum Markov games with sample complexity milder than exponential in the number of players?
\end{quote}
This paper makes steps towards answering the above question by considering multi-player general-sum Markov games (MGs) with $m$ players, $H$ steps, $S$ states, and $A_i$ actions per player. We make two lines of investigations: (1) Can we learn alternative notions of equilibria with better sample complexity than learning Nash; (2) Can the Nash equilibrium be learned with better sample complexity under additional structural assumptions on the game. This paper makes contributions on both ends, which we summarize as follows.
\begin{itemize}[leftmargin=2em, topsep=0pt]
    \item We first design an algorithm that learns the $\eps$-approximate Coarse Correlated Equilibrium (CCE) with $\tO(H^5S\max_{i\in[m]} A_i / \eps^2)$ episodes of play (Section~\ref{section:cce}). Our algorithm \multiv~is a multi-player adaptation of the Nash V-Learning algorithm of~\citet{bai2020near}.
    % combined with a certified correlated policy technique for outputting a policy that approximate CCE.
    
    \item We design an algorithm \cev~which learns the stricter notion of $\eps$-approximate Correlated Equilibrium (CE) with $\tO(H^6S\max_{i\in[m]} A_i^2 / \eps^2)$ episodes of play (Section~\ref{section:ce}). For Markov games, these are the first line of sample complexity results for learning CE and CCE that only scales polynomially with $\max_{i\in[m]} A_i$, and improves significantly in the $A_i$ dependency over the current best algorithm which scales with $\prod_{i\in[m]} A_i$.
    
    \item Technically, our algorithm \cev~makes several major modifications over \multiv~in order to learn the CE (Section~\ref{section:ce-techniques}). Notably, inspired by the connection between CE and \emph{low swap-regret} learning, we use a mixed-expert Follow-The-Regularized Leader algorithm within its inner loop to achieve low swap-regret for a particular adversarial bandit problem. Our analysis also contains new results for adversarial bandits on weighted swap regret and weighted regret with predicable weights, which may be of independent interest.
    
    \item Finally, we consider learning Nash equilibrium in \emph{Markov Potential Games} (MPGs), an important subclass of general-sum Markov games. By a reduction to single-agent RL, we design an algorithm \nashca~that achieves $\tO(\Phi_{\max} H^3S\sum_{i\in[m]} A_i / \epsilon^3)$ sample complexity, 
    where $\Phi_{\max}\le Hm$ is the bound on the potential function (Section~\ref{sec:MPG}). Compared with the recent result of~\citet{leonardos2021global}, we significantly improves the $\eps$ dependence from their $1/\eps^6$.
    % This significantly improves over the existing algorithm ~\yub{cite} which requires $\wt{O}(1/\epsilon^6)$ samples, and is better than the ~\yub{Nash-VI which does not require assumptions on the game but pays $\prod A_i$}.
    
    % Our algorithm builds on ~\yub{ascent on potential function...}
    
    
    
    % \item We present a lower bound of $\Omega(H^2 \sum A_i / \epsilon^2)$ for learning pure-strategy Nash in MPGs, when $A_i$ are all equal. The dependence on $A_i$ improves over the naive $\max A_i$ obtained by a reduction from MPGs to single-player Markov Decision Processes.~\yub{compared with our upper bound (which also guarantees to output pure-strategy Nash) we are tight in $A_i$ dependency but there is a gap in $\epsilon$.}
\end{itemize}

==> Sections/preliminary.tex <==
\section{Preliminaries}\label{sec:preliminaries}
%\begin{itemize}
%    \item Markov games
%     \item Policy
%     \item Non-Markov policy
%     \item Nash
%     \item pure Nash
% \end{itemize}

% We consider multi-player general-sum Markov games. In such games, there are many players. Unlike multi-agent reinforcement learning, 

We present preliminaries for multi-player general-sum Markov games as well as the solution concept of (approximate) Nash equilibrium. Alternative solution concepts and other concrete subclasses of Markov games considered in this paper will be defined in the later sections.

\paragraph{Markov games}
A multi-player general sum Markov game (MG;~\citet{shapley1953stochastic,littman1994markov}) with $m$ players can be described by a tuple $\text{MG}(H, \mathcal{S},\left\{\mathcal{A}_{i}\right\}_{i=1}^{m}, \mathbb{P},\left\{r_{i}\right\}_{i=1}^{m})$, where $H$ is the episode length, $\mc{S}$ is the state space with $|\mc{S}|=S$, $\mc{A}_i$ is the action space for the \ith player with $|\mc{A}_i|=A_i$. Without loss of generality, we assume $\mc{A}_i=[A_i]$. We let $\bm{a}\defeq (a_1,\cdots,a_m)$ denote the vector of joint actions taken by all the players and $\mc{A}=\mc{A}_1\times\cdots\times\mc{A}_m$ denote the joint action space. Throughout this paper we assume that $S$ and $A_i$ are finite. The transition probability $\P=\{\P_h\}_{h\in[H]}$ is the collection of transition matrices, where $\P_h(\cdot|s,\bm{a})\in \Delta_{\mc{S}}$ denotes the distribution of the next state when actions $\bm{a}$ are taken at state $s$ at step $h$. The rewards $r_i=\{r_{h,i}\}_{h\in[H],i\in[m]}$ is the collection of reward functions for the \ith player, where $r_{h,i}(s,\bm{a})\in[0,1]$ gives the deterministic\footnote{Our results can be straightforwardly generalized to Markov games with stochastic rewards.} reward of \ith player if actions $\bm{a}$ are taken at state $s$ at step $h$. Without loss of generality, we assume the initial state $s_1$ is deterministic. A key feature of general-sum games is that the rewards $r_i$ are in general different for each player $i$, and the goal of each player is to maximize her own cumulative reward. 

% For any $n\in\mathbb{N}$, $[n]\defeq\{1,2,\cdots,n\}$. 
% ~\yub{note : this is def of product policy.} 

% \paragraph{Policy, value function}
% A product policy is a collection of $m$ policies $\pi\defeq \{\pi_i\}_{i\in[m]}$, where $\pi_i=\{\pi_{h,i}: (\mc{S} \times \mc{A})^{h-1} \times \mc{S} \to \Delta_{\mc{A}_i}\}_{h\in[H]}$, and $\pi_{h,i}(a_i|s)$ is the probability for the \ith player to take action $a_i$ at state $s$ at step $h$. For a policy $\pi$ and $i\in[m]$, we use $\pi_{-i} \defeq \set{\pi_j}_{j\in[m],j\neq i}$ to denote the policy of all but the \ith player. The value function $V^{\pi}_{h,i}(s):\mc{S}\to \mathbb{R}$ is defined as the expected cumulative reward for the \ith player when policy $\pi$ is taken starting from state $s$ and step $h$:
% \begin{align}
% \label{equation:def-value-function}
%     V^{\pi}_{h,i}(s)\defeq \E_{\pi}\brac{\sum_{h'=h}^H r_{h',i}(s_{h'},\bm{a}_{h'}) \Bigg| s_h=s}.
% \end{align}
% % gives the expected cumulative rewards received by \ith player. 
% The Q-value function $Q_h^\pi:\mc{S}\times\mc{A}\to \mathbb{R}$ is defined similarly as the expected cumulative rewards received by the \ith player starting from state-action pair $(s,\bm{a})$ and step $h$:
% \begin{align}\label{equation:def-Q-function}
%     Q^{\pi}_{h,i}(s,\bm{a})\defeq \E_{\pi}\brac{\sum_{h'=h}^H r_{h',i}(s_{h'},\bm{a}_{h'}) \Bigg| s_h=s,\bm{a}_h=\bm{a}}.
% \end{align}
% For convenience of notation, we define operators $\P_h$ and $\mathbb{D}_\pi$: For any value function $V$ and any action-value function $Q$, 
% \begin{align*}
%     [\P_hV](s,\bm{a})\defeq \E_{s'\sim\P_h(\cdot|s,\bm{a})}V(s'),\quad
%     [\mathbb{D}_\pi Q] (s)\defeq \E_{\bm{a}\sim\pi(\cdot|s)} Q(s,\bm{a}).
% \end{align*}
% From these definitions, we have the Bellman equations
% \begin{align*}
%     Q_{h,i}^\pi(s,\bm{a})=(r_{h,i}+\P_h V_{h+1,i}^\pi)(s,\bm{a}),\quad
%     V_{h,i}^\pi(s) = (\mathbb{D}_{\pi_h}Q_{h,i}^\pi )(s)
% \end{align*}
% for all $(i,s,\bm{a},h)\in[m]\times\mc{S}\times\mc{A}\times[H]$ (where we have set $V_{H+1,i}^\pi(s)=0$ for all $h,i\in[H]\times[m]$).



% Last version Oct 5
\paragraph{Markov product policy, value function}
A product policy is a collection of $m$ policies $\pi\defeq \{\pi_i\}_{i\in[m]}$ where $\pi_i$ is the general (potentially history-dependent) policy for the $i$-th player. We first focus on the case of Markov product policies, in which $\pi_i=\{\pi_{h,i}:\mc{S}\to \Delta_{\mc{A}_i}\}_{h\in[H]}$, and $\pi_{h,i}(a_i|s)$ is the probability for the \ith player to take action $a_i$ at state $s$ at step $h$. For a policy $\pi$ and $i\in[m]$, we use $\pi_{-i} \defeq \set{\pi_j}_{j\in[m],j\neq i}$ to denote the policy of all but the \ith player. The value function $V^{\pi}_{h,i}(s):\mc{S}\to \mathbb{R}$ is defined as the expected cumulative reward for the \ith player when policy $\pi$ is taken starting from state $s$ and step $h$:
\begin{align}
\label{equation:def-value-function}
    V^{\pi}_{h,i}(s)\defeq \E_{\pi}\brac{\sum_{h'=h}^H r_{h',i}(s_{h'},\bm{a}_{h'}) \Bigg| s_h=s}.
\end{align}
%Definition of the Q function and Bellman equations can be found in Appendix~\ref{appendix:bellman}. 


% gives the expected cumulative rewards received by \ith player. 







% In multi-player games, because different player may receive different reward, it may be impossible for all player to get the maximal rewards. In game theory, a well-studied notion of solution of multi-player games is Nash equilibrium.~\yub{I am here.}

\paragraph{Best response \& Nash equilibrium} 
For any product policy $\pi=\set{\pi_i}_{i\in[m]}$, the \emph{best response}~for the \ith player against $\pi_{-i}$ is defined as any policy $\pi^\dagger$ such that $V_{1,i}^{\pi^\dagger,\pi_{-i}}(s_1)=\sup_{\pi'_i}V_{1,i}^{\pi'_i,\pi_{-i}}(s_1)$. For any Markov product policy, this best response is guaranteed to exist (and be Markov) as the above maximization problem is equivalent to solving a Markov Decision Process (MDP) for the \ith player. We will also use the notation $V_{1,i}^{\dagger, \pi_{-i}}(s_1)$ to denote the above value function $V_{1,i}^{\pi^\dagger,\pi_{-i}}(s_1)$.

% \ziang{Existence of Nash}~\yub{Nash 1951 only shows existence for one-step games?}~\yub{dagger notation?}

% We view Nash equilibrium as the optimal policy in a multi-player general-sum Markov games. To measure the suboptimality, we introduce
% \ziang{maximum$\to$sum, discussion} 

We say $\pi$ is a \emph{Nash equilibrium} (e.g.~\citet{nash1951non,perolat2017learning}) if all players play the best response against other players, i.e., for all $i\in[m]$,
\begin{align*}
    V_{1,i}^{\pi}(s_1)=V_{1,i}^{\dagger,\pi_{-i}}(s_1) .
\end{align*}
Note that in general-sum MGs, there may exist multiple Nash equilibrium policies with different value functions, unlike in two-player zero-sum MGs~\citep{shapley1953stochastic}. To measure the suboptimality of any policy $\pi$, we define the \NEgap~as
\begin{align*}
    \NEgap(\pi)\defeq \max_{i\in[m]}\brac{\sup_{\mu_i}V_{1,i}^{\mu_i,\pi_{-i}}(s_1)- V_{1,i}^{\pi}(s_1)}.
\end{align*}
For any $\epsilon\ge 0$, we say $\pi$ is $\epsilon$-approximate Nash equilibrium ($\eps$-Nash) if $\NEgap(\pi)\le \epsilon$.

% A Nash equilibrium $\pi$ is a policy $\pi$ such that $\NEgap(\pi)=0$. Moreover, 

% Policy can be deterministic or stochastic. $\pi$ is deterministic

% \paragraph{Pure-strategy Nash equilibrium}
% We say policy $\pi$ is a pure strategy (deterministic policy) if and only if for any $(h,i,s)\in[H]\times[m]\times\mc{S}$, $\pi_{h,i}(a_i|s)=\mathbb{I}_{a_i=a'_{h,i}(s)}$ for some $a_{h,i}'(s)$. We say $\pi$ a \emph{pure-strategy Nash equilibrium} if $\pi$ is a pure-strategy and is a Nash equilibrium. Similarly, we say $\pi$ is a pure-strategy $\epsilon$-approximate Nash equilibrium if $\pi$ is a pure strategy and $\NEgap(\pi)\le \epsilon$. Pure-strategy Nash equilibrium does not always exist in general-sum MGs, but is guaranteed to exist (as we will see) in special subclasses of MGs such as Markov Potential Games.

\paragraph{General correlated policy \& Its best response} 
A general correlated policy $\pi$ is a set of $H$ maps $\pi \defeq \{\pi_{h}: \Omega \times(\mc{S}\times \mc{A} )^{h-1}\times \mc{S}\to\Delta_{\mc{A}} \}_{h\in[H]}$. The first argument of $\pi_h$ is a random variable $\omega \in \Omega$ sampled from some underlying distribution, and the other arguments contain all the history information and the current state information (unlike Markov policies in which the policies only depend on the current state information). The output of $\pi_h$ is a general distribution of actions in $\mc{A} = \mc{A}_1\times\cdots\times\mc{A}_m$ (unlike product policies in which the action distribution is a product distribution). %The random variable $\omega$ is sampled from some underlying distribution. %which may be shared among all steps $h\in[H]$. 

For any correlated policy $\pi = \{ \pi_h \}_{h \in [H]}$ and any player $i$, we can define a marginal policy $\pi_{-i}$ as a set of $H$ maps $\pi_{-i} \defeq \{\pi_{h,-i}: \Omega \times(\mc{S}\times \mc{A})^{h-1}\times \mc{S}\to\Delta_{\mc{A}_{-i}} \}_{h\in[H]}$ where $\mc{A}_{-i} \defeq \mc{A}_1\times\cdots\times\mc{A}_{i-1}\times\mc{A}_{i+1}\times\cdots\times\mc{A}_{m}$, and the output of $\pi_{h,-i}$ is defined as the marginal distribution of the output of $\pi_{h}$ restricted to the space $\mc{A}_{-i}$. 
For any general correlated policy $\pi$, we can define its initial state value function $V_{1,i}^\pi(s_1)$ similar as~\eqref{equation:def-value-function}. The best response value of the \ith player against $\pi$ is $V^{\dagger,\pi_{-i}}_{1,i}(s_1)=\sup_{\mu_i}V^{\mu_i,\pi_{-i}}_{1,i}(s_1)$,
where $V^{\mu_i,\pi_{-i}}_{1,i}(s_1)$ is the value function of the policy $(\mu_i, \pi_{-i})$ (the \ith player plays according to general policy $\mu_i$, and all other players play according to $\pi_{-i}$), and the supremum is taken over all general policy $\mu_i$ of the \ith player. 


%Given a general policy of the \ith player %$\mu_i = \{\mu_{i, h}: \mathbb{R} \times(\mc{S}\times \mc{A}\times\mathbb{R})^{h-1}\times \mc{S}\to\Delta_{\mc{A}_i} \}_{h\in[H]}$ with random variable $z_i$ (that is independent of $z$ in the correlated policy $\pi$) as the first argument of $\mu_{i,h}$, 
%we can define the value functions of the policy $(\mu_i, \pi_{-i})$ as 
%\[
%V^{\mu_i,\pi_{-i}}_{1,i}(s_1) \defeq \E_{z, z_i} \brac{\E_{a_{h, i} \sim \mu_{i, h}, \bm{a}_{h, -i} \sim \pi_{h, -i}}\brac{\sum_{h'=1}^H r_{h',i}(s_{h'},(a_{h, i}, \bm{a}_{h', -i})}}.
%\]




% but with an additional expectation with respect to the random variable $z$. 
% \[
% V^{\pi}_{1,i}(s_1)\defeq \E_z\brac{\E_{\bm{a}_h \sim \pi_h}\brac{\sum_{h'=1}^H r_{h',i}(s_{h'},\bm{a}_{h'})}}.
% \]


%Since general policies depend on the full history, the definitions of their value functions of later steps and the Q functions are subtle, and we will define them later whenever necessary. 

%\ziang{the randomness of $\pi_{-i}$ }.\yub{say that value at step 1 is well-defined} \yub{define its marginal $\pi_{-i}$} \yub{define BR using value at step 1.}\ziang{$\surd$}


\paragraph{Learning setting}
Throughout this paper we consider the interactive learning (i.e. exploration) setting where algorithms are able to play episodes within the MG and observe the realized transitions and rewards. Our focus is on the PAC sample complexity (i.e. number of episodes of play) for any learning algorithm to output an approximate equilibrium.

==> Sections/related_work.tex <==
\subsection{Related work}
% \ziang{at least all the papers mentioned are added into bib}

\paragraph{Learning equilibria in general-sum games}
The sample (query) complexity of learning Nash, CE, and CCE from samples in \emph{one-step} (i.e. normal form) general-sum games with $m$ players and $A_i$ actions per player has been studied extensively in literature~\citep{hart2000simple,hart2005adaptive,stoltz2005incomplete,cesa2006prediction,blum2007external,fearnley2015learning,babichenko2015query,chen2015well,fearnley2016finding,goldberg2016bounds,babichenko2016query,rubinstein2016settling,hart2018query}. It is known that learning Nash equilibrium requires exponential in $m$ samples in the worst case~\citep{rubinstein2016settling}, whereas CE and CCE admit efficient ${\rm poly}(m, \max_{i\le m}A_i)$-sample complexity algorithms by independent no-regret learning~\citep{hart2000simple,hart2005adaptive,syrgkanis2015fast,goldberg2016bounds,chen2020hedging,daskalakis2021near}. Our results for learning CE and CCE can be seen as extension of these works into Markov games. We remark that even when the game is fully known, the computational complexity for finding Nash in general-sum games is PPAD-hard~\citep{daskalakis2013complexity}.

% Learning Nash. Lower bounds: Cheng yu et al., 2015, Rubenstein et al. 2016. Other upper bounds from game-theory community. Different query models (e.g. algorithms under full information. computational PPAD hardness by Costis et al which shows even 2-player general-sum Nash is PPAD complete. noiseless payoff query, noisy payoff query).
% \yub{no need to mention PPAD in main paper?}

%\ziang{\cite{babichenko2015query} gives exponential (in m) (lower bound) number of querys for CE for deterministic algorithm}

% Other solution concepts: CCE, CE. (Find some sample complexity results). CCE is known to only depends on summation of action space (Bounds for the Query Complexity of Approximate Equilibria, Goldberg and Roth 2014), our first part of result can be viewed as extension of this into Markov games. \yub{Noah Golowich new paper on fast convergence to CCE of general-sum matrix games via no-regret learning, and reference therein.} \yub{TODO: Check Goldberg and Roth to see whether they need $\sum A_i$ or $\max A_i$ queries.}\ziang{$\sum A_i$}

% \paragraph{Multi-player General-sum Matrix Games / Normal-form games / strategic games}
% For the complexity of computing Nash equilibrium in normal form games.  \cite{daskalakis2013complexity} shows that
% computing Nash in two-player general-sum games is PPAD-complete. Recently,  \cite{chen2015well}, \cite{babichenko2016query},  \cite{rubinstein2016settling} established query complexity lower bound with exponential dependency on the number of players.

% For Coarse Correlated Equilibrium (CCE), empirical plays of no-regret learning is known to converge to CCE \citep{hart2000simple,hannan20164,goldberg2016bounds,daskalakis2021near}. But negative results indicate that it fails to learn Nash in general-sum games \citep{viossat2013no,flokas2020no}. Our first part of result can be viewed as extension of this into Markov games.


\paragraph{Markov games}
Markov games~\citep{shapley1953stochastic,littman1994markov} is a widely used framework for game playing with sequential decision making, e.g. in multi-agent reinforcement learning. Algorithms with asymptotic convergence have been proposed in the early works of~\citet{hu2003nash,littman2001friend,hansen2013strategy}. A recent line of work studies the non-asymptotic sample complexity for learning Nash in two-player zero-sum Markov games \citep{bai2020provable,xie2020learning,bai2020near,zhang2020model,liu2021sharp,chen2021almost,jin2021power,huang2021towards} and learning various equilibria in general-sum Markov games~\citep{liu2021sharp,bai2021sample}, building on techniques for learning single-agent Markov Decision Processes sample-efficiently~\citep{azar2017minimax,jin2018q}. Learning the Nash equilibrium in general-sum Markov games are much harder than that in zero-sum Markov games. \citet{liu2021sharp}~present the first line of results for learning Nash, CE, and CCE in general-sum Markov games; however their sample complexity scales with $\prod_{i\le m}A_i$ due to the model-based nature of their algorithm. Algorithms for computing CE in extensive-form games has been widely studied \citep{von2008extensive,celli2020no,farina2021simple,morrill2021efficient}, though we remark Markov games and extensive-form games are different frameworks and our results do not imply each other.


\paragraph{Markov potential games}
Lastly, a recent line of works considers Markov potential games~\citep{macua2018learning,leonardos2021global, zhang2021gradient}, a subset of general-sum Markov games in which the Nash equilibrium admits more efficient algorithms. \cite{leonardos2021global} gives a sample-efficient algorithm based on the policy gradient method \citep{agarwal2021theory}. The special case of Markov cooperative games is studied empirically in e.g.~\cite{lowe2017multi,yu2021surprising}. For one step potential games, \citet{kleinberg2009multiplicative,palaiopanos2017multiplicative,cohen2017learning} show the convergence to Nash equilibria of no-regret dynamics. 






% \paragraph{Markov Games}
% Formulation (Shapley 1953), and early algorithms (Nash Q-learning). Recently a line of RL results tackle two-player zero-sum Markov Games. \yub{mention these works build on the techniques of solving single-agent MDP sample-efficiently, e.g. Azar et al., Jin et al.} Zero-sum games rely BLAH which fails to hold in general-sum games.

% General-sum Markov games is studied in (Liu et al. 2020) which shows BLAH. 

% Markov potential games.~\yub{Li Na and Panageas et al., and others, and Macua et al.}

% \yub{What term should we use for "matrix" general-sum game?}

% \yub{Provably Efficient Cooperative Multi-Agent Reinforcement Learning with Function Approximation.}

% % \paragraph{Extensive-form games}

% % We briefly remark the convergence / complexity of solving multi-player general-sum games is also studied in the framework of extensive-form games~\yub{cite a lot of papers}. 

% % \yub{cite neurips best paper, or one or two more on extensive form games.} We note that these results are incomparable (and do not imply) sharp results for MGs since they assume tree structure + incomplete information, whereas MGs do not have tree stucture.~\yub{just say why extensive-form games do not translate to sharp results for MGs since you need to pay full tree size}

==> Sections_arxiv/algorithm.tex <==
\section{Simplified version Algorithm 1 with theoretical guarantee}

If we consider a simplified version of algorithm \ref{algorithm:nash_v_adv}, i.e. the update rule is \begin{align*}
    \text{If } n\in\mathcal{L}, \text{ then } 
    \up{V}_h(s_h) \setto \frac{\check{v}}{\check{n}}+\bar{b},
\end{align*}
we can prove that this algorithm achieve regret bound $\mathcal{O}(H^5S(A+B)K)$.

\yub{switch to using V-OL algorithm of Tiancheng et al.?}


\begin{lemma} For each update time, the following inequality holds with high probability, where $\check{k}_i$ represent the index of the ith visit at s at the h-th step in this stage
\begin{align*}
    \max_\mu \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu\times\nu_h^{\check{k}_i}}\left(r_h + \mathbb{P}_h\up{V}_{h+1}^{\check{k}_i}\right)(s)&-
    \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \left[r_h\left(s,a_h^{\check{k}_i},b_h^{\check{k}_i}\right) + \up{V}_{h+1}^{\check{k}_i}\left(s_{h+1}^{\check{k}_i}\right)\right]\\
    &\le c\sqrt{\frac{2H^2 A\iota}{\check{n}}}.
\end{align*} 
\end{lemma}
\begin{proof-of-lemma}[1]
First, by Azuma-Hoeffding, 
\begin{align*}
    \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu_h^{\check{k}_i}\times\nu_h^{\check{k}_i}}\left(r_h + \mathbb{P}_h\up{V}_{h+1}^{\check{k}_i}\right)(s)&-
    \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \left[r_h\left(s,a_h^{\check{k}_i},b_h^{\check{k}_i}\right) + \up{V}_{h+1}^{\check{k}_i}\left(s_{h+1}^{\check{k}_i}\right)\right]\\
    &\le 2\sqrt{\frac{2H^2 \iota}{\check{n}}}.
\end{align*}
To bound $$R_{\check{n}}=\max_\mu \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu\times\nu_h^{\check{k}_i}}\left(r_h + \mathbb{P}_h\up{V}_{h+1}^{\check{k}_i}\right)(s)-\sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu_h^{\check{k}_i}\times\nu_h^{\check{k}_i}}\left(r_h + \mathbb{P}_h\up{V}_{h+1}^{\check{k}_i}\right)(s)
,$$ we use the bandit lemma in [\cite{}], then we have
\begin{align*}
    R_{\check{n}}/H&\le 2\frac{1}{\check{n}}\sqrt{A\check{n}\iota}+\frac{3\sqrt{A\iota}}{2}\sum_{i=1}^{\check{n}} \frac{1}{\check{n}\sqrt{i}}+\frac{1}{2}\frac{1}{\check{n}}\iota+\sqrt{2\iota\sum_{i=1}^{\check{n}} \frac{1}{\check{n}^2}}\\
    &=\mathcal{O}(\sqrt{\frac{A\iota}{\check{n}}}).
\end{align*}
Combining these two result together, we can get the desired result. Note that we can get a similar result for the min player.
\end{proof-of-lemma}
\begin{remark}
Every $\up{V}_h$ and $\underline{V}_h$ in this lemma should be considered as capped value (restricted in $[0,H-h+1]$).  
\end{remark}

\begin{lemma}
With high probability, the following two conclusions holds,
\begin{align*}
    \up{V}_h^k(s)\ge V_h^\star(s)\ge \underline{V}_h^k (s) \text{ for all } (s,h,k)\in\mathcal{S}\times[K]\times[H].
\end{align*}
\begin{align*}
    (1/K)\sum_{k=1}^K( \up{V}_h^k-\underline{V}_h^k )(s_1)\le \mathcal{O}(\sqrt{H^5S(A+B)\iota/K}).
\end{align*}
\end{lemma}
\begin{proof-of-lemma}[2]
The first claim can be proved by backward induction. First of all, we should always keep in mind that at each stage, $\up{V}_h^k(s), \underline{V}_h^k(s)$ is fixed. We only update them when a stage is over.  So at each stage, the value of  $\up{V}_h^k(s), \underline{V}_h^k(s)$ only depends on the last stage before this stage. The claim is true for $h=H+1$. Assume for any s, $\up{V}_{h+1}^k(s)\ge V_{h+1}^\star(s)\ge \underline{V}_{h+1}^k (s)$. For fixed $s$ and $k$, let $\check{n}$ be the number of s was visited at h-th step in last stage and the index of such time is $\check{k}_1,\dots,\check{k}_{\check{n}}$, By Bellman equation,
\begin{align*}
    V_h^\star(s)&=\max_\mu \min_\nu \mathbb{D}_{\mu\times\nu}\left(r_h + \mathbb{P}_h V_{h+1}^\star\right)(s)\\
    &=\max_\mu \sum_{i=1}^{\check{n}}\frac{1}{\check{n}}\min_\nu \mathbb{D}_{\mu\times\nu}\left(r_h + \mathbb{P}_h V_{h+1}^\star\right)(s)\\
    &\le \max_\mu \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu\times\nu_h^{\check{k}_i}}\left(r_h + \mathbb{P}_h V_{h+1}^\star\right)(s)\\
    &\le \max_\mu \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu\times\nu_h^{\check{k}_i}}\left(r_h + \mathbb{P}_h\up{V}_{h+1}^{\check{k}_i}\right)(s).
\end{align*}
Comparing with the last lemma, if we choose bonus $\up{\beta} = c\sqrt{H^2A\iota/\check{n}}$. We would have $\up{V}_h^k(s)\ge V_h^\star(s)$. Similarly, $\underline{\beta} = c\sqrt{H^2B\iota/\check{n}}$ gives $V_h^\star(s)\ge \underline{V}_h^k (s)$.

Finally, we are ready to prove the regret bound. Letting $\delta_h^k := \up{V}_h^k(s_h^k)-\underline{V}_h^k (s_h^k)$, $\check{n}_h^k$ be the number of $s_h^k$ was visited at h-th step in last stage and the index of such time is $\check{l}_h^1,\dots,\check{l}_h^{\check{n}_h^k}$ . $\check{n}_h^k=0$ if this is the first stage. By this algorithm, 
\begin{align*}
    \delta_h^k &= \up{V}_h^k(s_h^k)-\underline{V}_h^k (s_h^k)\\
    &= H\mathbf{1}_{\{\check{n}_h^k=0\}}+
    \sum_{i=1}^{\check{n}_h^k}\frac{1}{\check{n}_h^k}\paren{\up{V}_{h+1}^{\check{l}_h^i}(s_{h+1}^{\check{l}_h^i})-\underline{V}_{h+1}^{\check{l}_h^i}(s_{h+1}^{\check{l}_h^i})}+\up{\beta}_k-\underline{\beta}_k\\
    &\le H\mathbf{1}_{\{\check{n}_h^k=0\}}+
    \sum_{i=1}^{\check{n}_h^k}\frac{1}{\check{n}_h^k}\paren{\up{V}_{h+1}^{\check{l}_h^i}(s_{h+1}^{\check{l}_h^i})-\underline{V}_{h+1}^{\check{l}_h^i}(s_{h+1}^{\check{l}_h^i})}+ c\sqrt{\frac{H^2 (A+B)\iota }{\check{n}_h^k}}\mathbf{1}_{\{\check{n}_h^k>0\}}\\
    &=H\mathbf{1}_{\{\check{n}_h^k=0\}}+
    \sum_{i=1}^{\check{n}_h^k}\frac{1}{\check{n}_h^k}\delta_{h+1}^{\check{l}_h^i}+ c\sqrt{\frac{H^2 (A+B)\iota }{\check{n}_h^k}}\mathbf{1}_{\{\check{n}_h^k>0\}}.
\end{align*}

Taking the summation w.r.t. k, the first term is 
\begin{align*}
    \sum_{k=1}^K H\mathbf{1}_{\{\check{n}_h^k=0\}}\le HSe_1.
\end{align*}

The second term is 
\begin{align*}
    \sum_{k=1}^K \sum_{i=1}^{\check{n}_h^k}\frac{1}{\check{n}_h^k}\delta_{h+1}^{\check{l}_h^i}\le 
    \sum_{k=1}^K \delta_{h+1}^k(1+\frac{1}{H}).
\end{align*}
To get this inequality, we first exchange the order of summation, then we find that the coefficient of $\delta_{h+1}^k$ is contributed by the next stage's k. Because $e_{i+1}=\floor{(1+1/H)e_i}$, the coefficients are bounded by $1+\frac{1}{H}.$

The last term is 
\begin{align*}
    \sum_{k=1}^K c\sqrt{\frac{H^2 (A+B)\iota }{\check{n}_h^k}}\mathbf{1}_{\{\check{n}_h^k>0\}}
    &=c \sum_s\sum_{k:s_h^k = s}\sqrt{\frac{H^2 (A+B)\iota }{\check{n}_h^k}}\mathbf{1}_{\{\check{n}_h^k>0\}}\\
    &\le c(1+\frac{1}{H}) \sum_s \sum_{0<i<N_s^K}\sqrt{H^2(A+B)\iota e_i},
\end{align*}
where $N_s^K$ means till K, s is in its $N_s^K$-th stage at step h. When $N_s^K$ equal for all $s$, we attain maximum. So we can further derive
\begin{align*}
    \sum_{k=1}^K c\sqrt{\frac{H^2 (A+B)\iota }{\check{n}_h^k}}\mathbf{1}_{\{\check{n}_h^k>0\}}&\le
    \mathcal{O}(1)S\sum_{i=1}^{N}\sqrt{H^2(A+B)\iota e_i}\\&=\mathcal{O}(1)S\sqrt{H^2(A+B)\iota e_1}\frac{\sqrt{1+1/H}^N-1}{\sqrt{1+1/H}-1},
\end{align*}
where $$N \approx \frac{\log \paren{1+\frac{K}{SHe_1}}}{\log\paren{1+\frac{1}{H}}}.$$
After some calculation, we get
\begin{align*}
    \sum_{k=1}^K c\sqrt{\frac{H^2 (A+B)\iota }{\check{n}_h^k}}\mathbf{1}_{\{\check{n}_h^k>0\}}&\le \mathcal{O}(1)S\sqrt{H^2(A+B)\iota e_1}\mathcal{O}(H\sqrt{\frac{K}{SHe_1}})\\
    &=C\sqrt{H^3S(A+B)\iota K}
\end{align*}

So
\begin{align*}
    \sum_{k=1}^K \delta_h^k&\le HSe_1+(1+\frac{1}{H})\sum_{k=1}^K \delta_{h+1}^k+C\sqrt{H^3S(A+B)\iota K})\\
    &=SH^2+(1+\frac{1}{H})\sum_{k=1}^K \delta_{h+1}^k+C\sqrt{H^3S(A+B)\iota K}).
\end{align*}
If $K\to \infty$, this gives
$$
(1/K)\sum_{k=1}^K( \up{V}_h^k-\underline{V}_h^k )(s_1)\le \mathcal{O}(\sqrt{H^5S(A+B)\iota/K}).
$$
\end{proof-of-lemma}

We can define certified policies (Algorithm \ref{algorithm:certified policy})to extract a policy afer playing. This policy can achieve sample complexity $\mathcal{O}(H^5S(A+B)/\epsilon^2)$ and the algorithm is model-free.

\begin{algorithm}[t]
% \setstretch{1.2}
   \caption{Certified policy}
   \label{algorithm:certified policy}
   \begin{algorithmic}[1]
      \STATE sample k $\setto$ Uniform([K]).
      \FOR{step $h=1,\dots,H$}
      \STATE observe $s_h$, and set $t\setto \check{n}_h^k(s_h)$.
      \STATE sample $m\in[t]$ with $\P(m=i) = 1/t$.
      \STATE $k\setto \check{l}_t^i(s_h)$.
      \STATE take action $a_h\sim \mu_h^k(\cdot|s_h)$.
      \ENDFOR
   \end{algorithmic}
\end{algorithm}

\section{Discussion on Sample Complexity Lower Bound of Finding Approximate Nash Equilibrium in General-Sum Markov Games}
In this section, we investigate the query complexity for computing Nash or approximate Nash in bimatrix games. 

\subsection{Sample complexity upper bound}

\subsection{Lower bound of query complexity in general-sum games}
\begin{theorem}
There exists a general sum Markov games M=\text{MG}$(H,\mc{S},\{\mc{A}_i\}_{i=1}^m,\mathbb{P},\{r_i\}_{i=1}^m)$ and two positive number $epsilon$ and c such that: for any algorithm, after $2^{\Omega(m/\log m)}$ episodes, with probability at least $p=1-2^{-cm/\log m}$, the algorithm failed to output a $\epsilon$-Nash equilibrium.
\end{theorem}
\yub{Cite Rubinstein 16 and Cheng Yu et al. 15}.

\begin{lemma}
There exists two constant $\epsilon>0$ and $c>0$ such that:

$$
\text{QC}_p(\text{ANE}(m,\epsilon))=2^{\Omega(m/\log m)}, \text{ where } p=2^{-cm/\log m}.
$$
\end{lemma}
Even in this case, with $m$ players, and $A_i=2$, with noiseless payoff query, there is still $2^{\Omega(m)}$ query complexity lower bound for finding $\epsilon$-Nash with $\epsilon$ being some small constant. 

\section{Approximate CCE for General Sum Markov Games}
In this section, we present an algorithm which can find CCE for general sum markov games in $\tilde O(H^5 S \sum_{i=1}^m A_i /\epsilon^2)$ episodes.
\begin{algorithm}[t]
% \setstretch{1.2}
   \caption{Nash-V-Learning for the i-th player}
   \label{algorithm:nash_v_general}
   \begin{algorithmic}[1]
      \STATE {\bfseries Initialize:} For any $(s, a, h)$, set $\up{V}_{h,i}(s)\setto H$, $\underline{V}_{h,i}(s)\setto 0$, $\up{L}_{h,i}\setto 0$, $\mu_h(a|s) \setto 1/A_i$, $N_h(s)\setto 0$.
      \FOR{episode $k=1,\dots,K$}
      \STATE Receive $s_1$.
      \FOR{step $h=1,\dots, H$}
      \STATE Take action $a_h \sim \mu_h(\cdot |s_h)$, observe the action $a'_h$ from the other players.
      \STATE Observe reward $r_h=r_h(s_h, a_h, a'_h)$ and next state $s_{h+1}$ from the environment.
      \STATE Update accumulators: $t\defeq N_{h}(s_h)\setto N_{h}(s_h) + 1$.
      \STATE $\up{V}_{h,i}\left(s_{h}\right) \setto  \left(1-\alpha_{t}\right) \bar{V}_{h,i}\left(s_{h}\right)+\alpha_{t}\left(r_{h,i}\left(s_{h}, a_{h}, a'_{h}\right)+\bar{V}_{h+1,i}\left(s_{h+1}\right)+\bar{\beta}_{t}\right)$
      \STATE $\underline{V}_{h,i}\left(s_{h}\right) \setto  \left(1-\alpha_{t}\right) \underline{V}_{h,i}\left(s_{h}\right)+\alpha_{t}\left(r_{h,i}\left(s_{h}, a_{h}, a'_{h}\right)+\underline{V}_{h+1,i}\left(s_{h+1}\right)-\bar{\beta}_{t}\right)$
      \FOR{all $a \in \mc{A}_i$}
      \STATE $\up{\ell}_{h,i}(s_h, a) \setto [H - r_{h,i}-\min\{\up{V}_{h+1,i}(s_{h+1}),H-h\}] \mathbb{I}\{a_h=a\}/[\mu_h(a_h|s_{h}) +\up{\eta}_{t}]$.
      \STATE $\up{L}_{h,i}(s_h,a)\setto (1-\alpha_t)\up{L_{h,i}}(s_h,a)+\alpha_t\up{L}_{h,i}(s_h,a)$
      % \STATE $\up{L}_h( s_h, a)  \setto ( 1-\alpha _t )\up{L}_h( s_h,a ) +\alpha_t \up{\ell}_h(s_h, a)$.
      \ENDFOR
      \STATE Set $\mu_h(\cdot |s_h) \propto \exp[-(\up{\eta}_t/\alpha_t) \up{L}_{h,i}( s_h, \cdot)]$.
      \ENDFOR
      \ENDFOR
   \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
% \setstretch{1.2}
   \caption{Certified policy $\hat\pi$ for general-sum Markov games}
   \label{certified_policy_general}
   \begin{algorithmic}[1]
      \STATE sample $k$ $\setto$ Uniform([K]).
      \FOR{step $h=1,\dots,H$}
      \STATE observe $s_h$, and set $t\setto N_h^k(s_h)$.
      \STATE sample $l\in[t]$ with $\P(l=j) = \alpha_t^j$.
      \STATE $k\setto k_t^l(s_h)$.
      \STATE jointly take action $(a_{h,1}, a_{h,2},\dots,a_{h,m})\sim \prod_{i=1}^m\mu_{h,i}^k(\cdot|s_h)$.
      \ENDFOR
   \end{algorithmic}
\end{algorithm}

We choose all hyperparameters as follows, for some large constant $c$, and log factors $\iota$.
\begin{align*}
    \alpha_{t}=\frac{H+1}{H+t}, \quad \eta_{t}=\sqrt{\frac{H\log A_i}{A_i t}}, \quad \bar{\beta}_{t}=c \sqrt{\frac{H^{3} A_i \iota}{t}}.
\end{align*}
Value function of certified policy can be decomposed as 
$$
V^{\hat\pi}_{1,i}(s) = \frac{1}{K}\sum_{k=1}^K V^{\hat\pi^k}_{1,i}(s),
$$
where the decomposition is due to the first line in the algorithm: sample $k\setto $Uniform([K]).

After running  Algorithm \ref{algorithm:nash_v_general} for all $m$ players and Algorithm \ref{certified_policy_general}, we can learn a certified policy $\hat\pi$. Then,
\begin{theorem}\label{proof_general_cce}
With probability at least $1-p$, if we run Algorithm \ref{algorithm:nash_v_general} for all $m$ players and Algorithm \ref{certified_policy_general} for $K$ episodes with 
$$
K\ge \Omega(H^5 S \max_{i\in[m]}A_i \iota /\epsilon^2),
$$
then the certified policy $\hat\pi$ will be $\epsilon$-approximate CCE, i.e. $V_{1,i}^{\dagger,\hat\pi_{-i}}(s)- V_{1,i}^{\hat\pi} (s)\le \epsilon$ for all $i=1,2,\dots,m$ and $s\in \mc{S}$.
\end{theorem}

Before proving Theorem \ref{proof_general_cce}, there's a simple consequence of the update rule in Algorithm \ref{algorithm:nash_v_general}, which will be used several times later. To simplify the notation, we omit index $i$ which represent the i-th player.
\begin{lemma}
Let $t=N_h^k(s)$ and suppose s was previously visited at episodes $k^1,\dots,k^t<k$ at the h-th step. The update rule in Algorithm \ref{algorithm:nash_v_general} is equivalent to the following equations.
\begin{align}
    \up{V}_{h}^{k}(s)&=\alpha_{t}^{0} H+\sum_{j=1}^{t} \alpha_{t}^{j}\left[r_{h}\left(s, a_{h}^{k^{j}}, {a'}_{h}^{k^{j}}\right)+\up{V}_{h+1}^{k^{j}}\left(s_{h+1}^{k^{j}}\right)+\bar{\beta}_{j}\right]\\
    \underline{V}_{h}^{k}(s)&=\sum_{j=1}^{t} \alpha_{t}^{j}\left[r_{h}\left(s, a_{h}^{k_{h}^{j}}, {a'}_{h}^{k_{h}^{j}}\right)+\underline{V}_{h+1}^{k_{h}^{j}}\left(s_{h+1}^{k_{h}^{j}}\right)-\up{\beta}_{j}\right]
\end{align}
\end{lemma}

\begin{lemma}
\label{bandit_lemma_general}
Let $t=N_h^k(s)$ and suppose s was previously visited at episodes $k^1,\dots,k^t<k$ at the h-th step. With probability $1-\frac{p}{2m}$, for any $(s,h,t)\in\mc{S}\times[H]\times[K]$, there exist a constant c s.t.

\begin{gather*}
    \max _{\mu} \sum_{j=1}^{t} \alpha_{t}^{j} \mathbb{D}_{\mu \times \mu_{h,-i}^{k^{j}}}\left(r_{h}+\mathbb{P}_{h} \min\{\up{V}_{h+1,i}(s_{h+1}),H-h\}\right)(s)\\-\sum_{j=1}^{t} \alpha_{t}^{j}\left[r_{h}\left(s, a_{h}^{k^{j}}, b_{h}^{k^{j}}\right)+\min\{\up{V}_{h+1,i}(s_{h+1}),H-h\}\left(s_{h+1}^{k^{i}}\right)\right] \leq c \sqrt{2 H^{3} A \iota / t}
\end{gather*}

\end{lemma}
\begin{proof-of-lemma}[\ref{bandit_lemma_general}]
The proof consists of two parts, the first one is applying Azuma-Hoeffding inequality and another is (\red{slight stronger}) adversarial bandit lemma.
\end{proof-of-lemma}
\begin{remark}
The inequality in Lemma \ref{bandit_lemma_general} holds with probability $1-p/2m$. Take a union bound, we can conclude that the inequality holds for all the player with probability $1-p/2$.
\end{remark}

\begin{lemma}
\label{key-lemma-general}
If the inequality in Lemma \ref{bandit_lemma_general} holds for all m players, then we have
\begin{align*}
    \up{V}_{h,i}^k(s)\ge V_{h,i}^{\dagger,\hat\pi_{-i}^k}(s),\quad
    \underline{V}_{h,i}^k(s)\le V_{h,i}^{\hat\pi^k}(s)
\end{align*}
for all $[k,h,s]\in [K]\times[H]\times\mc{S}$ with probability at least $1-p/2$.
\end{lemma}
\begin{proof-of-lemma}[\ref{key-lemma-general}]
We proof the first claim by backward induction. The claim is true for $h = H + 1$. Suppose the claim is true for $h+1$.
We begin with $V_{h,i}^{\dagger,\hat\pi_{-i}^k}(s)$, by the definition of certified policy, letting $t = N_h^k(s)$, we have
\begin{align*}
    V_{h,i}^{\dagger,\hat\pi_{-i}^k}(s) &= \sup_{\mu_i}\mathbb{D}_{\mu_i\times\hat\pi_{-i}^k} [r_{h,i}+\mathbb{P}_h V_{h+1,i}^{\dagger,\hat\pi_{-i}^k}](s)\\
    &=\sup_{\mu_i}\sum_{j=1}^t \alpha_t^j \mathbb{D}_{\mu_i\times\mu_{h,-i}^{k^j}}[r_{h,i}+\mathbb{P}_h V_{h+1,i}^{\dagger,\hat\pi_{-i}^k}](s)\\
    &\le \sup_{\mu_i}\sum_{j=1}^t \alpha_t^j \mathbb{D}_{\mu_i\times\mu_{h,-i}^{k^j}}[r_{h,i}+\mathbb{P}_h \min\{\up{V}_{h+1,i}(s_{h+1}),H-h\}](s)\\
    &\le\sum_{j=1}^{t} \alpha_{t}^{j}\left[r_{h}\left(s, a_{h}^{k^{j}}, b_{h}^{k^{j}}\right)+\min\{\up{V}_{h+1,i}(s_{h+1}),H-h\}\left(s_{h+1}^{k^{i}}\right)\right] + c \sqrt{2 H^{3} A \iota / t}\\
    &\le \sum_{j=1}^{t} \alpha_{t}^{j}\left[r_{h}\left(s, a_{h}^{k^{j}}, b_{h}^{k^{j}}\right)+\min\{\up{V}_{h+1,i}(s_{h+1}),H-h\}\left(s_{h+1}^{k^{i}}\right)+\up{\beta}_j\right]\\
    &= \up{V}_{h,i}^k(s).
\end{align*}
Here, the first inequality is due to induction hypothesis and bounded value function. For the last inequality, we use $\frac{1}{\sqrt{t}} \leq \sum_{i=1}^{t} \frac{\alpha_{t}^{i}}{\sqrt{i}} \leq \frac{2}{\sqrt{t}}$. So if we choose $\up{\beta}_t = c\sqrt{\frac{H^3 A_i \iota}{t}}$ for large $c$, the inequality holds. 
Meanwhile, by the definition of certified policy, 
\begin{align*}
    V_{h,i}^{\hat\pi^k}(s) &= \sum_{j=1}^t \alpha_t^j \mathbb{D}_{\pi^{k^j}}[r_h+\mathbb{P}_h V_{h+1,i}^{\hat\pi^{k^j}}](s)\\
    &\ge \sum_{j=1}^t \alpha_t^j \mathbb{D}_{\pi^{k^j}}[r_h+\mathbb{P}_h \underline{V}^{k^j}_{h+1,i}](s).
\end{align*}
So by Azuma-Hoeffding inequality, with probability at least $1-\frac{p}{2SKH}$
\begin{align*}
    \sum_{j=1}^t \alpha_t^j \mathbb{D}_{\pi^{k^j}}[r_h+\mathbb{P}_h \underline{V}^{k^j}_{h+1,i}](s)&\ge \sum_{j=1}^{t} \alpha_{t}^{j}\left[r_{h}\left(s, a_{h}^{k_{h}^{j}}, {a'}_{h}^{k_{h}^{j}}\right)+\underline{V}_{h+1}^{k_{h}^{j}}\left(s_{h+1}^{k_{h}^{j}}\right)\right] -\sqrt{\frac{H^3 A_i\iota}{t}}\\
    &\ge\sum_{j=1}^{t} \alpha_{t}^{j}\left[r_{h}\left(s, a_{h}^{k_{h}^{j}}, {a'}_{h}^{k_{h}^{j}}\right)+\underline{V}_{h+1}^{k_{h}^{j}}\left(s_{h+1}^{k_{h}^{j}}\right)-\up{\beta}_{j}\right]\\
    & = \underline{V}^{k^j}_{h,i}(s).
\end{align*}
Taking a union bound, then Lemma \ref{key-lemma-general} is proved by induction.
\end{proof-of-lemma}

Equipped with these lemmas, we are ready to prove Theorem \ref{proof_general_cce}. 

\begin{proof-of-theorem}[\ref{proof_general_cce}]
Suppose Lemma \ref{bandit_lemma_general} and Lemma \ref{key-lemma-general} all hold (this happens with probability at least $1-p$), then 
\begin{align*}
    V_{1,i}^{\dagger,\hat\pi^k_{-i}}(s_1)- V_{1,i}^{\hat\pi^k} (s_1)\le \up{V}_{1,i}^k(s_1)-\underline{V}_{1,i}^k(s_1).
\end{align*}
So we have
\begin{align*}
     V_{1,i}^{\dagger,\hat\pi_{-i}}(s_1)- V_{1,i}^{\hat\pi} (s_1)
     \le&\frac{1}{K} \sum_{k=1}^K\left( V_{1,i}^{\dagger,\hat\pi^k_{-i}}(s_1)- V_{1,i}^{\hat\pi^k} (s_1)\right)\\
     \le& \frac{1}{K} \sum_{k=1}^K\left(\up{V}_{1,i}^k(s_1)-\underline{V}_{1,i}^k(s_1)\right) .
\end{align*}

Letting $\delta_{h,i}^k := \up{V}_{h,i}^k(s_h^k)-\underline{V}_{h,i}^k (s_h^k)$ and $t=N_h^k(s)$. By the update rule, 
\begin{align*}
    \delta_{h,i}^k &= \up{V}_{h,i}^k(s_h^k)-\underline{V}_{h,i}^k (s_h^k)\\
    &= \alpha^0_t H + \sum_{j=1}^t \alpha_t^j [\up{V}_{h+1,i}^k(s_{h+1}^{k^j})-\underline{V}_{h+1,i}^k(s_{h+1}^{k^j})+2\up{\beta_j}]\\
    &= \alpha_t^0H +\sum_{j=1}^t\alpha_t^j \delta_{h+1,i}^{k^j}+\sum_{j=1}^t 2\alpha_t^j\up{\beta}_j\\
    &\le \alpha_t^0H +\sum_{j=1}^t\alpha_t^j \delta_{h+1,i}^{k^j}+ 2c\sqrt{\frac{A_iH^3\iota}{t}}
\end{align*}

Taking the summation w.r.t. k, by the same argument in Nash V learning, we can get 
\begin{align*}
    &\frac{1}{K} \sum_{k=1}^K\left(\up{V}_{1,i}^k(s_1)-\underline{V}_{1,i}^k(s_1)\right) =\frac{1}{K} \sum_{k=1}^K \delta_{h,i}^k\\
    \le& eSH^2/K+ \mathcal{O}\left(\sqrt{H^{5} S\max_{i\in[m]} A_i \iota/K}\right).
\end{align*}
This complete the proof of Theorem \ref{proof_general_cce} because when $K\to\infty$, $\sqrt{H^{5} S\max_{i\in[m]} A_i \iota/K}$ is the dominant term.
\end{proof-of-theorem}


% \section{Difficulties in Finding Approximate Nash Equilibrium in General-Sum Markov Games}
% \subsection{Query complexity with noiseless payoff query}



% \subsection{Computation complexity}
% \subsection{No-regret learning}
% \subsection{Sub-linear regret and last iteration convergence}

\section{Efficient Algorithm to Compute pure $\epsilon$ Nash in Markov Potential Games}
%With the setting in [Li Na's <Gradient Play...>]. For softmax parameterization:
% \begin{align*}
%     \pi_{i,\theta_i}(a_i|s)=\frac{\exp \theta_{s,a_i}}{\sum_{a_j\in\mc{A}_i}\exp \theta_{s,a_j}}.
% \end{align*}
% Since this is a differentiable parameterization that explicitly constrains $\pi_\theta(\cdot|s)$ to be in the simplex, then we have
% \begin{align*}
%     \nabla_{\theta} \mathbb{E}_{s_{0} \sim \rho} V_{i}^{\theta}\left(s_{0}\right)=\frac{1}{1-\gamma} \mathbb{E}_{s \sim d_{\theta}} \mathbb{E}_{a \sim \pi_{\theta}(\cdot | s)}\left[\nabla_{\theta} \log \pi_{\theta}(a \mid s) A_{i}^{\theta}(s, a)\right], \quad i=1,2, \ldots, n.
% \end{align*}
% Moreover, we have
% \begin{align*}
%     \frac{\partial \log \pi_{\theta}\left(a^{\prime} | s^{\prime}\right)}{\partial \theta_{s, a_{i}}}=\frac{\partial \log \pi_{\theta_{i}}\left(a_{i}^{\prime} | s^{\prime}\right)}{\partial \theta_{s, a_{i}}} &=\textbf{1}\left\{ s^{\prime}=s\right\} \paren{\textbf{1}\{a'=a\}-\pi_{\theta_i}(a_i|s)}\\
% &=\textbf{1}\left\{a_{i}^{\prime}=a_{i}, s^{\prime}=s\right\} -\textbf{1}\{s'=s\}\pi_{\theta_i}(a_i|s).
% \end{align*}
% So we can prove that
% \begin{lemma}
% $$\frac{\partial J_i(\theta)}{\partial \theta_{s,a_i}} =\frac{1}{1-\gamma} d_\theta(s)\pi_{\theta_i}(a_i|s) \up{A_i^\theta}(s,a_i). $$
% Moreover, if this is a Markov Potential Game(MPG) with potential function $\Phi$, then
% $$
% \frac{\partial \Phi (\theta)}{\partial \theta_{s,a_i}}=\frac{\partial J_i(\theta)}{\partial \theta_{s,a_i}} =\frac{1}{1-\gamma} d_\theta(s)\pi_{\theta_i}(a_i|s) \up{A_i^\theta}(s,a_i). 
% $$
% \end{lemma}
% Another important lemma is the \textbf{Performance difference lemma}:
% \begin{align*}
%     J_{i}\left(\theta^{\prime}\right)-J_{i}(\theta)=\frac{1}{1-\gamma} \mathbb{E}_{s \sim d_{\theta^{\prime}}} \mathbb{E}_{a \sim \pi_{\theta^{\prime}}} A_{i}^{\theta}(s, a), \quad i=1,2, \ldots, n.
% \end{align*}

% The NPG algorithm defines a Fisher information matrix
% (induced by $\pi$), and performs gradient updates in the geometry induced by this matrix as follows:
% \begin{align*}
%     \begin{array}{l}
% F_{\rho}(\theta)=\mathbb{E}_{s \sim d_\theta(\cdot)} \mathbb{E}_{a \sim \pi_{\theta}(\cdot| s)}\left[\nabla_{\theta} \log \pi_{\theta}(a | s)\left(\nabla_{\theta} \log \pi_{\theta}(a | s)\right)^{\top}\right] \\
% \theta^{(t+1)}=\theta^{(t)}+\eta F_{\rho}\left(\theta^{(t)}\right)^{\dagger} \nabla_{\theta} \Phi(\theta^{(t)}).
% \end{array}
% \end{align*}

% In multi-player case, this update rule doesn't have a convenient form.(?)

% Alternatively, we can consider another update rule. In each step, we perform NPG update for each single player (fix other players' policy) simultaneously ,i.e.
% \begin{align*}
%     \pi_i^{(t+1)}(a_i | s)=\pi_i^{(t)}(a_i | s) \frac{\exp \left(\eta \up{A_i^{\theta^{(t)}}}(s, a_i) /(1-\gamma)\right)}{Z_{i,t}(s)}, \quad i=1,2, \ldots, n.
% \end{align*}
% By performance difference lemma, 
% $$
% J_{i}\left(\theta_{i}^{\prime}, \theta_{-i}\right)-J_{i}\left(\theta_{i}, \theta_{-i}\right)=\frac{1}{1-\gamma} \sum_{s, a_{i}} d_{\theta^{\prime}}(s) \pi_{\theta_{i}^{\prime}}\left(a_{i} \mid s\right) \overline{A_{i}^{\theta}}\left(s, a_{i}\right),
% $$
% it's not difficult to get
% $$
% J_i(\theta_i^{(t+1)},\theta_{-i}^{(t)})-
% J_i(\theta_i^{(t)},\theta_{-i}^{(t)})\ge
% \frac{1-\gamma}{\eta}\mathbb{E}_{s_0\sim\rho}\log Z_{i,t}(s_0)\ge 0.
% $$
% By the definition of MPG, this becomes
% $$
% \Phi(\theta_i^{(t+1)},\theta_{-i}^{(t)})-
% \Phi(\theta_i^{(t)},\theta_{-i}^{(t)})\ge
% \frac{1-\gamma}{\eta}\mathbb{E}_{s_0\sim\rho}\log Z_{i,t}(s_0)\ge 0
% $$

% If we update each player's policy sequentially, we can get a coordinate ascent algorithm for $\Phi$.
% By performance difference lemma, 
% \begin{align*}
%   J_{i}\left(\theta_{i}^*, \theta_{-i}\right)-J_{i}\left(\theta_{i}, \theta_{-i}\right)
%   &=\frac{1}{1-\gamma} \sum_{s, a_{i}} d_{\theta^*}(s) \pi_{\theta_{i}^*}\left(a_{i} \mid s\right) \overline{A_{i}^{\theta}}\left(s, a_{i}\right) 
% \end{align*}

\yub{For the definition, we only need $V_1$. By the example we have seen (cite), this is much weaker than per-step, per-state potential game assumption.}


%\subsection{Algorithm with iteration complexity $\frac{Cn(\Phi_{\text{max}}-\Phi_{\text{min}})}{(1-\gamma)^2\epsilon^2}$}

\begin{algorithm}[t]
% \setstretch{1.2}
   \caption{Best response for general-sum Markov potential games}
   \label{algorithm:BR_general}
   \begin{algorithmic}[1]
   \REQUIRE Error tolerance $\epsilon$
      \WHILE{true}
      \STATE $\Delta,j,\{\hat\pi_j(\cdot|s)\}_{s\in\mc{S}}=$ \textbf{Estimate\_NE-Gap($\pi,\epsilon/8 $)}
      \IF{$\Delta>\epsilon/2$}
      \STATE update $\pi_j(\cdot|s)\setto \hat\pi_j(\cdot|s)$ for all $s\in\mc{S}$
      \ELSE 
      \STATE output $\pi$
      \STATE break
      \ENDIF
      \ENDWHILE
   \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
% \setstretch{1.2}
   \caption{Estimate\_NE-Gap($\pi,\delta$)}
   \label{algorithm:NEgap}
   \begin{algorithmic}[1]
      \FOR{player $i=1,\dots,n$}
      \STATE fix $\pi_{-i}$, run UCBVI-UPLOW   for i-th player with $K=\mc{O}(\frac{H^3SA_i\iota}{\delta^2})$ times and get a new policy $\hat\pi_i$
      \STATE Simulate the MDP with policy $\hat{\pi}_i,\pi_{-i}$ for $N=\frac{CH^2\iota}{\delta^2}$ times and get $\hat V_{1,i}(\hat\pi_i,\pi_{-i})$, which is an unbiased estimator of $V_{1,i}((\hat\pi_i,\pi_{-i}))$
      \STATE then we get $\Delta_i=\hat V_{1,i}(\hat\pi_i,\pi_{-i})-\hat V_{1,i}(\pi)$
      \ENDFOR
      \STATE $j\setto \arg\max_{i\in[n]} {\Delta_i}$
      \RETURN $\Delta_j,j,\hat\pi_j$
   \end{algorithmic}
\end{algorithm}
%\paragraph{Analysis:}
%For Algorithm \ref{NPG_general}, each time we update the policy, we have
%$$
%\Phi(\hat\pi_i,\pi_{-i})-\Phi(\pi) = J_i(\hat\pi_i,\pi_{-i})-J_i(\pi)\ge \epsilon/2 .
%$$
%So there are at most $2(\Phi_{\text{max}}-\Phi_{\text{min}})/\epsilon$ times update. On the other hand, if $\Delta\le\epsilon/2$, we have for all $i\in[n]$,
%\begin{align*}
%    J_i(\pi_i^*,\pi_{-i})-J_i(\pi)&=J_i(\pi_i^*,\pi_{-i})-J_i(\hat\pi_i,\pi_{-i})+J_i(\hat\pi_i,\pi_{-i})-J_i(\pi)\\
%    &\le \epsilon/2+\epsilon/2 .
%\end{align*}
%The inequality follows from the convergence rate of NPG and $\Delta\le\epsilon/2$.

%Overall, we need $\frac{2n(\Phi_{\text{max}}-\Phi_{\text{min}})}{\epsilon}$ times NPG, each NPG iterate $T=\frac{4}{(1-\gamma)^2\epsilon}$ times.

%\paragraph{Sample complexity:} While NPG update in subroutine gives a low iteration complexity, we can replace NPG with any other algorithm.

\subsection{Sample Complexity}
The overall sample complexity would be
$$
\mc{O}\paren{\frac{(\Phi_\text{max}-\Phi_\text{min})H^3S\sum_{i=1}^m A_i}{\epsilon^3}}. 
$$
Moreover, this algorithm is computation efficient. 

\yub{In this algorithm, use UCBVI-UPLOW to output a pure strategy. But mention that any efficient RL algorithm also works in principle, we only use this because it gives a pure strategy with high probability.}

\begin{theorem}\label{theorem:sample_complexity_general-sum}
For any $p\in(0,1]$, letting $\iota = \log(\frac{S\max_{1\le i\le m} A_i m}{\epsilon p})$, then with probability at least $1-p$, after at most 
$$
\mc{O}(\frac{(\Phi_\text{max}-\Phi_\text{min})H^3S\sum_{i=1}^m A_i \iota}{\epsilon^3})
$$
episodes, Algorithm \ref{BR_general} outputs a $\epsilon$-Nash pure policy $\hat\pi$.
\end{theorem}

\begin{lemma}
\label{lemma:NEgap}
For Algorithm \ref{NEgap}, with $\iota=\log(\frac{S\max_{1\le i\le m} A_i m}{\epsilon p})$, the output $\Delta_j,j,\hat\pi_j$ satisfied
$$
|V_{1,j}(\hat\pi_j,\pi_{-j})-V_{1,j}(\pi)- \Delta_j|\le2\delta, \quad
\max_{\pi_j}V_{1,j}(\pi_j,\pi_{-j})-V_{1,j}(\hat\pi_j,\pi_{-j})\le \delta
$$
with probability at least $1-\frac{p\epsilon}{4m}$.
\end{lemma}
\begin{proof-of-lemma}[\ref{lemma_NEgap}]
For the execution of UCBVI-UPLOW, it return a $\delta$-optimal pure policy with probability at least $1-\frac{p\epsilon}{8m^2}$. For the unbiased estimator $\hat V_{1,j}$, it's bounded by $H$. Thus by Hoeffding inequality,
$$
\mathbb{P}(|\hat V_{1,j}-V_{1,j}|\ge \delta)\le2\exp(-\frac{c\delta^2}{H^2 N}) 
$$
for some absolute constant $c$. For $N=CH^2/\delta^2\iota$ for some large constant $C$, we have
$$
|\hat V_{1,j}-V_{1,j}|\le \delta \quad \text{with probability at least }\quad 1-\frac{p\epsilon}{16m^2}.
$$
As a result, with probability at least $1-\frac{p\epsilon}{4m}$, for any $i\in[m]$,
\begin{equation}\label{equation:NE-gap_acuracy}
 \begin{gathered}
\max_{\pi_j}V_{1,j}(\pi_j,\pi_{-j})-V_{1,j}(\hat\pi_j,\pi_{-j})\le \delta\\
|\hat V_{1,j}(\hat\pi_j,\pi_{-j})-V_{1,j}(\hat\pi_j,\pi_{-j})|\le \delta\\
|\hat V_{1,j}(\pi)-V_{1,j}(\pi_j)|\le \delta.
\end{gathered}   
\end{equation}

By definition, $\Delta_j=\hat V_{1,j}(\hat\pi_j,\pi_{-j})-\hat V_{1,j}(\pi)$, so we must have
$$
|V_{1,j}(\hat\pi_j,\pi_{-j})-V_{1,j}(\pi)- \Delta_j|\le2\delta, \quad
\max_{\pi_j}V_{1,j}(\pi_j,\pi_{-j})-V_{1,j}(\hat\pi_j,\pi_{-j})\le \delta.
$$
This finishes the proof of this lemma.
\end{proof-of-lemma}
\begin{proof-of-theorem}[\ref{sample_complexity_general-sum}] 
First, we would prove that Estimate\_NE-Gap would be called for at most $\frac{4(\Phi_\text{max}-\Phi_\text{min})}{\epsilon}$ times. Suppose Lemma \ref{lemma_NEgap} holds for the first $4m/\epsilon$ calls. By Lemma \ref{lemma_NEgap}, this is true with probability at least $1-p$. When $\Delta_j>\epsilon/2$, by the definition of MPG
\begin{align*}
    \Phi(\hat\pi_j,\pi_{-j})-\Phi(\pi) &= V_{1,j}(\hat\pi_j,\pi_{-j})-V_{1,j}(\pi)\\
    &\ge \Delta_j-2\epsilon/8\\
    &\ge \epsilon/4.
\end{align*}
Note that $\frac{4(\Phi_\text{max}-\Phi_\text{min})}{\epsilon}\le \frac{4m}{\epsilon}$. This means there are at most $\frac{4(\Phi_\text{max}-\Phi_\text{min})}{\epsilon}$ calls for  Estimate\_NE-Gap with probability $1-p$. After that, algorithm would stop. When the algorithm stops, by \ref{equation:NE-gap_acuracy}, for any $i\in[m]$
\begin{align*}
\max_{\pi_i}V_{1,i}(\pi_i,\pi_{-i})-V_{1,i}(\pi)&=\max_{\pi_j}V_{1,i}(\pi_i,\pi_{-i})-V_{1,i}(\hat\pi_i,\pi_{-i})+V_{1,i}(\hat\pi_i,\pi_{-i})-V_{1,i}(\pi)\\
&\le \delta + V_{1,i}(\hat\pi_i,\pi_{-i})-V_{1,i}(\pi)\\
&\le \delta +2\delta+\Delta_j\\
&\le \epsilon.
\end{align*}
So Algorithm \ref{BR_general} outputs an $\epsilon$-Nash. Moreover, because UCBVI-UPLOW outputs a pure policy, the output of Algorithm \ref{BR_general} would also be a pure policy.

The sample complexity of Algorithm \ref{NEgap} is $\mc{O}(H^3S\sum A_i\iota/\epsilon^2+H^2m\iota/\epsilon^2)=\mc{O}(H^3S\sum A_i\iota/\epsilon^2)$. So the overall sample complexity is at most $\mc{O}(\frac{(\Phi_\text{max}-\Phi_\text{min})H^3S\sum_{i=1}^m A_i \iota}{\epsilon^3}).$ 



\end{proof-of-theorem}


\section{Lower bound of sample complexity for finding \red{pure} $\epsilon$-Nash Equilibrium}
$\mc{O}\paren{\frac{\sum_{i=1}^m A_i}{\epsilon^2}}$ for matrix games

$\mc{O}\paren{\frac{H^3 S \sum_{i=1}^m A_i}{\epsilon^2}}$ for MDP?
\subsection{General-sum stochastic matrix games}

\begin{theorem}\label{theorem:matrix_game_lowerbound}
Suppose $A_i\ge 2$, $i=1,\dots,m$ . Then, there exists an absolute constant $c_0$ such that for any $\epsilon\le\frac{1}{2m}$ and any online finetuning algorithm that outputs a \textbf{pure} strategy $\hat\pi=(\hat\pi_1,\dots,\hat\pi_m)$, if the number of samples 
$$n\le c_0 \frac{\sum_{i=1}^m A_i}{\epsilon^2},$$
then there exists a problem instance $M$ with stochastic payoff on which the algorithm suffers from $\epsilon/5$-suboptimality
$$
\mathbb{E}_M \text{NE-Gap}(\hat\pi)=\mathbb{E}_M\max_i\left[\max_{\pi_i}u_i^{(\pi_i,\hat\pi_{-i})}-u_i^{\hat\pi}\right]\ge\epsilon/5,
$$
where the expectation $\mathbb{E}_M$ is w.r.t. the randomness during the algorithm execution within game M.
\end{theorem}

We consider the following family of Bernoulli matrix games: : Let $\bm{a}=(a_1,a_2,\dots,a_m)$.
\begin{gather*}
  \mathfrak{M}(\epsilon)=\{\mc{M}^{\bm{a}^\star}\in\mathbb{R}^{A_1\times A_2\times\cdots\times A_m} \text{ with }\\ \mc{M}^{\bm{a}^\star}_{\bm{a}}=\frac{1}{2}+(\bm{1}\set{a_1^\star=a_1}+\cdot\bm{1}\set{a_1^\star=a_1\&a_2^\star=a_2}+\cdots+
  \bm{1}\set{a_1^\star=a_1\&a_2^\star=a_2\&\cdots\&a_m^\star=a_m})\epsilon:\\
  \bm{a}^\star\in [A_1]\times\cdots\times[A_m]
  \},  
\end{gather*}
where in matrix game $\mc{M}^{\bm{a}^\star}$, the reward is sampled from $\text{Bernoulli}(\mc{M}^{\bm{a}^\star}_{\bm{a}})$ if the i-th player picks $a_i$ where $\bm{a}=(a_1,a_2,\dots,a_m).$ Moreover, we define $\mc{M}^0$ as a game in  $\mathfrak{M}(0)$. Here, we assume the action space of the i-th player is $[A_i]=\{1,2,\cdots,A_i\}.$

We further let $\nu$ denote the uniform distribution on $[A_1]\times\cdots\times[A_m]$. 

\begin{proof-of-theorem}[\ref{theorem:matrix_game_lowerbound}]
Fix a matrix game $\mc{M}^{\bm{a}^\star}\in \mathfrak{M}(\epsilon)$, it's clear that the only Nash (pure) strategy is $\bm{a}^\star=(a_1^\star,a_2^\star,\cdots,a_m^\star)$. In other words, the i-th player's action should be $a_i^\star$. For any online finetuning algorithm $\mc{A}$ that outputs a pure strategy $\hat\pi$, suppose $\hat\pi$ means the i-th player's action is $\hat a_i$ and let $\bm{\hat a}=(\hat a_1,\hat a_2,\cdots,\hat a_m)$. From the structure of the $\mathfrak{M}(\epsilon)$, we know
\begin{align*}
    \text{NE-Gap}(\hat\pi)\ge \epsilon\P_{\bm{a}^\star}(\bm{\hat a} \not= \bm{a}^\star).
\end{align*}
So we only need to use $n$, the number of samples to give a lower bound of $\P_{\bm{a}^\star}(\bm{\hat a} \not= \bm{a}^\star)$ or $\P_{\bm{a}^\star}(\hat a_i \not= a_i^\star)$ 

Let $N(\bm{a})$ be the number of 1s when action $\bm{a}$ is taken. In fact, $\{N(\bm{a}):\bm{a}\in[A_1]\times\cdots\times[A_m]\}$ is a sufficient statistics for the posterior distribution $\bm{a}^\star$, so we have
\begin{align*}
    \E_{\bm{a}^\star\sim \nu}\P_{\bm{a}^\star}(\hat a_1\not= a^\star_1)&\ge\inf_g \E_{\bm{a}^\star\sim \nu}\P_{\bm{a}^\star}(\hat a_1\not= g_1\{N(\bm{a})\})\\
    &\overset{(i)}{\ge}
    \inf_g \E_{\bm{a}^\star\sim \nu}\P_0(\hat a_1\not= g_1\{N(\bm{a})\})
    -\E_{\bm{a}^\star\sim \nu}\text{TV}(\{N(\bm{a})\}|_{\P_0,\mc{A}},\{N(\bm{a})\}|_{\P_{\bm{a}^\star},\mc{A}})\\
    &\overset{(ii)}{\ge}
    \frac{1}{2}
    -\E_{\bm{a}^\star\sim \nu}\text{TV}(\{N(\bm{a})\}|_{\P_0,\mc{A}},\{N(\bm{a})\}|_{\P_{\bm{a}^\star},\mc{A}})\\
    &\overset{(iii)}{\ge}
    \frac{1}{2}
    -\E_{\bm{a}^\star\sim \nu}\sqrt{\frac{1}{2}\text{KL}(\{N(\bm{a})\}|_{\P_0,\mc{A}}\|\{N(\bm{a})\}|_{\P_{\bm{a}^\star},\mc{A}})}\\
    &\overset{(iv)}{=}\frac{1}{2}-\E_{\bm{a}^\star\sim \nu}\sqrt{\frac{1}{2}\sum_{\bm{a}} 
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    \text{KL}(\P_0(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}.
\end{align*}
Above, (i) follows from the definition of total variation distance; (ii) uses the fact that under $\mathbb{P}_0$, we can't get any information about $\bm{a}^\star$, so $\E_{\bm{a}^\star\sim \nu}\P_{\bm{a}^\star}(\bm{\hat a} \not= g\{N(\bm{a})\})=1-\frac{1}{A_1\cdots A_m}$; (iii) uses Pinsker’s inequality; (iv) uses KL divergence decomposition.
Define 
$$
d(\bm{a},\bm{a}^\star)=
\max\{i\in\mathbb{N},i\le m:\bm{a}_j=\bm{a}_j^\star \text{ for all } 1\le j\le i\},$$ where $\max \emptyset =0$. Apparently, $0\le d(\bm{a},\bm{a}^\star)\le m$. After introducing $d(\bm{a},\bm{a}^\star)$, the expected reward $\mc{M}^{\bm{a}^\star}_{\bm{a}}$ is equal to $\frac{1}{2}+d(\bm{a},\bm{a}^\star)\epsilon.$ For the KL divergence, we have
\begin{align*}
    \text{KL}(\P_0(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))
    =&\text{KL}\paren{\paren{\frac{1}{2},\frac{1}{2}}\|\paren{\frac{1}{2}-d(\bm{a},\bm{a}^\star)\epsilon,\frac{1}{2}+d(\bm{a},\bm{a}^\star)\epsilon}}\\
    =&\frac{1}{2}\log \frac{1}{1-4d^2(\bm{a},\bm{a}^\star)\epsilon^2}\\
    \le&4d^2(\bm{a},\bm{a}^\star)\epsilon^2
\end{align*}
for $\epsilon\le\frac{1}{2m}.$ Therefore,
\begin{align*}
    &\frac{1}{2}-\E_{\bm{a}^\star\sim \nu}\sqrt{\frac{1}{2}\sum_{\bm{a}} 
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    \text{KL}(\P_0(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}\\
    \overset{(i)}{\ge}&\frac{1}{2}-\sqrt{\frac{1}{2}\E_{\bm{a}^\star\sim \nu}\sum_{\bm{a}} 
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    \text{KL}(\P_0(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}\\
    = & \frac{1}{2}-\sqrt{\frac{1}{2}\E_{\bm{a}^\star\sim \nu}
    \sum_{k=0}^m\sum_{\bm{a}:d(\bm{a},\bm{a}^\star)=k} 
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    \text{KL}(\P_0(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}\\
    = & \frac{1}{2}-\sqrt{\frac{1}{2}
    \sum_{k=1}^m\E_{\bm{a}^\star\sim \nu}\sum_{\bm{a}:d(\bm{a},\bm{a}^\star)=k}
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    \text{KL}(\P_0(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}\\
    \overset{(ii)}{\ge} & \frac{1}{2}-\sqrt{2
    \sum_{k=1}^m\E_{\bm{a}^\star\sim \nu}\sum_{\bm{a}:d(\bm{a},\bm{a}^\star)=k}
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    k^2\epsilon^2}\\
    = & \frac{1}{2}-\sqrt{\frac{2}{A_1\cdots A_m}
    \sum_{\bm{a},\bm{a}^{\star}:d(\bm{a},\bm{a}^\star)>0}
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    d(\bm{a},\bm{a}^\star)^2\epsilon^2}\\
    = & \frac{1}{2}-\sqrt{\frac{2}{A_1\cdots A_m}
    \sum_{\bm{a}}
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    \sum_{\bm{a}^\star} d^2(\bm{a},\bm{a}^\star)\epsilon^2}\\
    \overset{(iii)}{\ge} & \frac{1}{2}-\sqrt{\frac{20}{A_1}
    \sum_{\bm{a}}
    \E_{\P_0,\mc{A}}[N(\bm{a})]
    \epsilon^2}\\
    =&\frac{1}{2}-\sqrt{\frac{20}{A_1}
    n
    \epsilon^2}
    % \overset{(iv)}{\ge}& \frac{1}{2}-\sqrt{\frac{40}{A_1}
    % \E_{\bm{a}^\star\sim \nu} \sum_{\bm{a}:a_1\not=a_1^\star}
    % \E_{\P_0,\mc{A}}[N(\bm{a})]
    % \epsilon^2}. 
\end{align*}
Above, (i) uses Jensen inequality; (ii) uses the KL divergence's upper bound that we derived. (iii) uses $\#\{\bm{a}^\star:d(\bm{a},\bm{a}^\star)=k\}=(A_{k+1}-1)\prod_{i=k+2}^{m}A_i$, so 
$$
\sum_{\bm{a}^\star}\frac{d^2(\bm{a},\bm{a}^\star)}{A_1\cdots A_m}\le
\sum_{k=1}^\infty \frac{k^2}{2^{k}}<10.
$$
%(iv) uses the fact that $\E_{\P_0,\mc{A}}[N(\bm{a})]$ is independent of $\bm{a}^\star$, so 
% $$
% \sum_{\bm{a}}\E_{\P_0,\mc{A}}[N(\bm{a})]=\frac{A_1}{A_1-1}\E_{\bm{a}^\star\sim \nu} \sum_{\bm{a}:a_1\not=a_1^\star}\E_{\P_0,\mc{A}}[N(\bm{a})].
% $$.
To summarize the argument, we proved that
\begin{align}
\label{equation:proof_lower_bound}
\E_{\bm{a}^\star\sim \nu}\P_{\bm{a}^\star}(\hat a_1 \not= a^\star_1)
\ge
\frac{1}{2}-\sqrt{\frac{20}{A_1}
    n
    \epsilon^2}.    
\end{align}
(\ref{proof_lower_bound}) tells us that if $n<\frac{A_1}{160\epsilon^2}$, we have
$$
\E_{\bm{a}^\star\sim \nu}\P_{\bm{a}^\star}(\hat a_1\not= a^\star_1)
\ge\frac{1}{4}.
$$
As a result, 
\begin{align*}
    \E_{\bm{a}^\star\sim \nu} \sum_{\bm{a}:\hat a_1\not= a^\star_1}
    \E_{\P_{\bm{a}^\star,\mc{A}}}N(a) &= \E_{\bm{a}^\star\sim \nu} \sum_{t=1}^n\P_{\bm{a}^\star}(\hat a_1\not= a^\star_1)\\
    &\ge \frac{n}{4}.
\end{align*}
To avoid $\epsilon/4$-sub-optimality, we must have $n\ge \frac{A_1}{160\epsilon^2}$, we still have
\begin{align}
\label{inequality:lowerbound1}
    \E_{\bm{a}^\star\sim \nu} \sum_{\bm{a}:\hat a_1\not= a^\star_1}
    \E_{\P_{\bm{a}^\star,\mc{A}}}N(a)
    \ge \frac{n}{4}\ge\frac{A_1}{640\epsilon^2}.
\end{align}
 
If we choose $\P_{\bm{a}^\star,k}$ as a base game, such that $\P_{\bm{a}^\star,k}$ and $\P_{\bm{a}^\star}$ only differ at $\bm{a}:d(\bm{a},\bm{a}^\star)> k$ where the reward of $\P_{\bm{a}^\star,k}$ is sampled from Bernoulli($\frac{1}{2}+k\epsilon$). Let $\bm{a}_{-k}$ denotes $(a_{k+1},\dots,a_m)$ and $\nu_{-k}$ denotes the uniform distribution on $[A_{k+1}],\dots,[A_m]$. Then fix $a^\star_1,\dots,a^\star_k$, by a similar argument, we can proved that to avoid $\epsilon/4$-sub-optimality for all game instance, we must have
\begin{align}
\label{inequality:lowerbound2}
    \E_{\bm{a}^\star_{-k}\sim \nu_{-k}} \sum_{\bm{a}:a_1=a^\star_1,\dots,a_k=a^\star_k,\hat a_{k+1}\not= a^\star_{k+1}}
    \E_{\P_{\bm{a}^\star,\mc{A}}}N(a)
    \ge\frac{A_{k+1}}{640\epsilon^2}.
\end{align}
Putting (\ref{inequality:lowerbound1}) and (\ref{inequality:lowerbound2}) together, to avoid $\epsilon/4$-sub-optimality, we must have 
\begin{align*}
    n&= \sum_{k=0}^{m-1}\E_{\bm{a}^\star\sim \nu}\sum_{\bm{a}:a_1=a^\star_1,\dots,a_k=a^\star_k,\hat a_{k+1}\not= a^\star_{k+1}}
    \E_{\P_{\bm{a}^\star,\mc{A}}}N(a)\\
    &\ge \frac{\sum_{i=1}^m A_i}{640\epsilon^2}.
\end{align*}
So we can choose $c_0$ as $\frac{1}{640}.$
\begin{align*}
    \E_{\bm{a}^\star_{-k}\sim \nu_{-k}}\P_{\bm{a}^\star}(\hat a_{k+1} \not= a_{k+1}^\star)&\ge\inf_g \E_{\bm{a}^\star_{-k}\sim \nu_{-k}}\P_{\bm{a}^\star}(\hat a_{k+1} \not= g_{k+1}\{N(\bm{a})\})\\
    &\ge\frac{1}{2}-\E_{\bm{a}^\star_{-k}\sim \nu_{-k}}\sqrt{\frac{1}{2}\sum_{\bm{a}} 
    \E_{\P_{\bm{a}^\star,k},\mc{A}}[N(\bm{a})]
    \text{KL}(\P_{\bm{a}^\star,k}(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}\\
    &\ge\frac{1}{2}-\sqrt{\frac{1}{2}\E_{\bm{a}^\star_{-k}\sim \nu_{-k}}\sum_{\bm{a}} 
    \E_{\P_{\bm{a}^\star,k},\mc{A}}[N(\bm{a})]
    \text{KL}(\P_{\bm{a}^\star,k}(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}\\
    &=  \frac{1}{2}-\sqrt{\frac{1}{2}\E_{\bm{a}^\star_{-k}\sim \nu_{-k}}
    \sum_{j=k+1}^m\sum_{\bm{a}:d(\bm{a},\bm{a}^\star)=j} 
    \E_{\P_{\bm{a}^\star,k},\mc{A}}[N(\bm{a})]
    \text{KL}(\P_{\bm{a}^\star,k}(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}\\
    &=  \frac{1}{2}-\sqrt{\frac{1}{2}
    \sum_{j=k+1}^m\E_{\bm{a}^\star_{-k}\sim \nu_{-k}}\sum_{\bm{a}:d(\bm{a},\bm{a}^\star)=j}
    \E_{\P_{\bm{a}^\star,k},\mc{A}}[N(\bm{a})]
    \text{KL}(\P_{\bm{a}^\star,k}(\cdot|\bm{a})\|\P_{\bm{a}^\star}(\cdot|\bm{a}))}\\
    &\ge\frac{1}{2}-\sqrt{2
    \sum_{j=k+1}^m\E_{\bm{a}^\star_{-k}\sim \nu_{-k}}\sum_{\bm{a}:d(\bm{a},\bm{a}^\star)=j}
    \E_{\P_{\bm{a}^\star,k},\mc{A}}[N(\bm{a})]
    (j-k)^2\epsilon^2}\\
     &= \frac{1}{2}-\sqrt{\frac{2}{A_{k+1}\cdots A_m}
    \sum_{\bm{a},\bm{a}^{\star}:d(\bm{a},\bm{a}^\star)>k}
    \E_{\P_{\bm{a}^\star,k},\mc{A}}[N(\bm{a})]
    (d(\bm{a},\bm{a}^\star)-k)^2\epsilon^2}\\
    &\ge \frac{1}{2}-\sqrt{\frac{20}{A_{k+1}}
    \sum_{\bm{a}:a_1=a_1^\star,\dots,a_k=a_k^\star}
    \E_{\P_{\bm{a}^\star,k},\mc{A}}[N(\bm{a})]
    \epsilon^2}. 
\end{align*}
 
\end{proof-of-theorem}


==> deprecated/CCE.tex <==
\section{Approximate CCE for General-Sum Markov Games}
\label{section:cce}

Motivated by~\yub{exp hardness...}, in this section, we consider whether alternative solution concepts can be learned without the exponential in $m$ sample complexity lower bound.~\yub{say that CE, CCE coincide with Nash in 2p0s, but are more general solution concepts in general-sum. copy some citation from Liu et al.}

In this section, we present an algorithm which can find CCE for general-sum markov games in $\tilde O(H^5 S \sum_{i=1}^m A_i /\epsilon^2)$ episodes. We first define CCE in general-sum Markov games.

% \begin{definition}[general (non-Markov) policy]
% A general (non-Markov) policy $\pi$ is a set of $Hm$ maps 
% $\pi \defeq \{\pi_{h,i}: 
% \mathbb{R} \times(\mc{S}\times \mc{A}\times \mc{B}\times\mathbb{R})^{h-1}\times \mc{S}\to\Delta_{\mc{A}_i}
% \}_{h\in[H],i\in[m]}$, from a random number $z\in \mathbb{R}$ and a history of length h to a distribution over actions in $\mc{A}$. The random number $z$ is sampled from some underlying distribution $\mc{D}$, but may be shared among all steps $h\in[H]$.\ziang{in preliminary, copied from V-learning}
% \end{definition}

\begin{definition}[general correlated policy]
A general correlated policy $\pi$ is an set of $H$ maps $\pi \defeq \{\pi_{h}: 
\mathbb{R} \times(\mc{S}\times \mc{A}\times\mathbb{R})^{h-1}\times \mc{S}\to\Delta_{\mc{A}}
\}_{h\in[H]}$, from a random number $z\in \mathbb{R}$ and a history of length h to a distribution over actions in $\mc{A}$, where $\mc{A}=\mc{A}_1\times\cdots\times\mc{A}_m$. The random number $z$ is sampled from some underlying distribution $\mc{D}$, but may be shared among all steps $h\in[H]$. 
\end{definition}
% \yub{move to prelim?}
%\ yub{remove $\mc{B}$, and move to preliminaries}



\begin{definition}[$\epsilon$-approximate CCE in Markov games]
We say a general correlated policy $\pi$ is an \emph{$\epsilon$-approximate Coarse Correlated Equilibrium (CCE)} if
$$
V_{1,i}^{\dagger,\pi_{-i}}(s_1)- V_{1,i}^{\pi} (s_1)\le \epsilon \quad\text{ for all } i=1,2,\dots,m
$$
where we use $\mu_i,\pi_{-i}$ to denote the policy that i-th player play policy $\mu_i$ and the other players play according to policy $\pi$. ~\yub{Assume deterministic $s_1$.}~\ziang{$\surd$}
And the best response is defined as 
$$
V_{1,i}^{\dagger,\pi_{-i}}(s_1)\defeq \sup_{\mu_i}V_{1,i}^{\mu_i,\pi_{-i}}(s_1).
$$
When $\epsilon=0$, $\pi$ is an coarse correlated equilibrium.
\end{definition}
To put it another way, CCE plays an role of a contract, if every player abide by this contract, then no player have motivation to change its policy. CCE always exists because Nash equilibrium is also a CCE. 

\subsection{Algorithm Description}
\yub{Change alg name to $V$-Learning.}
The algorithm is adapted from Nash V-learning~\citep{bai2020near,tian2021online}. There, Nash V-learning is proved to be a near optimal algorithm in learning $\epsilon$-approximate Nash equilibrium in zero-sum games with sample complexity $\widetilde O (H^6S\max\{A,B\})/\epsilon^2)$ , where $A,B$ is the number of actions of max-player and min-player. The output of Nash V-learning is a nested mixture of Markov policies. Here, we apply Nash V-learning in general-sum Markov games to learn $\epsilon$-approximate CCE. 

\paragraph{Nash V-learning}
In Algorithm \ref{algorithm:nash_v_general}, this part is almost the same with Nash V-learning.  \ziang{and move 
'min' to another place?} We choose all hyperparameters as follows, for some large constant $c$, and log factors $\iota=\log (\frac{K\max_{i\in[m]} A_i SH}{p\epsilon})$.
\begin{align*}
    \alpha_{t}=\frac{H+1}{H+t}, \quad \eta_{t}=\sqrt{\frac{H\log A_i}{A_i t}}, \quad \up{\beta}_{t}=c \sqrt{\frac{H^{3} A_i \iota}{t}}.
\end{align*}
These choices of stepsize %~\yub{choice of stepsize}\ziang{$\surd$} 
come from V-OL algorithm in \cite{tian2021online} which helps to shave off an $H$ factor in the sample complexity.~\yub{new choice of stepsize using $\iota$?}

% ~\yub{in the sample complexity}.

\paragraph{Certified policy} 
The certified policy is constructed on the history of Algorithm \ref{algorithm:nash_v_general}, i.e. $\{\mu_{h,i}^k\}$ and $\{s_h^k\}$ for $h,i,k\in[H]\times[m]\times[K]$. $N_h^k(s_h)$ refers to the times that $s_h$ is observed at step $h$ in the first $k$ episodes. $k_t^l(s_h)$ refers to the episodes index when $s_h$ is observed for the l-th time. $\alpha_t^j$ is defined as 
$$
\alpha_{t}^{0}:=\prod_{j=1}^{t}\left(1-\alpha_{j}\right), \alpha_{t}^{i}:=\alpha_{i} \prod_{j=i+1}^{t}\left(1-\alpha_{j}\right)
.$$
Note that we need all players use the same $k$ in certified policy, so $\hat\pi$ would be a correlated policy. This in different from Nash V-learning.


Nash V-learning use independent certified for max-player and min-player. In fact, V-learning enables players to perform no-regret learning. In zero-sum games, no-regret learning against another player's empirical policy is equivalent to no-regret learning against another player's certified policy. Thus Nash equilibrium can be learned. However, in general-sum games, though each player still learns policy in a no-regret learning manner, other player's empirical policy is related to certified correlated policy. We can't decouple the correlation of empirical policy. Thus in general-sum games, independent certified policy does not work. So here, the learning objective becomes CCE.~\yub{Note to self: polish this discussion}

Because each player independently follows no-regret learning, the sample complexity is only related to $A_i$, so the overall sample complexity only requires $\max_{i\in[m]}A_i$, getting rid of the (exponential) dependence of $m$.

After running  Algorithm \ref{algorithm:nash_v_general} for all $m$ players, we use joint certified policy (Algorithm \ref{algorithm:certified_policy_general}) to get a general (non-Markov) correlated policy which is an $\epsilon$-approximate CCE.~\yub{Say in essence what is learned by V learning, and why that gives CCE.}~\yub{Later, comment on why this only requires $\max A_i$ samples. this is because of independent learning.}\ziang{$\surd$}

\begin{algorithm}[t]
% \setstretch{1.2}
   \caption{V-Learning for Markov Games ($i$-th player)}
   \label{algorithm:nash_v_general}
   \begin{algorithmic}[1]
      \STATE {\bfseries Initialize:} For any $(s, a, h)$, set $\up{V}_{h,i}(s)\setto H$, $\underline{V}_{h,i}(s)\setto 0$, $\up{L}_{h,i}\setto 0$, $\mu_h(a|s) \setto 1/A_i$, $N_h(s)\setto 0$.
      \FOR{episode $k=1,\dots,K$}
      \STATE Receive $s_1$.
      \FOR{step $h=1,\dots, H$}
      \STATE Take action $a_h \sim \mu_h(\cdot |s_h)$, observe the action $a'_h$ from the other players.
      \STATE Observe reward $r_{h,i}=r_{h,i}(s_h, a_h, a'_h)$ and next state $s_{h+1}$ from the environment.
      \STATE Update accumulators: $t\defeq N_{h}(s_h)\setto N_{h}(s_h) + 1$.
      \STATE $\up{V}_{h,i}\left(s_{h}\right) \setto  \left(1-\alpha_{t}\right) \up{V}_{h,i}\left(s_{h}\right)+\alpha_{t}\left(r_{h,i}\left(s_{h}, a_{h}, a'_{h}\right)+\up{V}_{h+1,i}\left(s_{h+1}\right)+\up{\beta}_{t}\right)$
      \STATE $\underline{V}_{h,i}\left(s_{h}\right) \setto  \left(1-\alpha_{t}\right) \underline{V}_{h,i}\left(s_{h}\right)+\alpha_{t}\left(r_{h,i}\left(s_{h}, a_{h}, a'_{h}\right)+\underline{V}_{h+1,i}\left(s_{h+1}\right)-\up{\beta}_{t}\right)$
      \FOR{all $a \in \mc{A}_i$}
      \STATE $\up{\ell}_{h,i}(s_h, a) \setto [H - r_{h,i}-\min\{\up{V}_{h+1,i}(s_{h+1}),H-h\}] \mathbb{I}\{a_h=a\}/[\mu_h(a_h|s_{h}) +\up{\eta}_{t}]$.
      \STATE $\up{L}_{h,i}(s_h,a)\setto (1-\alpha_t)\up{L}_{h,i}(s_h,a)+\alpha_t\up{L}_{h,i}(s_h,a)$
      % \STATE $\up{L}_h( s_h, a)  \setto ( 1-\alpha _t )\up{L}_h( s_h,a ) +\alpha_t \up{\ell}_h(s_h, a)$.
      \ENDFOR
      \STATE Set $\mu_h(\cdot |s_h) \propto \exp[-(\up{\eta}_t/\alpha_t) \up{L}_{h,i}( s_h, \cdot)]$.
      \ENDFOR
      \ENDFOR
   \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
% \setstretch{1.2}
   \caption{Certified correlated policy $\hat\pi$ for general-sum Markov games}
   \label{algorithm:certified_policy_general}
   \begin{algorithmic}[1]
      \STATE sample $k$ $\setto$ Uniform([K]).
      \FOR{step $h=1,\dots,H$}
      \STATE observe $s_h$, and set $t\setto N_h^k(s_h)$.
      \STATE sample $l\in[t]$ with $\P(l=j) = \alpha_t^j$.
      \STATE $k\setto k_t^l(s_h)$.
      \STATE jointly take action $(a_{h,1}, a_{h,2},\dots,a_{h,m})\sim \prod_{i=1}^m\mu_{h,i}^k(\cdot|s_h)$.~\yub{all players use the same $k$, therefore is correlated policy}
      \ENDFOR
   \end{algorithmic}
\end{algorithm}

After running  Algorithm \ref{algorithm:nash_v_general} for all $m$ players and Algorithm \ref{algorithm:certified_policy_general}, we can learn a certified policy $\hat\pi$. Then,

\begin{theorem}\label{theorem:proof_general_cce}
With probability at least $1-p$, if we run Algorithm \ref{algorithm:nash_v_general} for all $m$ players and Algorithm \ref{algorithm:certified_policy_general} for $K$ episodes with 
$$
K\ge \Omega(H^5 S \max_{i\in[m]}A_i \iota /\epsilon^2),
$$
then the certified joint policy $\hat\pi$ will be $\epsilon$-approximate CCE, i.e. $V_{1,i}^{\dagger,\hat\pi_{-i}}(s_1)- V_{1,i}^{\hat\pi} (s_1)\le \epsilon$ for all $i=1,2,\dots,m$.
\end{theorem}

The proof is deferred to appendix, section \ref{section:proof in CCE}. We can learn the approximate CCE from general-sum Markov games efficiently. This sample complexity upper bound $\widetilde O(H^5S\max_{i\in[m]}A_i/\epsilon^2)$ significantly improves the best existing sample complexity upper bound for approximate CCE, $\widetilde O(H^3S^2\prod_{i=1}^mA_i/\epsilon^2)$ in \cite{liu2021sharp}. And from Theorem \ref{theorem:proof_general_cce}, we know that there's no exponential barrier w.r.t. $m$ in computing the approximate CCE in general-sum Markov games.%~\yub{proof is deferred to appendix xx}



==> deprecated/old.tex <==
% \section{Algorithm and analysis}

% We describe our algorithm Nash-V-Advantage in Algorithm~\ref{algorithm:nash_v_adv}.

% \paragraph{Stage-wise updates}
% Define $e_1=H$ and $e_{i+1}=\floor{(1+1/H)e_i}$ for all $i\ge 1$. Let $\mc{L}\defeq \set{\sum_{i=1}^j e_i: j=1,2,3,\dots}$ denote the indices for the end of the stages.

% \paragraph{Learning $\up{V}$ and $\up{V}^{\rf}$}
% Whenever we observe a tuple $(s_h, a_h, b_h, r_h, s_{h+1})$, we perform the following moving average updates to the estimated mean and variances of the value functions:~\yub{Notation $\check{\mu}$ does not have upper bar. To be changed.}
% \begin{align}
%     & \check{\mu} \defeq \check{\mu}_h(s_h) \settoplus \up{V}_{h+1}(s_{h+1}) - \up{V}^{\rf}_{h+1}(s_{h+1}); \qquad
%     \check{v} \defeq \check{v}_h(s_h) \settoplus r_h + \up{V}_{h+1}(s_{h+1}) \label{equation:mu-update} \\
%     & \check{\sigma} \defeq \check{\sigma}_h(s_h) \settoplus \paren{\up{V}_{h+1}(s_{h+1}) - \up{V}^{\rf}_{h+1}(s_{h+1})}^2. \label{equation:sigma-update}
% \end{align}
% Also the following updates:
% \begin{align}
%     \label{equation:mu-ref-update}
%     \mu^{\rf} \defeq \mu^{\rf}_h(s_h) \settoplus r_h + \up{V}^{\rf}_{h+1}(s_{h+1}); \qquad
%     \sigma^{\rf} \defeq \sigma^{\rf}_h(s_h) \settoplus \paren{r_h + \up{V}^{\rf}_{h+1}(s_{h+1})}^2.
% \end{align}
% We also set
% \begin{align}
%     \label{equation:n0}
%     N_0 \defeq \ceil{c_4SAH^5\iota / \beta^2}
% \end{align}
% to be the visitation threshold for updating the reference value function, where $\beta$ is an accuracy parameter to be determined.

% \paragraph{Certified policies}
% We use Algorithm ??? to extract a policy after playing.~\yub{TBA.}

% \begin{algorithm}[t]
% % \setstretch{1.2}
%   \caption{Nash-V-Advantage (the max-player version)}
%   \label{algorithm:nash_v_adv}
%   \begin{algorithmic}[1]
%       \REQUIRE Learning rate $\set{\up{\eta}_t}_{t\ge 1}$. Constants $c_1,c_2,c_3>0$. Accuracy parameter $\beta>0$.
%       \STATE {\bfseries Initialize:} For any $(s, a, h)$, set $N_h(s)\setto 0$, $\check{N}_h(s)\setto 0$, $\up{V}_{h}(s)\setto H-h+1$, $\up{V}^{\rf}_h(s)\setto H$, $\mu_h(a|s) \setto 1/A$.
%       \FOR{episode $k=1,\dots,K$}
%       \STATE Receive $s_1$.
%       \FOR{step $h=1,\dots, H$}
%       \STATE Take action $a_h \sim \mu_h(\cdot |s_h)$, observe the action $b_h$ from opponent.
%       \STATE Observe reward $r_h=r_h(s_h, a_h, b_h)$ and next state $s_{h+1}$ from the environment.
%       \STATE Update accumulators: $n\defeq N_{h}(s_h)\setto N_{h}(s_h) + 1$, $\check{n}\defeq \check{N}_h(s_h)\setto \check{N}_h(s_h) + 1$. 
%       \STATE {{\color{blue} \tt \# Update policy}}
%       \FOR{all $a \in \mc{A}$}
%       \STATE $\up{\ell}_h(s_h, a) \setto [H-h+1 - r_h-\up{V}_{h+1}(s_{h+1})] \mathbb{I}\{a_h=a\}/[\mu_h(a_h|s_{h}) +\up{\eta}_{\check{n}}]$.
%       % \STATE $\up{L}_h( s_h, a)  \setto ( 1-\alpha _t )\up{L}_h( s_h,a ) +\alpha_t \up{\ell}_h(s_h, a)$.
%       \ENDFOR
%       \STATE Set $\mu_h(\cdot |s_h) \propto \mu_h(\cdot | s_h) \cdot \exp[-\up{\eta}_{\check{n}} \up{\ell}_h( s_h, \cdot)]$.
%       \STATE {{\color{blue} \tt \# Track statistics and optionally update the value estimates}}
%       \STATE Perform updates~\eqref{equation:mu-update},~\eqref{equation:sigma-update}, and~\eqref{equation:mu-ref-update}.
%       \IF{$n\in\mc{L}$}
%       \STATE {{\color{blue} \tt \# Compute bonus and update $\up{V}$}}
%       \begin{align}
%           & b \setto c_1\sqrt{\frac{\sigma^{\rf}/n - (\mu^{\rf}/n)^2}{n}\iota} + c_2\sqrt{\frac{\check{\sigma}/\check{n} - (\check{\mu}/\check{n})^2}{\check{n}}\iota} + c_3\cdot \frac{H\iota}{\check{n}^{3/4}}; \\
%           & \bar{b} \setto 2\sqrt{H^2A\iota/\check{n}}; \\
%           & \up{V}_h(s_h) \setto \min\set{\frac{\check{v}}{\check{n}}+\bar{b}, \frac{\mu^{\rf}}{n} + \frac{\check{\mu}}{\check{n}} + b, \up{V}_h(s_h)}.
%       \end{align}
%       \STATE {{\color{blue} \tt \# Reset accumulators and policy}}
%       \STATE $\check{N}_h(s_h),\check{\mu}_h(s_h),\check{v}_h(s_h), \check{\sigma}_h(s_h)\setto 0$.
%       \STATE Set $\mu_h(\cdot | s_h) \setto 1/A$.
%       \ENDIF
%       \IF{$N_h(s_h)=N_0$ (where $N_0$ is defined in~\eqref{equation:n0})}
%       \STATE $\up{V}^{\rf}_h(s_h)\setto \up{V}_h(s_h)$. \quad {{\color{blue} \tt \# Learn $\up{V}^{\rf}$}}
%       \ENDIF
%       \ENDFOR
%       \ENDFOR
%   \end{algorithmic}
% \end{algorithm}

% \section{Problems to be solved}
% \subsection{Stronger Adversarial bandit lemma}
% Using a superscript $k$ to denote values at the beginning of the kth episode. 
% To prove the UCB is valid, we need to prove $\up{V}^{k}_h(s) \ge V_h^\star (s) \ge \underline{V}_h^k(s)$ for all $(s,h,k)\in \mc{S} \times [K] \times [H]$ with a high probability.

% Following the proof of Nash V-Learning, we can prove this by backward induction. The chaim is true for $h=H+1$. Assume it's true for $h+1$, we have
% \begin{align}
%     V_h^\star(s)&=\max_\mu \min_\nu \mathbb{D}_{\mu\times\nu}\left(r_h + \mathbb{P}_h V_{h+1}^\star\right)(s)\\
%     &=\max_\mu \sum_{i=1}^{\check{n}}\frac{1}{\check{n}}\min_\nu \mathbb{D}_{\mu\times\nu}\left(r_h + \mathbb{P}_h V_{h+1}^\star\right)(s)\\
%     &\le \max_\mu \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu\times\nu_h^{\check{k}_i}}\left(r_h + \mathbb{P}_h V_{h+1}^\star\right)(s)\\
%     &\le \max_\mu \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu\times\nu_h^{\check{k}_i}}\left(r_h + \mathbb{P}_h\up{V}_{h+1}^{\check{k}_i}\right)(s).
% \end{align}

% So we need a lemma similar to lemma 14 in Nash V-learning:
% \begin{equation}
% \begin{aligned}
%     \max_\mu \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu\times\nu_h^{\check{k}_i}}\left(r_h + \mathbb{P}_h\up{V}_{h+1}^{\check{k}_i}\right)(s)&-
%     \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \left[r_h\left(s,a_h^{\check{k}_i},b_h^{\check{k}_i}\right) + \up{V}_{h+1}^{\check{k}_i}\left(s_{h+1}^{\check{k}_i}\right)\right]\\
%     &\le \text{Bonus}.
% \end{aligned}   
% \label{Superiority-of-mu}
% \end{equation}

% By Hoeffding inequality,
% \begin{equation}
% \begin{aligned}
%     \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu_h^{\check{k}_i}\times\nu_h^{\check{k}_i}}\paren{r_h+\mathbb{P}_h\up{V}_{h+1}^{\check{k}_i}}(s)
%     &-
%      \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \left[r_h\left(s,a_h^{\check{k}_i},b_h^{\check{k}_i}\right) + \up{V}_{h+1}^{\check{k}_i}\left(s_{h+1}^{\check{k}_i}\right)\right]\\
%      &\le 2\sqrt{H^2\iota/\check{n}}.
% \end{aligned}    
% \end{equation}

% So we only need to bound
% \begin{align}
%     \max_\mu \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu\times\nu_h^{\check{k}_i}}\left(r_h + \mathbb{P}_h\up{V}_{h+1}^{\check{k}_i}\right)(s)
%     -
%     \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu_h^{\check{k}_i}\times\nu_h^{\check{k}_i}}\paren{r_h+\mathbb{P}_h\up{V}_{h+1}^{\check{k}_i}}(s) .
% \end{align}

% Back to the definition of $\up{V}_h(s_h)$, $\up{V}_h(s_h) \setto \min\set{\frac{\check{v}}{\check{n}}+\bar{b}, \frac{\mu^{\rf}}{n} + \frac{\check{\mu}}{\check{n}} + b, \up{V}_h(s_h)}.$

% If new value of $\up{V}_h(s_h)$ equals $\frac{\check{v}}{\check{n}}+\bar{b}$, then $\up{V}^{k}_h(s) \ge V_h^\star (s)$ because we can get (\ref{Superiority-of-mu}) with bonus $\bar{b} = C\sqrt{H^2A\iota/\check{n}}$ by applying the bandit lemma in Nash V-learning.

% If new value of  $\up{V}_h(s_h)$ equals $\frac{\mu^{\rf}}{n} + \frac{\check{\mu}}{\check{n}} + b$, we may need something different from the bandit lemma in Nash V-learning to show $\up{V}^{k}_h(s) \ge V_h^\star (s)$. First, we want to get an upper bound of 
% \begin{align}
%     \max_\mu\sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu\times\nu_h^{\check{k}_i}}\paren{\mathbb{P}_h\paren{\up{V}_{h+1}^{\check{k}_i}-\up{V}_{h+1}^{\text{ref},\check{k}_i}}}(s)-
%      \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \left[ \up{V}_{h+1}^{\check{k}_i}\left(s_{h+1}^{\check{k}_i}\right)-\up{V}_{h+1}^{\text{ref},\check{k}_i}\left(s_{h+1}^{\check{k}_i}\right)\right](s)
% \end{align}
% like $C\sqrt{A\cdot\frac{\check{\sigma}/\check{n} - (\check{\mu}/\check{n})^2}{\check{n}}\iota} + \text{something} $.

% Again, by concentration inequality, we need to bound ( however, here, the price of using Hoeffding concentration inequality is still $\frac{cH}{\check{n}^{1/2}}$, larger than $\frac{cH}{\check{n}^{3/4}}$. Bernstein inequality may be needed.)
% \begin{align}
%     \max_\mu\sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu\times\nu_h^{\check{k}_i}}\paren{\mathbb{P}_h\paren{\up{V}_{h+1}^{\check{k}_i}-\up{V}_{h+1}^{\text{ref},\check{k}_i}}}(s)-
%     \sum_{i=1}^{\check{n}}\frac{1}{\check{n}} \mathbb{D}_{\mu_h^{\check{k}_i}\times\nu_h^{\check{k}_i}}\paren{\mathbb{P}_h\paren{\up{V}_{h+1}^{\check{k}_i}-\up{V}_{h+1}^{\text{ref},\check{k}_i}}}(s)
% \end{align}
% with $C\sqrt{A\cdot \frac{\check{\sigma}/\check{n} - (\check{\mu}/\check{n})^2}{\check{n}}\iota}.$ This can again formalized as an adversarial linear bandit problem.

% The loss vector is 
% \begin{align}
% l_t(a) = \mathbb{E}_{b\sim\nu_h^{\check{k}_t},s\sim P(\cdot |s_h^{\check{k}_t},a,b)}\paren{\up{V}_{h+1}^{\check{k}_t}(s)- \up{V}_{h+1}^{\text{ref},{\check{k}_t}}(s)}.
% \end{align}
% Thus, the above quantity we want to bound becomes 
% \begin{align}
%     \max_\mu\frac{1}{T}\sum_{t=1}^T \langle \mu,l_t\rangle-\frac{1}{T}
%     \sum_{t=1}^T\langle \mu^{t},l_t\rangle.
% \end{align}
% Suppose at time $t$, the agent select action $a^t$. After time $t$, the agent can observe loss $\Tilde{l}_t(a^t)$ which is unbiased estimator of $l_t(a^t).$

% \textbf{Question}: For fixed action space, can we design an update rule for $\mu$, such that 
% \begin{align}
% \max_\mu\frac{1}{T}\sum_{t=1}^T \langle \mu,l_t\rangle-\frac{1}{T}
%     \sum_{t=1}^T\langle \mu^{t},l_t\rangle
%     \le
%     \mc{O}\paren{\sqrt{\frac{A \sum_{t=1}^T\paren{\Tilde{l}_t(a^t)-\bar{l}}^2}{T^2}}}
% \end{align}
% with high probability, where $\bar{l}$ is the arithmetic mean of $\Tilde{l}_t(a^t),t=1,2,\dots,T.$ 

% We can consider the case in which the agent knows the exact value of $l_t(a^t)$ after time $t$, i.e. $\Tilde{l}_t(a^t)=l_t(a^t)$ first.~\yub{correct, we only need to consider this case. The entire adv bandit problem has no randomness in $\ell_t$, and we then apply it where $\ell_t$ is the realization of some random variables.}

% {\bf Question}: Find an update rule jointly for $(\mu, \nu)$ such that
% \begin{align}
% \max_\mu\frac{1}{T}\sum_{t=1}^T \langle \mu,Q_t\nu^t\rangle -\min_\nu \frac{1}{T}
%     \sum_{t=1}^T\langle \mu^{t},Q_t \nu\rangle
%     \le
%     \mc{O}\paren{\sqrt{\frac{(A+B) \sum_{t=1}^T\paren{\Tilde{l}_t(a^t, b^t)-\bar{l}}^2}{T^2}}}
% \end{align}
% where $\Tilde{l}_t(a^t, b^t)$ is a random sample with mean $\langle \mu^t, Q_t\nu^t\rangle$, and $\bar{l}$ is the artihmetic mean of $\Tilde{l}_t(a^t, b^t)$ over $t=1,\dots,T$. Can we prove this when $Q_t\equiv Q$?

% \subsection{More efficient algorithm for zero-sum matrix game}
% There's another model-based way may be possible to achieve optimal algorithms for Markov games. So can we achieve $\mathcal{O}(\sqrt{(A+B)T})$ regret bound for stochastic zero-sum matrix game with UCB-type algorithm. (i.e. don't use bandit lemmas because we still don't have bernstein type bound for bandit problem.) Classical UCB type algorithm based on Hoeffding inequality gives regret bound $\mathcal{O}(\sqrt{ABT})$.

==> deprecated/value_iteration.tex <==
\section{Value iteration for CCE}

\begin{align*}
    V^{\dagger_i, \hat{\pi}^k_{h, -i}}_{h,i}(s) = \max_{\pi_i} \sum_{j=1}^t \alpha_t^j \mathbb{D}_{\pi_i \times \pi^{k^j}_{h, -i}} \brac{r_{h,i} + V^{\dagger_i, \hat{\pi}^{k^j}_{h+1, -i}}_{h+1, i}}(s).
\end{align*}

\begin{align*}
    V^{\mu, \hat{\pi}^k_{1, -i}}_{1, i}(s_1)
\end{align*}
where $\mu=\set{\mu_h(\cdot | s_h, s_{h-1}, a_{h-1}, r_{h-1}, \dots, s_1, a_1, r_1)}$.

We argue $\hat{\pi}^K_{1, -i}$ is a general non-Markovian and correlated policy. $\hat{\pi} = \{\hat{\pi}_{h}(a_{1:m} \vert s_h, history) \}$. We define $\hat{\pi}_{-i} \defeq \set{ \hat{\pi}_h(a_{-i} \vert s_h, history)  }$. We then argue for the specific $\hat{\pi}^k_{1}$, the induced $\hat{\pi}_{-i}$ satisfies the above recursion.

\begin{align*}
    V^{\pi}_{h, i}(s)
\end{align*}

\begin{align*}
    V^{\pi}_{h, i}(s_h, history)
\end{align*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

